Thresholding based Efficient Outlier Robust PCA

We consider the problem of outlier robust PCA (OR-PCA) where the goal is to recover principal directions despite the presence of outlier data points. That is, given a data matrix $M^*$, where $(1-\alpha)$ fraction of the points are noisy samples from a low-dimensional subspace while $\alpha$ fraction of the points can be arbitrary outliers, the goal is to recover the subspace accurately. Existing results for \OR-PCA have serious drawbacks: while some results are quite weak in the presence of noise, other results have runtime quadratic in dimension, rendering them impractical for large scale applications. In this work, we provide a novel thresholding based iterative algorithm with per-iteration complexity at most linear in the data size. Moreover, the fraction of outliers, $\alpha$, that our method can handle is tight up to constants while providing nearly optimal computational complexity for a general noise setting. For the special case where the inliers are obtained from a low-dimensional subspace with additive Gaussian noise, we show that a modification of our thresholding based method leads to significant improvement in recovery error (of the subspace) even in the presence of a large fraction of outliers.

==> ArXiv/algCl.tex <==
%!TEX root = rpca.tex
%\subsection{Algorithms}
\label{sec:algCl}

Recall that the goal is to estimate $\Uo$, the left singular vectors of $\Lo$. However, SVD of $\Mo$ can lead to singular vectors arbitrary far from $\Uo$, because a few column of $\Co$ can be so large that they can bias entire singular vectors in their direction. 

Our algorithm instead tries to exploit two key structural properties of the problem: sparsity of $\Co$ and incoherence of $\Lo$. Our algorithm maintains a column-sparse estimate $\Cot{t}$ of $\Co$. Each iteration of the algorithm computes a low-rank approximation of an estimate of the inliers $\Mo-\Cot{t}=\Lo+\Co-\Cot{t}$. Note that if $(I-\Uo(\Uo)^\top)\Co=(I-\Uo(\Uo)^\top)\Cot{t}$, then left singular vectors of $\Mo-\Cot{t}$ will be $\Uo$. 

%Now, $\norm{(I-\Uo(\Uo)^\top)(\Co-\Cot{t})}$ can be bounded effectively using {\em column-sparsity} of $\Co$.Hence, using standard matrix perturbation results, top singular vectors $\Uot{t}$ of $\Mo-\Cot{t}$ will be close to $\Uo$. 

Our next step finds {\em residual} length of each column $\Mo_i$ when projected on to the orthogonal subspace to $\Uot{t}$. If length of each outlier is smaller compared to the smallest singular value of $\Lo$, then using sparsity of $\Cot{t}$ and $\Co$, we can show that $\Uot{t}$ is "close" to $\Uo$ in all directions. So, the residual of some of the outliers will stand out and those columns can be removed. This is achieved by the hard-thresholding step 5, 8 of Algorithm~\ref{alg:ncpcacl}. 

A big challenge in this scheme is that if a column of the perturbation matrix $\Co-\Cot{t}$ is "very" long compared to smaller singular values of $\Lo$, then they can  perturb some directions of $\Uo$ significantly. This will lead to a failure of the above thresholding approach. However, in such a case, some of the columns of $\Co-\Cot{t}$ will be close to a few spurious singular vectors in $\Uot{t}$ (our current estimate of $\Uo$). Hence, projection of such outliers along $\Uot{t}$ will be inordinately long. On the other hand, due to incoherence of $\Lo$, inliers' projection along $\Uot{t}$ can be bounded in magnitude. So, we can safely threshold out certain outliers. Steps 6, 8 of Algorithm~\ref{alg:ncpcacl} perform this thresholding operation.  

In summary, our algorithm computes low-rank approximation of $\Mo-\Cot{t}$ and uses the obtained singular vectors $\Uot{t}$ to threshold out a few columns of $\Cot{t}$ to obtain next estimate $\Cot{t+1}$ of $\Co$. See Algorithm \ref{alg:ncpcacl} for a pseudo-code of our approach. 

{\em Time Complexity}: Note that the computationally most expensive operation in each iteration is that of SVD which requires $O(ndr)$ time. So, the overall time complexity of the algorithm is $O(ndr\cdot T)$. As we show in Section~\ref{sec:po}, as long as $\Co$ is column-sparse, $T\approx \log \frac{1}{\epsilon}$ suffices to obtain an $\epsilon$ approximation to $\Uo$. So, the overall complexity of the algorithm is $O(ndr\cdot \log\frac{20\|\Mo\|_2}{\epsilon})$. Note that typically SVD computation is approximate, while all three of our algorithms and analyses assumes exact SVD. However, extension of our analysis to allow for small additive error is straightforward and we ignore it in favor of simplicity and readability. 

{\em Parameters}: The algorithm requires an estimate of rank $r$ and threshold parameter $\rho$ which in turn depends on estimate of incoherence $\mu$ of $\Lo$. We propose to set these parameters via cross-validation. Note that setting rank to be any value larger than rank of $\Lo$ will lead to recovery of $\Uo$, as long as $\Co$ is sparse enough. Similarly, if estimation of $\mu$ is larger than incoherence of $\Lo$, then it only effects number of corrupted columns in $\Co$ that can be allowed. So, a simple cross-validation approach with appropriately chosen grid-size leads to recovery of $\Uo$ as long as $\Co$ is sparse enough (as specified in Theorem~\ref{thm:thmCln}). 
% Hence, if each column of $\Co-\Cot{t}$ is "small", i.e., at the scale of $\|\Lo\|_2 \frac{\mu\sqrt{r}}{\sqrt{n}}$, then due to sparsity of $\Co-\Cot[t]$, $\Uo$ is not perturbed significantly (see Lemma~\ref{lem:}). 
%
%On the other hand, if one of the columns of 
%
%Recall that in this case, we are given $\Mo = \Do +\Co$ where $\Do = \Lo$ is a rank-$r$, $\mu$-incoherent matrix and $\Co$ has at most $\alpha$ non-zero columns. Our goal is to recover the subspace spanned by the columns of $\Lo$.
%Our algorithm consists of a single loop where in each iteration, we revise our estimate of the principal subspace $U^*$ and threshold data points which we believe to be outliers. The main insights involved in the design of the algorithm are as follows:
%
%\begin{enumerate}
%	\item If the estimate of the principal subspace is far from the true subspace, then this can only be due to the presence of outliers in the points used to compute the principal subspace. Since there are much fewer outliers than clean data points, they will express much more along the estimated principal directions than the true data points and thus, can be efficiently detected and removed.
%	\item If an outlier has a large residual, thresholding it removes its influence on the principal directions beyond $r$.
%	\item If an outlier has not been thresholded, it does not influence the obtimal principal directions heavily and therefore does not hurt the performance of the algorithm.
%\end{enumerate}

%\begin{algorithm}[!h]
%  \caption{$U ~ =$ \ncpcacl$(M, r, \nThresh, \epsilon)$}
%  \label{alg:ncpcacl}
%  \begin{algorithmic}[1]
%    \STATE {\bf Input}: Data $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Threshold fraction $\nThresh$, Convergence criterion $\epsilon$
%    
%    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
%    \STATE $\Mt[0] \leftarrow M$
%
%    \FOR{Iteration $q = 0$ to $q = T$}
%      \STATE $[U_q, \Sigma_q, V_q] \leftarrow \mathcal{SVD}_r\lprp{\Mt[q]}$
%      
%      \STATE $E \leftarrow \Sigma_q^{-1} U_q^\top M$
%      \STATE $R \leftarrow (I - U_qU_q^\top)M$
%      
%      \STATE $\Mt[q + 1] \leftarrow \mathcal{HT}_{\nThresh} \lprp{M, E}$
%      \STATE $\Mt[q + 1] \leftarrow \mathcal{HT}_\nThresh \lprp{\Mt[q + 1], R}$
%    \ENDFOR
%      
%    \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_q\lprp{\Mt[T + 1]}$
%
%    \STATE {\bf Return: }$U$
%  \end{algorithmic}
%\end{algorithm}
\begin{algorithm}[!h]
	\caption{Thresholding based Outlier Robust PCA ($\ncpcacl$)}
	\label{alg:ncpcacl}
	\begin{algorithmic}[1]
		\STATE \textbf{Input}: Data $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Threshold fraction $\nThresh$, Number of iterations $T$
		
		% \STATE $T \leftarrow \log{\frac{20n\sigma_1(\Mo)}{\epsilon}}$
%		\STATE $\Mt[0] \leftarrow \Mo$
		\STATE $\Ct[0] \leftarrow 0$
		
		\FOR{Iteration $t = 0$ to $t = T$}
		\STATE $[\Uot{t}, \Sigma^{(t)}, \Vot{t}] \leftarrow \mathcal{SVD}_r\lprp{\Mo - \Ct[t]};\; \Lt[t] \leftarrow \Uot{t} \Sigma^{(t)} (\Vot{t})^{\top}$ \hspace{1em}{\color{blue}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\end{array} \right\}%
				{\small \begin{tabular}{c}Projection onto \\ space of \\ low rank matrices \end{tabular}}$}}}

%		\STATE $[U_q, \Sigma_q, V_q] \leftarrow \mathcal{SVD}_r\lprp{\Lt[q]}${\em /* SVD of $\Lt[q]$ */}
%		
		\STATE $R \leftarrow (I - \Uot{t}(\Uot{t})^\top)\Mo$ {\em /* Compute residual */}
		\STATE $E \leftarrow (\Sigma^{(t)})^{-1} (\Uot{t})^\top \Mo${\em /* Compute incoherence */}
		\STATE $\cs^{(t + 1)} \leftarrow \mathcal{HT}_\nThresh \lprp{R} \cup \mathcal{HT}_{\nThresh} \lprp{E} $ \hspace{14em}{\color{red}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\end{array} \right\}%
				{\small \begin{tabular}{c}Projection onto \\ space of \\ column sparse \\ matrices \end{tabular}}$}}}
		\STATE $\Ct[t + 1] \leftarrow \Mo_S $\\{\em /* Threshold points with high coherence or high residual*/}
		\ENDFOR
		
		\STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_r\lprp{\Mo - \Ct[T + 1]}$
		
		\STATE \textbf{Return: }$U$
	\end{algorithmic}
\end{algorithm}


==> ArXiv/algG.tex <==
%!TEX root = rpca.tex

%\subsection{Algorithm}

\begin{algorithm}[!ht]
	\caption{Thresholding based Outlier Robust PCA with Gaussian Noise ($\ncpcag$)}
	\label{alg:ncpcag}
	\begin{algorithmic}[1]
		\STATE \textbf{Input}: Corrupted matrix $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Incoherence Parameter $\mu$, Noise Level $\sigma$
		\STATE $\M \leftarrow \Mo$, $\tau \leftarrow true$
		\STATE $\zeta_1 \leftarrow \sigma \lprp{\frac{5}{4} \mu \sqrt{r} + d^{\frac{1}{2}} + 2 d^{\frac{1}{4}} \sqrt{\log\lprp{\frac{\mu^2 r}{c_2}}}}$, $\zeta_2 \leftarrow \sigma \sqrt{2r} \lprp{\frac{5}{4} \mu + 2 \sqrt{\log \lprp{\frac{\mu^2r^2d}{c_1}}}}$
		\STATE $\Ct[0] \leftarrow 0$, $\cs^{(0)} \leftarrow \{\}$, $\cs^{(-1)} \leftarrow \{0\}$, $t \leftarrow 0$
		
		\WHILE{$\cs^{(t)} \neq \cs^{(t - 1)}$}
		\STATE $[\Uot{t}, \Sigot{t}, \Vot{t}] \leftarrow \mathcal{SVD}_{r + 1} (\Mo - \Ct[t])$, $\ \ \Lt[t] \leftarrow \Uot{t}\Sigot{t}(\Vot{t})^\top$ \hspace{0em}{\color{blue}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\end{array} \right\}%
				\begin{tabular}{c}Projection onto\\ space of \\ low rank matrices \end{tabular}$}}} 
		\vspace{1em}
		\STATE $\mathcal{E}^{(t)} \leftarrow \{x: x = \Uot{t}\Sigot{t} y \text{ for some } \norm{y} \leq 2\mu \sqrt{r / n}\}$ 
		
		\STATE $\widehat{L}^{(t)} \leftarrow \Pr{\mathcal{E}^{(t)}}(\Lt[t])$ {\em /* Projection onto incoherent matrices */}
		\STATE $\mathcal{I} \leftarrow \left\{i: \norm{\Lt[t]_{i} - \widehat{L}^{(t)}_{i}} > \zeta_2\right\}$ {\em /* Points with large influence */}
		
		\STATE $\cs^{(t + 1)} \leftarrow \cs^{(t)} \cup \widetilde{\HT{\zeta_1}} \lprp{\Lt[t] - \widehat{L}^{(t)}}$ \\ {\em /* Updating support of outliers */}
		
		\IF{$\abs{I} \geq \frac{24nc_1}{\mu^2dr}$}
		\STATE $\cs^{(t + 1)} \leftarrow \cs^{(t + 1)} \cup \widetilde{\HT{\zeta_2}} \lprp{\Lt[t] - \widehat{L}^{(t)}}$ \hspace{5em}{\color{red}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\\{}\\{}\\{}\\{}\end{array} \right\}%
				\begin{tabular}{c}Projection onto space of \\ column sparse matrices \end{tabular}$}}} \\ {\em /* Update support of outliers */}
		\ENDIF
		\STATE $\Ct[t + 1] \leftarrow \Mo_{\cs^{(t + 1)}}$ \\ {\em /* Compute Sparse Projection */}
		\STATE $t \leftarrow t + 1$
		\ENDWHILE
		\STATE \textbf{Return: } U
	\end{algorithmic}
\end{algorithm}
%
%Recall from the notations, the second hard-thresholding operator $\widetilde{\HT{\zeta}}(N)$ is defined as:
%\begin{equation}
%  \label{eqn:httDef}
%  \widetilde{\HT{\zeta}}(N)=\{i:\ \text{s.t. } \|N_{i}\|_2 \geq \zeta\}.
%\end{equation}

%Our algorithm, \ncpcag\ for the special case of Gaussian random noise is presented in Algorithm \ref{alg:ncpcag}. %Before moving on, we would like to note that Theorem \ref{thm:thmGen} yields trivial results as soon as $\sigma \approx \frac{\sigma^*_1}{\sqrt{mn}}$. We will see that exploiting properties of Gaussian random vectors, enables us to tolerate values of $\sigma$ up to $\frac{\sigma^*_1}{\sqrt{n\log m}}$ which is almost a $\sqrt{m}$ improvement over the trivial application of Theorem \ref{thm:thmGen}. 
At a high level the philosophy of our \ncpcag\  algorithm is similar to \ncpcacl, i.e., we iteratively revise estimate of $\Co$ and the top singular vectors $\Uo$ using SVD and thresholding. That is, we iteratively threshold columns of $\Mo$, that we estimate are corrupted. However, due to Gaussian noise structure our thresholding step is significantly different than that of \ncpcacl\ or \ncpca. 

In particular, the choice of our thresholding criteria (see lines 10, 12 of Algorithm~\ref{alg:ncpcag}) uses the following two insights:
\begin{enumerate}[leftmargin=*,labelindent=\labelwidth+\labelsep]
	\item Length based thresholding (with respect to $\zeta_1$---line 10 of Algorithm~\ref{alg:ncpcag}): This thresholding step is used to ensure that the noise in each data point is at most $\order{\sigma \sqrt{d}}$. As the length of random Gaussian vector is at most $\order{\sigma \sqrt{d}}$ with high probability, only a small number of inliers are thresholded in this step (Lemma~\ref{lem:gauLthConc}).
	\item Projection based thresholding (with respect to $\zeta_2$---line 12 of Algorithm~\ref{alg:ncpcag}): In this step, we threshold points that have large projection along the estimated principal subspace. Note that out of $n$ columns of $\No$, at most $\order{\frac{1}{\mu^2 r d}}$ fraction of points have projected lengths greater than $\order{\sigma \sqrt{\log (d)}}$ along any direction (Lemma~\ref{lem:gauipConc}). Thus, chances of a inliers being thresholded in this step is low. On the other hand, any outlier that heavily influences a principal direction will be thresholded by this step.
\end{enumerate}
Algorithm~\ref{alg:ncpcag} provides a detailed pseudo-code of \ncpcag. Step 6 of the algorithm computes \textbf{rank}-$\mathbf{(r+1)}$ SVD of the estimate of inlier matrix $\Mo-\Co$. Step 7 defines a set of vectors, whose projection onto singular vectors of $\Lot{t}$ is ``typical'' for an inlier which is composed of a low-dimensional point perturbed by Gaussian noise vector of length $O(\sigma \sqrt{d})$. 

This set is used in step 10 to threshold outliers using the hard-thresholding operator $\widetilde{\HT{\zeta}}$ as defined in~\eqref{eqn:httDef}. Next, the set $\mathcal{I}$ consists of points which have a large influence on the estimated principal components. In the absence of outliers, the size of this set is bounded by $\frac{12 n c_1}{\mu^2 d r}$ with high probability. A large deviation in the size of this set indicates the presence of of outliers and the entire set is thresholded.

Note on Approximate Computation: We would like to note that the projection operator defined in step~8 of the algorithm can be computed efficiently to arbitrary accuracy. A pseudo-code for computing the required projection can be found in Algorithm~\ref{alg:fpr}. Algorithm~\ref{alg:fpr} reduces the problem to the univariate problem of finding the root of a monotonically decreasing function in a bounded interval which can be found efficiently via binary search. For the sake of simplicity, we assume that the projection step and the $\mathcal{SVD}$ are computed exactly. Our analysis can be extended to the case where the projection and $\mathcal{SVD}$ are computed approximately with some added technical difficulty. 

% if there are "too many" points with $\|Lt[t]_{:,i}-\hat{\Lt[t]}_{:,i}\|_2\geq \zeta_2$, then that indicates presence of outliers and our thresholding mechanism removes a fraction of those outliers.  ANY SUGGESTIONS FOR BETTER WORDING HERE?
% \begin{algorithm}[!h]
%   \caption{$L ~ =$ \ncpcag$(M, r, \mu, \sigma)$}
%   \label{alg:ncpcag}
%   \begin{algorithmic}[1]
%     \STATE {\bf Input}: Corrupted matrix $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Incoherence Parameter $\mu$, Noise Level $\sigma$
%     \STATE $\M \leftarrow \Mo$
%     \STATE $\tau \leftarrow true$
%     \STATE $\zeta_1 \leftarrow \sigma \lprp{\frac{5}{4} \mu \sqrt{r} + d^{\frac{1}{2}} + d^{\frac{1}{4}} \sqrt{\log\lprp{\frac{\mu^2 r}{c_2}}}}$
%     \STATE $\zeta_2 \leftarrow \sigma \sqrt{r} \lprp{\frac{5}{4} \mu \sqrt{r} + 2 \sqrt{\log \lprp{\frac{\mu^2rm}{c_1}}}}$

%     \WHILE{$\tau$}
%       \WHILE{$\tau$}
%         \STATE $\tau \leftarrow false$
%         \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_{r + 1} (\M)$
%         \STATE $\mathcal{E} \leftarrow \{x: x = U\Sigma y \text{ for some } \norm{y} \leq \mu \sqrt{r / n}\}$
%         \IF{$\HT{\zeta_1} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{U, \Sigma, 2\mu\sqrt{r / n}}\lprp{\M}} \neq \M$}
%           \STATE $\tau \leftarrow true$
%           \STATE $\M \leftarrow \HT{\zeta_1} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{U, \Sigma, 2\mu\sqrt{r / n}}\lprp{\M}}$
%         \ENDIF
%       \ENDWHILE

%       \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_{r + 1} (\M)$

%       \IF{$\frac{\abs{\left\{i: \norm{\Pr{U}(\M_i) - \Pr{U, \Sigma, 2\mu\sqrt{r / n}}(\M_i)} \geq \zeta_2\right\}}}{n} \geq \frac{6c_1}{\mu^2d}$}
%         \STATE $\tau \leftarrow true$
%         \STATE $\M \leftarrow \HT{\zeta_2} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{U, \Sigma, 2\mu\sqrt{r / n}} \lprp{\M}}$
%       \ENDIF
%     \ENDWHILE
%   \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[!h]
%   \caption{$L ~ =$ \ncpcag$(M, r, \mu, \sigma)$}
%   \label{alg:ncpcag}
%   \begin{algorithmic}[1]
%     \STATE {\bf Input}: Corrupted matrix $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Incoherence Parameter $\mu$, Noise Level $\sigma$
%     \STATE $\M \leftarrow \Mo$
%     \STATE $\tau \leftarrow true$
%     \STATE $\zeta_1 \leftarrow \sigma \lprp{\frac{5}{4} \mu \sqrt{r} + d^{\frac{1}{2}} + d^{\frac{1}{4}} \sqrt{\log\lprp{\frac{\mu^2 r}{c_2}}}}$
%     \STATE $\zeta_2 \leftarrow \sigma \sqrt{r} \lprp{\frac{5}{4} \mu + 2 \sqrt{\log \lprp{\frac{\mu^2rm}{c_1}}}}$

%     \WHILE{$\tau$}
%       \WHILE{$\tau$}
%         \STATE $\tau \leftarrow false$
%         \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_{r + 1} (\M)$
%         \STATE $\mathcal{E} \leftarrow \{x: x = U\Sigma y \text{ for some } \norm{y} \leq 2\mu \sqrt{r / n}\}$
%         \IF{$\HT{\zeta_1} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{\mathcal{E}}\lprp{\M}} \neq \M$}
%           \STATE $\tau \leftarrow true$
%           \STATE $\M \leftarrow \HT{\zeta_1} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{\mathcal{E}}\lprp{\M}}$
%         \ENDIF
%       \ENDWHILE

%       \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_{r + 1} (\M)$
%       \STATE $\mathcal{E} \leftarrow \{x: x = U\Sigma y \text{ for some } \norm{y} \leq 2\mu \sqrt{r / n}\}$

%       \IF{$\frac{\abs{\left\{i: \norm{\Pr{U}(\M_i) - \Pr{\mathcal{E}}(\M_i)} \geq \zeta_2\right\}}}{n} \geq \frac{6c_1}{\mu^2d}$}
%         \STATE $\tau \leftarrow true$
%         \STATE $\M \leftarrow \HT{\zeta_2} \lprp{\M, \Pr{U}\lprp{\M} - \Pr{\mathcal{E}} \lprp{\M}}$
%       \ENDIF
%     \ENDWHILE
%   \end{algorithmic}
% \end{algorithm}


==> ArXiv/algSimp.tex <==
%!TEX root = rpca.tex
%\subsection{Algorithm}
\label{sec:algGen}

Our algorithm for the general \orpca\ problem builds upon the \ncpcacl\ algorithm but with added complexity due to the presence of noise matrix $\No$. That is the algorithm alternately updates estimate of the outliers $\Cot{t}$ and the principal direction $\Uot{t}$ using two thresholding  operators along with SVD. %an estimate of $\Co$ and uses low-rank projection of $\Mo-\Co$ to obtain $\Uot{t}$, an estimate of $\Uo$. The algorithm then thresholds columns of $\Mo$ whose residual in orthogonal space to $\Uot{t}$ is large or along $\Uot{t}$ is abnormally large. 
However due to noise $\No$, our estimate of $\Uot{t}$ gets perturbed furthermore leading to arbitrary perturbation of the singular vectors of $\Uo$ corresponding to smaller eigenvalues of $\Lo$ and hence cannot be recovered. To alleviate this concern, our \ncpca\ algorithm proceeds via a pair of nested loops: 
\begin{enumerate}[leftmargin=*,labelindent=\widthof{\textbf{Outer Iteration on k:}}]
	\item[\textbf{Outer Iteration on k:}] The outer loop iterates over the rank-variable $k$ which represents the rank of the principal subspace we wish to estimate.
	\item[\textbf{Inner Iteration on t:}] The inner loop iteratively revises estimates of the principal subspace and a set of outliers until a stopping criteria is triggered.
\end{enumerate}
Intuitively, as in Algorithm~\ref{alg:ncpcacl}, each inner iteration of Algorithm~\ref{alg:ncpca} obtains a better estimate of $\Co$ and top-$k$ singular components of $\Lo$. That is, the $k$-th outer iteration after several of such inner iterations estimates $\Uo$ up to $\approx \sigma_k(\Lo)$. But when the noise $\|\No\|_F$ becomes comparable to the $k^{th}$ singular value of $\Lo$, then the algorithm terminates (Line 14, Algorithm~\ref{alg:ncpca}) as at that point it may not be possible to estimate the remaining singular vectors of $\Lo$. As we don't know $\|\No\|_F$ explicitly, we detect this event based on the number of data points which have a large influence on the estimated singular vectors (see lines 11, 12 of Algorithm~\ref{alg:ncpca}). 

Roughly, our stopping criterion allows us to make two statements regarding the termination of the algorithm:
\begin{enumerate}[leftmargin=*]
	\item When the algorithm terminates, the outlier columns that we have not thresholded will only have small influence on the estimated principal vectors. This is because all points with large influence will be thresholded before the estimate is computed.
	\item The algorithm will not terminate if $\sigma^*_k > > \frob{\No}$: The bound on $\frob{\No}$ ensures that not many inlier points can have large influence on estimate of the $k^{th}$ singular vector.
\end{enumerate}
By using the above two claims, our analysis shows that \ncpca\ recovers $\Uo$ up to $\sim \|\No\|_F$ error. 

{\em Time Complexity}: Time complexity of each inner iteration of \ncpca\ is $O(ndk)$. Hence, overall time complexity is $O(ndr^2)$, as $k$ can be as large as $r$. However, using a slightly more complicated algorithm and analysis (see Algorithm~\ref{alg:ncpcab}), we can search for appropriate $k$ using binary search, so the time complexity of the algorithm can be improved to $O(ndr\log r)$. %We present the simpler algorithm with worse time complexity for ease of exposition. 

{\em Parameter Estimation}: The algorithm requires $3$ parameters: rank $r$, threshold $\rho$ which depends on incoherence $\mu$ of $\Lo$ and expressivity parameter $\eta$. We can search for these parameters using a coarse-grid search as estimates of these parameters up to constants are enough for our algorithm to succeed albeit with a slightly stricter restriction (by constant factors) on the number of corrupted data points. 
% \begin{algorithm}[!h]
%   \caption{$U ~ =$ \ncpca$(M, r, \thresh, \nThresh, \epsilon)$}
%   \label{alg:ncpca}
%   \begin{algorithmic}[1]
%     \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Expressivity Parameter $\thresh$, Outlier Fraction $\nThresh$, Convergence criterion $\epsilon$
%     \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
%     \STATE $\Mt[0] \leftarrow M$
%     \STATE $U \leftarrow [e_1, \dots, e_r]$

%     \FOR{Outer Iteration $k = 1$ to $k = r$}
%     \STATE $\Mt[0] \leftarrow M$
%     \STATE $terminate \leftarrow false$
%       \FOR{Inner Iteration $q = 0$ to $q = T$}
%         \STATE $[U_q, \Sigma_q, V_q] \leftarrow \mathcal{SVD}_k\lprp{\Mt[q]}$
        
%         \STATE $E \leftarrow \Sigma_q^{-1} U_q^\top M$
%         \STATE $R \leftarrow (I - U_qU_q^\top)M$
        
%         \STATE $\Mt[q + 1] \leftarrow \mathcal{HT}_{2\nThresh} \lprp{M, E}$
%         \STATE $\Mt[q + 1] \leftarrow \mathcal{HT}_\nThresh \lprp{\Mt[q + 1], R}$

%         \STATE $nOut \leftarrow \abs{\{i: \norm{E_{i}} \geq \thresh\}}$
%         \STATE $\tau \leftarrow nOut \geq 2\nThresh n$
%       \ENDFOR
%       \IF{$\tau$}
%       	\STATE $break$
%       \ENDIF
%       \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_q\lprp{\Mt[T + 1]}$
%     \ENDFOR

%     \STATE {\bf Return: }$U$
%   \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[!ht]
  \caption{Thresholding based Noisy Outlier Robust PCA ($\ncpcan$)}
  \label{alg:ncpca}
  \begin{algorithmic}[1]
    \STATE \textbf{Input}: Corrupted matrix $\Mo \in \mathbb{R}^{d\times n}$, Target rank $r$, Expressivity parameter $\thresh$, Threshold fraction $\nThresh$, Inner iterations $T$
    % \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    % \STATE $\Mt[0] \leftarrow M$
    %\STATE $U \leftarrow [e_1, \dots, e_r]$

    \FOR{$k = 1$ to $k = r$}
    % \STATE $\Mt[0] \leftarrow M$
    \STATE $\Ct[0] \leftarrow 0$, $\tau \leftarrow false$
      \FOR{$t = 0$ to $t = T$}
        \STATE $[\Uot{t}, \Sigot{t}, \Vot{t}] \leftarrow \mathcal{SVD}_k\lprp{\Mo - \Ct[t]}$, $\Lt[t] \leftarrow \Uot{t}\Sigot{t}(\Vot{t})^\top$ \hspace{1em}{\color{blue}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}{}\end{array} \right\}%
        \begin{tabular}{c}Projection onto space of \\ low rank matrices \end{tabular}$}}}
        \vspace*{1.5em}
        \STATE $E \leftarrow (\Sigot{t})^{-1} (\Uot{t})^\top \Mo$ {\em /* Compute Incoherence */}
        \STATE $R \leftarrow (I - \Uot{t}(\Uot{t})^\top) \Mo$ {\em /* Compute residual */} 
        \hspace{5.7em}{\color{red}\rlap{\smash{$\left.\begin{array}{@{}c@{}}\\{}\\{}\\{}\end{array} \right\}%
        		\begin{tabular}{c}Projection onto space of \\ column sparse matrices \end{tabular}$}}}
        \STATE $\cs^{(t + 1)} \leftarrow \mathcal{HT}_{2\nThresh} \lprp{\Mo, E} \cup \mathcal{HT}_\nThresh \lprp{\Mo, R}$ 
        \STATE $\Ct[t + 1] \leftarrow \Mo_{\cs^{(t + 1)}}$

        \STATE $\nOut \leftarrow \abs{\{i: \norm{E_{i}} \geq \thresh\}}$ {\em /* Compute high incoherence points */}
        \STATE $\tau \leftarrow \tau \vee (\nOut \geq 2\nThresh n)$ {\em /* Check termination conditions */}
      \ENDFOR
      \IF{$\tau$}
        \STATE $break$
      \ENDIF
      \STATE $[U, \Sigma, V] \leftarrow \mathcal{SVD}_k\lprp{\Mo - \Ct[T + 1]}$
    \ENDFOR

    \STATE \textbf{Return: }$U$
  \end{algorithmic}
\end{algorithm}



==> ArXiv/algo.tex <==
%!TEX root = main.tex
\section{Algorithm - Without Noise}\label{sec:prob}

Here, we present our algorithm for solving the Robust PCA problem.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \ncpca$(M, r, \thresh, \beta, \epsilon)$}
  \label{alg:ncpca}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Thresholding Parameter $\thresh$, Incoherence Thresholding Parameter $\beta$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    % \FOR {Iteration $q = 0$ to $q = T$}
    %   \STATE $\zeta \leftarrow \thresh \sigma_1 (\Mt[q])$
    %   \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q]}$
    % \ENDFOR
    %
    % \STATE $\Mt[0] \leftarrow \Mt[T + 1]$

    \FOR{Outer Iteration $k = 0$ to $k = r$}
      \FOR{Inner Iteration $q = 0$ to $q = T$}
        \STATE $L = \Pk[k] (\Mt[q])$
        \STATE $\zeta \leftarrow \thresh \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma_{k}(\Mt[q]) + \sigma_{k + 1}(\Mt[q])}$
        \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q] - L}$
      \ENDFOR
      \IF{$\sigma_{k + 1}(\Mt[T + 1]) \leq \frac{\epsilon}{2n}$}
        \STATE \textbf{break}
      \ENDIF
      \STATE $[U, S, V] \leftarrow \mathcal{SVD}_{k + 1} \lprp{\Mt[T + 1]}$
      \STATE $\zeta \leftarrow 2\thresh \sigma_{k + 1}(\Mt[T + 1])$
      \STATE $\Mt[0] \leftarrow \HTz \lprp{\Mt[T + 1], \Mt[T + 1] - USV^\top}$
      \STATE $\Mt[0] \leftarrow \HTb \lprp{\Mt[0], US^{-1}U^{\top} \Mt[T + 1]}$
    \ENDFOR
    \STATE {\bf Return: }$\Pr{r}(\Mt[T + 1])$
  \end{algorithmic}
\end{algorithm}

Here, we $\mathcal{HT}_{\gamma}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htDef}
  (\mathcal{HT}_{\gamma}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ \norm{N_{:, i}} \leq \gamma \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}


==> ArXiv/algoAux.tex <==
%! TEX root = main.tex

\section{Algorithm - Auxilliary}
\label{sec:algAux}
Here, we introduce our algorithm which has a threshold on the maximum number of columns that are thresholded by the matrix at any time.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \auxAlgo$(M, r, \alpha^\prime, \epsilon)$}
  \label{alg:aux}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Maximum Thresholding fraction $\alpha^\prime$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    \FOR{Iteration $t = 0$ to $t = T$}
      \STATE $U^{(t)} \leftarrow LSV_r \lprp{\Mt[t]}$
      \STATE $\Mt[t + 1] \leftarrow \HTap\lprp{M, \Pr{U^{(t)}}^\perp \lprp{M}}$
    \ENDFOR
    \STATE {\bf Return: }$\Mt[T + 1]$
  \end{algorithmic}
\end{algorithm}

Here, we $\mathcal{HT}_{\alpha}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htADef}
  (\mathcal{HT}_{\alpha}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ N_{:, i} \text{ is one of the } \alpha n \text{ longest columns of N} \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}


==> ArXiv/algoN.tex <==
%!TEX root = main.tex
\section{Algorithm - Noisy Case}\label{sec:prob}

Here, we present our algorithm for solving the Robust PCA problem with noise. Due to the noise, it might be possible for columns in the support of $\Lo$ to get thresholded by our algorithm. To solve this problem, we will use the algorithm introducted for the case where there is no noise (Algorithm \ref{alg:ncpca}) except that we will only let $k$ range from $0$ till $r - 1$. Instead of the final outer iteration, we will run Algorithm \ref{alg:aux} which has a bound on the maximum number of columns that are ever thresholded in an iteration. We prove that if the noise ($\frob{\No}$) is suitably small, we will not threshold too many clean columns till we run Algorithm \ref{alg:aux}.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \ncpcan$(M, r, \thresh, \beta, \alpha^\prime, \mu, \epsilon)$}
  \label{alg:ncpcan}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Thresholding Parameter $\thresh$, Incoherence Thresholding Parameter $\beta$, Maximum Thresholding Parameter $\alpha^\prime$, Incoherence Parameter $\mu$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    \FOR{Outer Iteration $k = 0$ to $k = r - 1$}
      \FOR{Inner Iteration $q = 0$ to $q = T$}
        \STATE $L = \Pk[k] (\Mt[q])$
        \STATE $\zeta \leftarrow \thresh \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma_{k}(\Mt[q]) + \sigma_{k + 1}(\Mt[q])}$
        \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q] - L}$
      \ENDFOR

      \IF{$\sigma_{k + 1}(\Mt[T + 1]) \leq \frac{\epsilon}{2n}$}

        \STATE $[U^\prime, S^\prime, V^\prime] \leftarrow SVD_k(\Mt[T + 1])$
        \STATE $\widehat{L} \leftarrow \Pr{U^\prime S^\prime, 2\mu \sqrt{r / n}} (M)$
        \STATE $\widehat{C} \leftarrow M - \widehat{L}$

        \STATE \textbf{Return: } $(\widehat{L}, \widehat{C})$
      \ENDIF

      \STATE $[U, S, V] \leftarrow \mathcal{SVD}_{k + 1} \lprp{\Mt[T + 1]}$
      \STATE $\zeta \leftarrow 2\thresh \sigma_{k + 1}(\Mt[T + 1])$
      \STATE $\Mt[0] \leftarrow \HTz \lprp{\Mt[T + 1], \Mt[T + 1] - USV^\top}$
      \STATE $\Mt[0] \leftarrow \HTb \lprp{\Mt[0], US^{-1}U^{\top} \Mt[T + 1]}$
    \ENDFOR

    \STATE $L^\prime \leftarrow $ \auxAlgo$(\Mt[T + 1], r, \alpha^\prime, \epsilon / n^2)$
    \STATE $[U^\prime, S^\prime, V^\prime] \leftarrow SVD_r(L^\prime)$
    \STATE $\widehat{L} \leftarrow \Pr{U^\prime, S^\prime, 2\mu \sqrt{r / n}} (M)$
    \STATE $\widehat{C} \leftarrow M - \widehat{L}$

    \STATE {\bf Return: }$(\widehat{L}, \widehat{C})$
  \end{algorithmic}
\end{algorithm}

Here, we define $\mathcal{HT}_{\gamma}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htDef}
  (\mathcal{HT}_{\gamma}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ \norm{N_{:, i}} \leq \gamma \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}

We also define the incoherence preserving projection operator ($\Pr{U, S, \delta}$) on a matrix $A$ as follows:

\begin{equation}
  \label{eqn:iProjDef}
  (\Pr{U, S, \delta} (A))_{:, i} = \argmin\limits_{\norm{U S^{-1} U^\top y} \leq \delta} \norm{A_{:, i} - y}
\end{equation}


==> ArXiv/analysis.tex <==
%!TEX root = main.tex
\renewcommand{\u}{\bm{u}}
\section{Analysis - Without Noise}\label{sec:analysis}

\begin{assumption}
  \label{as:rank}
  \textbf{Rank and incoherence of $\Lo$: } $\Lo\in \mathbb{R}^{m\times n}$ is a rank-$r$ incoherent matrix, i.e., $\twonorm{e_{i}^{\top}V^*} \leq \mu \sqrt{\frac{r}{n}} \ \forall i\in [n]$, where $\Lo = U^*\Sigma^* (V^*)^{\top}$ is the SVD of $\Lo$.
\end{assumption}

\begin{assumption}
  \label{as:colSup}
  \textbf{Column Sparsity of $\Co$: } $\Co \in \mathbb{R}^{m\times n}$ is a column sparse matrix with column sparsity $\colSp$ satisfying $\colSp \leq \frac{c}{\mu^2r}$ for some suitable small constant $c$.
\end{assumption}

Assumptions \ref{as:rank} and \ref{as:colSup} as standard assumptions for the Robust PCA problem. Note that column sparsity above $\frac{1}{\mu^2r}$ cannot be tolerated by any algorithm for robust PCA as the low rank component and the column sparse component may become indistinguishable.

We obtain the following theorem guaranteeing the optimality of our algorithm under the assumptions specified.

% \begin{theorem}
%   \label{thm:master}
%   Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $L$ satisfying:
%   \begin{equation*}
%     \frob{L - \Lo} \leq \epsilon
%   \end{equation*}
% \end{theorem}

\begin{theorem}
  \label{thm:master}
  Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $\Lo$.
\end{theorem}

\textbf{Notation}: We use $Pos^{*}(\sigma)$ to denote the number of singular values of $\Lo$ greater than $\sigma$. Let the column support of a matrix be denoted as $\supp{M}$. Let $\itnorm{M}$ denote the length of the longest column of a matrix.

We track two important quantities during outer iteration $k$ through the proof of Theorem \ref{thm:master}:
\begin{equation}
  \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])},\ \itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}
\end{equation}

We will now present some lemmas useful for the analysis. The first lemma bounds the norm of a column sparse matrix.

\begin{lemma}
  \label{lem:spNrm}
  Let $A \in \mathbb{R}^{m \times n}$ be a column sparse matrix with column sparsity $\alpha$ such that $\itnorm{A} \leq B$. Then $\norm{A} \leq \sqrt{\alpha n} B$
\end{lemma}

\begin{proof}
  The forbenius norm of $A$ is bounded by $\sqrt{\alpha n} B$ which is an upper bound on $\norm{A}$.
\end{proof}

In the next lemma, we show that adding columns in the column space of an incoherent matrix does not change the incoherence condition for the columns that were present previously.

\begin{lemma}
  \label{lem:clInc}
  Let $M \in \mathbb{R}^{m \times n}$ be a rank $r$, $\mu$ incoherent matrix with singular value decomposition $U\Sigma V^{\top}$. Then adding matrix $C$ to $M$ such that $\supp{C} \cap \supp{M} = \phi$ and $\Pr{U}(C) = C$, then if $U^\prime \Sigma^\prime (V^\prime)^\top$ is the singular value decomposition of $M + C$, then the following inequality holds:
  \begin{equation*}
    \norm{e_{i}^\top V^\prime} \leq \mu \sqrt{\frac{r}{n}},\ \forall i \in \supp{M}
  \end{equation*}
\end{lemma}

\begin{proof}
  First, let $V_c^\top = (V^\top + \Sigma^{-1}U^\top C)$. We can now write $M + C = U\Sigma (V + V_c)$. $V^\prime$ now forms an orthogonal basis for $V + V_c$. Note that $\supp{V^\top} \cap \supp{V_c^\top} = \phi$. Hence, there exists an upper triangular matrix $R$ and an orthogonal matrix $Q$ such that $(V + V_c)RQ = V^\prime$. Now, we note that $(Q^\top R^\top) (I + V_c^\top V_c) RQ = I$ which implies $R^\top (I + V_c^\top V_c)R = I$. From this, we obtain that $\norm{R} \leq 1$. We continue to bound the required quantity as follows:
  \begin{equation*}
    \norm{e_{i}^\top V^\prime} = \norm{e_{i}^\top (V + V_c)RQ} \overset{(\zeta_1)}{\leq} \norm{e_{i}^\top(V + V_c)} \overset{(\zeta_2)}{\leq} \mu\sqrt{\frac{r}{n}}
  \end{equation*}
  Where $(\zeta_1)$ and $(\zeta_2)$ follow from the bound on $\norm{R}$ and the fact that $i \in \supp{M}$.
\end{proof}

We will denote by $\Ct[q]$ as the corrupted columns that have not been thresholded by the algorithm before inner iteration $q$. We will see that we will never threshold a column $i \in \supp{\Lo}$. Therefore, we can write $\Mt = \Lo + \Ct[q]$. In all the lemmas that follow, we will assume that $\thresh$ and $\incThresh$ are set to $2\mu\sqrt{\frac{r}{n}}$ and $2\mu\sqrt{\frac{r}{n}}$ respectively.

The theorem is proved by induction over the inner and outer loops respectively. We will first state a lemma which guarantees progress in the inner iteration.

\begin{lemma}
  \label{lem:inItProg}
  Let $\Mo = \Lo + \Co$ be a matrix such that $\Lo$ and $\Co$ satisfies Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Also, assume that the following conditions hold before the $q^{th}$ inner iteration:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{1,\ldots,k-1\}$
  \end{enumerate}
  Then, after the $q^{th}$ inner iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\supp{\Lo} \subset \supp{\Mt[q + 1]}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  First, we note that $\sigma_{k}(\Mt{q}) \geq \sigma^*_{k}$. We now decompose $\Mt{q}$ as $\Pr{U^*_{\sigma^*_k / 2}}(\Mt{q}) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Lo) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])$. Let $U_k$ denote singular vectors corresponding to the top $k$ singular vales of $\Mt$. We will now bound $\norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k / 2}}}^\perp}$.

  % By Weyl's perturbation inequality, we have
  % \begin{equation}
  %   \sigma_{i}(\Mt[q]) \leq \sigma^*_{i} + \norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])} \overset{(\zeta_1)}{\leq} \frac{16}{31} \sigma^*_k
  % \end{equation}

  By the Davis Kahan theorem, we get the following bound:
  \begin{equation}
    \label{eqn:projBound}
    \norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k} / 2}}^\perp} \leq \frac{\norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])}}{\sigma_k(\Mt{q}) - \sigma^*_{Pos^*(\sigma^*_{k} / 2) + 1}} \leq \frac{2\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])}}{\sigma^*_k}
  \end{equation}

  We now prove that the columns in the support of $\Lo$ are not thresholded by the algorithm. We fix $i$ such that $i \in \supp{\Lo}$.

  \begin{align}
    \label{eqn:clBound}
    \norm{(I - U_kU_k^\top) \Lo_i} &= \norm{(I - U_kU_k^\top) (\Lo + \Pr{U^*}(\Ct[q])) e_i} \\
        &\leq \mu\sqrt{\frac{r}{n}} \norm{(I - U_kU_k^\top) (\Lo + \Pr{U^*}(\Ct[q]))} \\
        &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - U_kU_k^\top)\Mt{q}} + \norm{\Pr{U^*}^\perp(\Ct[q])}} \\
        &\leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1} (\Mt) + \norm{\Pr{U^*}^\perp(\Ct[q])}}
  \end{align}

  The above inequalities prove that a column in the support of $\Lo$ will not be thresholded as part of the thresholding procedure.

  We will now bound the quantity $\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])e_i},\ \forall i \in \{1,\ldots,n\}$. For a thresholded column, the quantity is bounded by $0$. For a column that is not thresholded, we have:
  \begin{align*}
    \eta \geq \norm{(I - U_kU_k^\top)\Ct[q + 1]e_i} &= \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i) + \Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i))} \\
    &\geq \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)U^*\Sigma^*v} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)\Lo} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Lo + \Pr{U^*_{\sigma^*_k/2}}(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Mt - \Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)
  \end{align*}

  From this, we get:
  \begin{equation}
    \label{eqn:corBound}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} \leq \frac{32}{31} \lprp{\zeta + 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)}
  \end{equation}

  With these inequalities in hand, we can proceed to bound the value of $\sigma_{k + 1}(\Mt)$. Using Weyl's inequality, we know that $\sigma_{k + 1}(\Mt) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct)}$. Here, we consider two cases:

  \textit{Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}}$.

  \textit{Case 2: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$.

  We now bound $\sigma_k(\Mt)$. Similar to Case 2 above, consider index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_k$. Again, we know that $\sigma_{k}(\Mt) \leq \sigma^*_{k} + \norm{\Pr{U^*_{k - 1}}^\perp (\Ct)}$. And we also have that $ 2\sigma^*_{k} \geq \sigma^*_{i + 1} $ and that $ (U^*_{k - 1})^\perp \subset (U^*_{\sigma^*_i / 2})^\perp $. From these two observations, we have $\sigma_k(\Mt) \leq \frac{33}{32} \sigma^*_k$.

  From \ref{eqn:clBound}, we have for $i \in \supp{\Lo}$:

  \begin{equation*}
    \norm{(I - U_kU_k^\top)L^*_i} \leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma^*_{k + 1} + \frac{1}{16} \lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}} + \frac{\sigma^*_{k + 1}}{32}} \leq 2\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{equation*}

  Similarly, from \ref{eqn:corBound}, we have:
  \begin{align*}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} &\leq \frac{32}{31} \lprp{\zeta + 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{18\sigma_{k + 1} + 2\lprp{\frac{1}{2}}^{q + 1}\sigma_{k} + 16\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + 18\sigma^*_{k + 1}} + 30 \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + 18\sigma^*_{k + 1}} + \frac{30}{32}\lprp{\lprp{\frac{1}{2}}^{q}\sigma^*_k + \sigma^*_{k + 1}}} \\
    &\leq 24 \mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  With the two inequalities defined above, we have proved the lemma.
\end{proof}

In the following lemma, we will prove that the thresholding steps at the end of the outer loop establishes control on the quantity, $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}$.

\begin{lemma}
  \label{lem:incohCont}
  Let $\Mo = \Lo + \Co$ be a matrix such that $\Lo$ and $\Co$ satisfies Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Also, assume that the following conditions hold after the inner iteration in the $k^{th}$ outer iteration concludes:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[T + 1])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{0,\ldots,k\}$
  \end{enumerate}
  Then, after the $k^{th}$ outer iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k + 1} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\supp{\Lo} \subset \supp{\Mt[0]}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  Similarly to the previous lemma, we bound $ \sigma_{k + 1}(\Mt[T + 1]) $ by $ \lprp{\sigma^*_{k + 1}(\Mt[T + 1]) + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}}$. Now consider the index $i := \argmax\limits_j \sigma^*_j \geq \sigma^*_{k + 1}$. From our assumptions, we know that $\sigma^*_{i + 1} \leq 2\sigma^*_{k + 1}$. Also, we know that $(U^*_{k})^\perp \subset (U^*_{\sigma^*_{i} / 2})^\perp$. This implies that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \frac{1}{32} \sigma^*_{k + 1}$ by our assumptions on $\alpha$ and by using Lemma \ref{lem:spNrm}.

  We first prove the second claim of the lemma where we show that any column $i$ such that $i \in \supp{\Lo}$ is not thresholded.

  For the thresholding with respect to $\zeta$, we have:
  \begin{align*}
    \norm{(I - UU^\top) \Lo_i} &\leq \mu\sqrt{\frac{r}{n}}\norm{(I - UU^\top) U^*\Sigma^*} \\
    &\leq \mu\sqrt{\frac{r}{n}} \norm{(I - UU^\top) (\Lo + \Pr{\sigma^*_{k} / 2} (\Ct[T + 1]))} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - UU^\top) \Mt[T + 1]} + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Mt[T + 1]) + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])}} \\
    &\leq \frac{34}{32}\mu\sqrt{\frac{r}{n}}\lprp{\sigma^*_{k + 1}}
  \end{align*}

  where the last inequality holds from Lemma \ref{lem:spNrm}, our assumption on $\alpha$ and our assumption on $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])}$.

  Now, we will prove that the column $i$ is not thresholded in the second thresholding step.

  \begin{align*}
    \norm{US^{-1}U^\top \Lo_i} &\leq \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top \Lo} \\
    &\leq \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top (\Lo + \Pr{U^*_{\sigma^*_{k} / 2}} (\Ct)} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{US^{-1}U^\top \Mt[T + 1]} + \norm{US^{-1}U^\top \Pr{U^*_{\sigma^*_{k} / 2}}^\perp (\Ct)}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{2}{\sigma^*_{k + 1}} \norm{\Pr{U^*_{\sigma^*_{k}}}^\perp (\Ct)}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{2}{\sigma^*_{k + 1}} \frac{\sigma^*_{k + 1}}{32}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}}
  \end{align*}

  Thus, we have proved the second claim of the lemma. We will now prove the first claim of the lemma. We first note that a column $i \in \supp{\Ct[T + 1]}$ can be written as $USv + v_{res}$ such that $\norm{v} \leq 2\mu\sqrt{\frac{r}{n}}$ and $\norm{v_{res}} \leq \zeta$. We now prove claim 2 as follows:

  \begin{align*}
    &\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]_i}\\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top (USv + v_{res})} \\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top USv} +  \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top v_{res}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 4\mu\sqrt{\frac{r}{n}} \frac{2}{\sigma^*_{k + 1}} \sigma_{k + 1}(\Mt[T + 1]) \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 9 \mu\sqrt{\frac{r}{n}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{2\sigma_{k + 1}(\Mt[T + 1])}{\sigma^*_{k + 1}}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{33}{16}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \lprp{\Lo + \Ct[T + 1]}}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{1 + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]}} \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\norm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \norm{\sum\limits_{i = Pos^*(\sigma^*_k / 2) + 1}^{Pos^*(\sigma^*_{k + 1} / 2)} \frac{u^*_i (u^*_i)^\top}{\sigma^*_i} \Ct[T + 1]}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\sqrt{\alpha n} \itnorm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \frac{2\sqrt{\alpha n}}{\sigma^*_{k + 1} / 2} \itnorm{\Pr{U^*_{\sigma^*_{k} / 2}}^\perp \Ct}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu \sqrt{\frac{r}{n}} \lprp{\frac{1}{32} + \frac{1}{32}} \\
    &\leq 16\mu\sqrt{\frac{r}{n}}
  \end{align*}

  This establishes Claim 2 of the lemma.

\end{proof}

We can now prove the main theorem of the paper.

\begin{proof}
  \textit{Proof of Theorem \ref{thm:master}}
  We analyze the first outer iteration separately. And we subsequently prove the theorem through induction on the inner and outer iterations.

  First, we note that $\sigma_1 (\Mo) \geq  \sigma^*_1$. For our setting of $\thresh$, this ensures that we never threshold a column $i \in \supp{\Lo}$. We now prove an upper bound on $\sigma_1(\Mt[T + 1])$ at the end of the first inner iteration.

  We have the following recurrence inequality for $\sigma_1(\Mt[q]) \ \forall q \geq 1$ from Weyl's inequality and our condition on $\alpha$.
  \begin{equation}
    \label{eqn:sig1Rec}
    \sigma_1(\Mt[q]) \leq \sigma_1^* + \norm{\Ct[q - 1]} \leq \sigma_1^* + \frac{1}{64} \sigma_1(\Mt[q - 1])
  \end{equation}

  By expanding on this recurrence and from our setting of $T$, we get:
  \begin{equation}
    \sigma_1(\Mt[T + 1]) \leq \sigma_1^* \sum\limits_{i = 0}^{T} \lprp{\frac{1}{64}}^i + \lprp{\frac{1}{64}}^T \sigma_1(\Mo) \leq \frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n}
  \end{equation}

  In the if condition at the end of the first inner iteration, we consider two cases:
  \\
  \textit{Case 1: The Algorithm Breaks} In this case, we know that $\frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n} \leq \frac{\epsilon}{10n}$ which implies that $\sigma^*_1 \leq \frac{\epsilon}{10n}$. With this inequality, we have $\frob{\Lo - \Pr{r}(\Mt[T + 1])} \leq \frob{\Lo} + \frob{\Pr{r}(\Mt[T + 1])} \leq \sqrt{r} (\frac{\epsilon}{10n} + \frac{\epsilon}{10n}) \leq \frac{\epsilon}{5\sqrt{n}}$. Also, given our assumption on $\epsilon$, we have eliminated all the corrupted columns of $\Mo$.
  \\
  \textit{Case 2: The Algorithm Continues To the Next Iteration} In this case, we know that $\sigma_1^* \geq \frac{\epsilon}{12n}$. We will now prove that the assumptions of Lemma 4 are satisfied at the end of the first inner iteration.

  We know that each column $i$, satisfies:
  \begin{equation*}
    \label{eqn:fItColBnd}
     \norm{\Ct[T + 1]_i} \leq 2\mu\sqrt{\frac{r}{n}}\frac{65}{64} \sigma^*_1 + \frac{\epsilon}{20n} \leq 4\mu\sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  The first assumption of Lemma \ref{lem:incohCont} is trivially satisfied as the inner summation is an empty sum. The second assumption also holds simply because of the bound on the length of each column from equation \ref{eqn:fItColBnd}.

  We can thus apply Lemma \ref{lem:incohCont} at the end of the first inner iteration.

  We will now use induction on $k$ and $q$, to prove the theorem. When using induction over $q$, we will assume that the conditions of Lemma \ref{lem:inItProg} hold at the beginning of each inner iteration $q$. Note that conditions 2 and 3 of Lemma \ref{lem:inItProg} hold throughout an inner iteration if they hold at the beginning. By applying Lemma \ref{lem:inItProg} inductively, we arrive at the following condition which holds at the end of the $(T + 1)^{th}$ inner iteration:

  \[
    \norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp(\frac{\epsilon}{20n} + \sigma^*_{k + 1})
  \]

  Now, we will prove the correctness of the algorithm under two cases: \\
  \textit{Case 1: The Algorithm Breaks} In this case, we have that $\sigma^*_{k + 1} \leq \frac{\epsilon}{2n}$. Also, given our assumption on $\epsilon$, we have eliminated all the corrupted columns as the length of a corrupted column is bounded by $24\mu\sqrt{\frac{r}{n}}\lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}}$. Now, the matrix that is returned is indeed $\Lo$ as we do not eliminate a column $i\ i\in \supp{\Lo}$.
  \\
  \textit{Case 2: The Algorithm Continues to the Next Iteration} In this case, we have $\frac{\epsilon}{2n} \leq \sigma_{k + 1}(\Mt[T + 1]) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}$. We prove the correctness of the theorem in two subcases:
  \\
  \textit{Sub Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[T + 1])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^{T}\sigma^*_k + \sigma^*_{k + 1}} \leq \frac{1}{32}\lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}}$. Also, with this in hand, we have $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. Note that, assumption 1 of Lemma \ref{lem:incohCont} holds via the inductive hypothesis. For the second assumption, note that $\norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}} \leq 48\mu\sqrt{\frac{r}{n}}$.
  \\
  \textit{Case 2: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$. From this we know that, similarly to the previous subcase, $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. The rest of the proof proceeds similarly to the previous subcase.

  By the induction, hypothesis and noting the fact that the algorithm will always terminate in at most $r$ outer iterations, we have the correctness of the theorem.
\end{proof}


==> ArXiv/analysisAux.tex <==
%!TEX root = main.tex
\section{Analysis - Auxilliary Algorithm}
\label{sec:analysisAux}

In this section, we will give some bounds explaining when the algorithm introduced in the previous section will work. For our analysis, we assume that the givem matrix $M$ can be decomposed as the sum of three matrices $\Lo$, $\Co$ and $\No$ where $\Lo$ and $\Co$ satisfy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. In addition to these, we require the following assumptions on $\No$ and $\Co$ to guarantee the success of Algorithm \ref{alg:aux}:

\begin{assumption}
  \label{as:nNorm}
  \textbf{Norm of $\No$: } The frobenius norm of the noise matrix $\No$ is bounded by a small constant times $\sigma^*_r$, i.e, $\frob{\No} \leq c \sigma^*_r$ for a small enough constant $c$.
\end{assumption}

\begin{assumption}
  \label{as:incResC}
  \textbf{Incoherence and Residual of $\Co$: } We require the following conditions on $\Co$:
  \begin{enumerate}
    \item $\infnorm{\Pr{U^*}^\perp \Co} \leq 60\mu\sqrt{\frac{r}{n}} \sigma^*_r$
    \item $\infnorm{\sum\limits_{i = 1}^{r} \frac{u_i^*(u_i^*)^\top \Co}{\sigma^*_i}} \leq 20\mu \sqrt{\frac{r}{n}}$
  \end{enumerate}
\end{assumption}

Assumption \ref{as:nNorm} is a bound on the amount of noise that we can tolerate while Assumption \ref{as:incResC} can be guaranteed by an initial run of Algorithm \ref{alg:ncpca} upto $k = r - 1$.

We will now prove a lemma which states that the removal of a small number of columns from an incoherent matrix preserves the incoherence and the singular values of the matrix.

\begin{lemma}
  \label{lem:clIncRem}
  Let $A \in \mathbb{R}^{m\times n}$ be a $\mu$-incoherent, rank-$r$ matrix. Let $S \subseteq [n]$ such that $\abs{S} \leq \alpha n$ with $\alpha \leq \frac{c}{\mu^2r}$ be used to index a subset of columns of $A$. Let $A^\prime$ be defined as follows:
  \begin{equation*}
    A^\prime_{:, i} =
    \begin{cases}
      & A_{:, i},\ i \not\in S \\
      & 0, \text{ otherwise}
    \end{cases}
  \end{equation*}

  In other words, $A^\prime$ is the matrix obtained by setting the columns corresponding to the indices in $S$ to $0$. Let the $A = USV^\top$ and $A^\prime = U^\prime S^\prime (V^\prime)^\top$ denote the singular value decompositions of $A$ and $A^\prime$ respectively. We have for all $S$ satisfying the contraints with small enough constant $c$, the following bound on the incoherence of $A^\prime$:

  \begin{equation*}
    \norm{e_i^\top V^\prime} \leq \frac{65}{64} \mu \sqrt{\frac{r}{n}}, \qquad A = U^\prime S^\prime V^{\prime\prime} \text{ with } \norm{e_i^\top V^{\prime\prime}} \leq \frac{65}{64} \mu \sqrt{\frac{r}{n}}, \qquad \frac{63}{64} \sigma_i(A) \leq \sigma_i(A^\prime) \leq \sigma_i(A)
  \end{equation*}
\end{lemma}

\begin{proof}
  It is easy to see that $V^\prime$ is a full rank matrix for small enough $c$. Now, since $V^\prime$ forms the basis of the right singular vectors of $A^\prime$, there exists a matrix $R \in \mathbb{m\times n}$ such that $(V - \Pr{S}(V)) R = V^\prime$. From our condition on $S$, we know that for any vector $x \in \{y \in \mathbb{R}^r:  \norm{y} = 1\}$, $\norm{(V - \Pr{S}(V))x}$ can be bounded as follows:
  \begin{equation*}
    1 - c \leq \norm{Vx} - \norm{\Pr{S}(V)x} \leq \norm{(V - \Pr{S}(V)) x} \leq 1
  \end{equation*}
  From this, we get that for any vector $w$ such that $\norm{w} = 1$, we have:
  \begin{equation*}
    (1 - c) \norm{Rw} \leq 1 \leq \norm{Rw}
  \end{equation*}
  This means that all the singular values of $R$ are between $1$ and $\frac{1}{1-c}$ where $c$ can be arbitrarily small. From the fact that $(V - \Pr{S}(V))R = V^\prime$, we have the first claim of the lemma.

  For the second claim of the lemmma, note that $U^\prime S^\prime (V^\prime)^\top = US(V - \Pr{S} (V))^\top$. Along with the fact that $(V - \Pr{S}(V))R = V^\prime$ and noting that $(V - \Pr{S}(V))$ is a full rank matrix, we get that $U^\prime S^\prime R^\top = US$. This means that we can write the matrix $A$ as $A = U^\prime S^\prime R^\top V^\top $. The second claim of the lemma follows from the incoherence of $V$ and the bound on singular values of $R$.

  For the final claim of the lemma, we note that the singular values of $A^\prime$ are the singular values of $USR^{-1}$. We will first prove the upper bound in the lemma. We know that $\sigma_i (A^\prime) = \min\limits_{W \in \mathbb{R}^{m \times i - 1}, W^\top W = I} \norm{(I - WW^\top) A^\prime}$. From this identity, the upper bound can be obtained by setting $W$ to $U_{:, 1:i - 1}$ and noting that the singular values of $R^{-1}$ are between $1 - c$ and $1$. For the lower bound, consider any $W$ which forms the basis of an $(i - 1)$-dimensional subspace. Now, there exists $v \in span(U_{:, 1:i}) : v^\top W = 0 \text{ and } \norm{v} = 1$. For this $v$, we have that $(1-c)\sigma_i(A) \leq v^\top USR^{-1}$. Since, such a $v$ exists for all choices of $W$, the lower bound is proved.
\end{proof}

We will denote the columns of $\Lo$, $\Co$ and $\No$ in the support of $\Mt{t}$ by $\Lot{t}$, $\Cot{t}$ and $\Not{t}$ respectively. An important quantity required for our proof to go through is the projection of $\Cot{t}$ orthogonal to the row space of $\Lo$, i.e $\frob{\Pr{U^*}^\perp (\Cot{t})}$. We will show progress in the estimation of the subspace depends on $\frob{\Pr{U^*}^\perp (\Cot{t})}$. Specifically, we show how the quantity $\frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}$ depends on $\frob{\Pr{U^*}^\perp (\Cot{t})}$

\begin{lemma}
  \label{lem:auxLProg}
  Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC}, and $\No$ satisfies \ref{as:nNorm}. In the $t^{th}$ iteration of the algorithm:
  \begin{equation*}
    \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \leq 4\frob{\No} + 2\frob{\Pr{U^*}^\perp (\Cot{t})}
  \end{equation*}
\end{lemma}

\begin{proof}
  We prove the lemma as follows:
  \begin{align*}
    & \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \overset{(\zeta_1)}{\leq} \frob{(I - U^{(t)}(U^{(t)})^\top) (\Lo - \Lot{t})} + \frob{(I - U^{(t)}(U^{(t)})^\top) \Lot{t}} \\
    & \leq (1 + \frac{1}{32}) \frob{(I - U^{(t)}(U^{(t)})^\top) \Lot{t}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^{(t)}(U^{(t)})^\top) \lprp{\Lot{t} + \Not{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    % & \leq \frac{33}{32} \lprp{\sigma_{r + 1}(\Lot{t} + \Not{t} + \Cot{t}) + \frob{\No}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^{(t)}(U^{(t)})^\top) \lprp{\Lot{t} + \Not{t} + \Cot{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^*(U^*)^\top) \lprp{\Lot{t} + \Not{t} + \Cot{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    & \overset{(\zeta_2)}{\leq} \frac{33}{32} \lprp{2\frob{\No} + \frob{\Pr{U^*}^\perp (\Not{t} + \Cot{t})}} \\
    & \leq \frac{33}{32} \lprp{3\frob{\No} + \frob{\Pr{U^*}^\perp (\Cot{t})}} \\
    & \leq 4\frob{\No} + 2\frob{\Pr{U^*}^\perp (\Cot{t})}
  \end{align*}
  where $(\zeta_1)$ follows from Lemma \ref{lem:clIncRem} and the column sparsity of $\Lo - \Lot{t}$ and $(\zeta_2)$ follows from Weyl's inequality and the fact that $\supp{\Cot{t}} \cap \supp{\Lot{t} + \Not{t}} = \phi$.
\end{proof}

In the next lemma, we show how the quantity $\frob{\Pr{U^*}^\perp (\Cot{t + 1})}$ depends on the improved estimation of $U^*$.

\begin{lemma}
  \label{lem:auxCProg}
  Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC}, and $\No$ satisfies \ref{as:nNorm}. In the $t^{th}$ iteration of the algorithm:
  \begin{equation*}
    \frob{\Pr{U^*}^\perp (\Cot{t + 1})} \leq 3 \frob{\No} + \frac{1}{20} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}
  \end{equation*}
\end{lemma}
\begin{proof}
  To prove the lemma, we bound quantity $\norm{\Pr{U^*}^\perp ((\Cot{t + 1})_{:, i})}$ for each column $i$. For a column $i \in \supp{\Co}$, we consider two cases: \\
  \textit{Case 1: Column $i$ is thresholded} \\
  In this case, we have directly $\norm{\Pr{U^*}^\perp ((\Cot{t + 1})_{:, i})} = 0$. \\
  \textit{Case 2: Column $i$ is not thresholded} \\
  If $i$ is not thresholded, there exists a column $j_i \in \supp{\Lo + \No}$ such that $\norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}} \leq \norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, i} + \Co_{:, i})}$ (Note that this can be done with a different index $j_i$ for each column $i$ that is not thresholded). We first begin by providing a lower bound on $\norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}}$. We do this as follows:
  \begin{multline*}
     \norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}} = \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}(\Co_{:, i}) + \Pr{U^*}^\perp(\Co_{:, i}))} \\ \geq \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}^\perp(\Co_{:, i})} - \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}(\Co_{:, i})} \\ \overset{(\zeta_1)}{\geq} \frac{31}{32} \norm{\Pr{U^*}^\perp (\Co_{:, i})} - 20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}
  \end{multline*}
  Here, $(\zeta_1)$ follows from a bound on $\Pr{U^{(t)}}^\perp \Pr{U^*}^\perp$ obtained via the Davis Kahan along with Assumptions \ref{as:nNorm} and \ref{as:incResC} for the first term and from using Assumption \ref{as:incResC} for the second term.

  We can now prove a bound on $\frob{\Pr{U^*}^\perp (\Cot{t + 1})}$:
  \begin{align*}
    & \frob{\Pr{U^*}^\perp (\Cot{t + 1})} \\
    & \leq \frac{33}{32} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \lprp{\norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, j_i} + \No_{:, j_i})} + 20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^2}^\frac{1}{2} \\
    & \leq \frac{33}{32} \sqrt{2} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \lprp{\norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, j_i} + \No_{:, j_i})}}^2 + \lprp{20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^2}^{\frac{1}{2}} \\
    & \leq \frac{33}{16} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2 + \norm{(I - U^{(t)}(U^{(t)})^\top) \No_{:, j_i}}^2}^\frac{1}{2} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \begin{aligned}
     & \leq \frac{33}{16} \lprp{\lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2}^\frac{1}{2} + \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \No_{:, j_i}}^2}^\frac{1}{2}} + \\
     & \qquad \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
     \end{aligned} \\
    & \leq \frac{33}{16} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2}^\frac{1}{2} + 3 \frob{\No} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \leq \frac{33}{16} \lprp{\mu^2\frac{r}{n}\sum\limits_{i \in \supp{\Cot{t + 1}}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^\frac{1}{2} + 3 \frob{\No} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \leq \frac{1}{20}  \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} + 3 \frob{\No}
  \end{align*}
\end{proof}

We are now ready to prove a theorem which guarantees the correctness of our algorithm under the assumptions stated. Recall that the true sparsity of $\Co$ is denoted by $\alpha$.

\begin{theorem}
  \label{thm:aux}
  Let $\Mo = \Lo + \Co + \No$ be given such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC} and $\No$ satisfies Assumption \ref{as:nNorm}. Then, Algorithm \ref{alg:aux} run with $\alpha^\prime = \alpha$. returns a matrix $\Mt[T + 1]$ which satisfies:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 20 \frob{\No} + \frac{\epsilon}{n^2}
  \end{equation*}
  where $U^{(T + 1)}$ denotes the top-$r$ left singular vectors of $\Mt[T + 1]$.
\end{theorem}

\begin{proof}
  Note that the first singular value of $\Mo$ is at least $\frac{31}{32} \sigma^*_1$ from using Weyl's inequality along with our assumptions on $\No$ and $\Co$. In addition, we also have:
  \begin{multline*}
    \frob{(I - U^{(0)}(U^{(0)})^\top) \Lo} \leq \frob{(I - U^{(0)}(U^{(0)})^\top) (\Lo + \No)} + \frob{\No} \overset{(\zeta_1)}{\leq} \frob{\No} + \frob{(I - U^{(0)}(U^{(0)})^\top) (\Lo + \No + \Co)} \\
    \overset{(\zeta_2)}{\leq} 2\frob{\No} + \frob{\Pr{U^*}^\perp \Co} \leq \frac{1}{8} \sigma^*_r
  \end{multline*}
  where $(\zeta_1)$ follows from the fact that $\supp{\Lo + \No} \cap \supp{\Co} = \phi$ and $(\zeta_2)$ follows from the fact that $U^{(0)}$ are the top-$r$ left singular vectors of $\Lo + \Co + \No$.

  Now, from Lemmas \ref{lem:auxLProg} and \ref{lem:auxCProg}, we get the following recursion:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 4\frob{\No} + 2 \frob{\Pr{U^*}^\perp (\Cot{T + 1})} \leq 10\frob{\No} + \frac{1}{20} \frob{(I - U^{(T)}(U^{(T)})^\top) \Lo}
  \end{equation*}
  By applying the recursion $T + 1$ times, we get:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 20\frob{\No} + \lprp{\frac{1}{20}}^{T + 1} \frob{(I - U^{(0)}(U^{(0)})^\top) \Lo} \leq 20\frob{\No} + \frac{\epsilon}{n^2}
  \end{equation*}
  where the last inequality follows from our bound on $\frob{(I - U^{(0)}(U^{(0)})^\top) \Lo}$ and out definition of $T$.
\end{proof}


==> ArXiv/analysisCl.tex <==
%!TEX root = rpca.tex

%\subsection{Result}
%\label{sec:resGen}
%The following theorem illustrates the theoretical guarantees obtained by Algorithm \ref{alg:ncpcacl}:
%\begin{theorem}[Noise-less Setting]
%	\label{thm:thmCln}
%	Let $\Mo$ be the given corrupted data matrix, i.e., $\Mo=D^*+\Co$ where $D^*=[x_1, \dots, x_n]\in \R^{d\times n}$ contains the clean data points and the corruption matrix $\Co$ has at most $\alpha\cdot n$ non-zero columns. Furthermore, let $D^*$ be rank-$r$ and $\mu$-incoherent matrix, i.e., it satisfies Assumption\ref{as:rank}. Then, for all $\alpha\leq \frac{1}{\mu^2 r}$, Algorithm~\ref{alg:ncpcacl} when run with parameter $\nThresh = \frac{1}{64\mu^2 r}$ for $T=\log \frac{10\|M\|_2\cdot n}{\epsilon}$ iterations, returns a subspace $U$ such that,  %	Let $\Mo = \Lo + \Co$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{64\mu^2 r}$, returns a subspace $U$ such that:
%	\begin{equation*}
%		\frob{(I - UU^\top) D^*} \leq \epsilon.
%	\end{equation*}
%\end{theorem}
%Remarks: subspace distance, run-time complexity (near optimal and contrast to existing results), bring down factor of $r$ furthermore using binary search, value of $\rho$, incoherence-standard assumption. 
%
%\subsection{Analysis}
\label{sec:anCl}
In this section, we present the proof of Theorem~\ref{thm:thmCln}.
Recall that we are given $\Mo = \Do + \Co$, where $\Do=\Lo$ is a rank-$r$, $\mu$-incoherent matrix and $\Co$ has at most a fraction of $\rho$ non-zero columns. We can assume with out loss of generality that $\Do$ and $\Co$ have disjoint column supports as we can rewrite $\Mo_i$, for $i\in \supp{\Co}$, as $\Mo_i = \Do_i+\Co_i=0+(\Co_i+\Do_i)$ thus absorbing $\Do_i$ in $\Co_i$ itself. 

Our proof consists of three main steps. Given any set of columns $S$ and letting $[U_{\setminus S},\Sigma_{\setminus S}, V_{\setminus S}]$ be the top-$r$ SVD of $\Mo_{\setminus S}$, we establish the following:
\begin{enumerate}[leftmargin=*,labelindent=\labelwidth+\labelsep]% , labelindent=0pt, labelwidth=!]
	\item[\textbf{Step 1:}] Every non-zero column of $\Do$ has significantly smaller residual when projected onto subspace orthogonal to $U_{\setminus S}$ than the norm of corrupted columns of $\Mo_{\setminus S}$ (Lemma~\ref{lem:clResCl}), so its likelihood of being thresholded (Line 6, 8 of Algorithm~\ref{alg:ncpcacl}) is small, 
	\item[\textbf{Step 2:}] Every non-zero column of $\Do$ has small incoherence with respect to $[U_{\setminus S},\Sigma_{\setminus S}, V_{\setminus S}]$ (Lemma~\ref{lem:clExpCl}), i.e., its projection onto $U_{\setminus S}$ cannot be ``too large''. Hence, its likelihood of being thresholded (Line 7,8 of Algorithm~\ref{alg:ncpcacl}) is also small, 
	\item[\textbf{Step 3:}] Any non-zero column of $\Co$ which has small residual and incoherence compared to those of a non-zero column of $\Do$ and hence won't be thresholded by Algorithm~\ref{alg:ncpcacl}, has small residual when projected onto $\Uo$ . That is, the column itself is close to subspace spanned by $\Uo$ and hence does not effect estimation of $\Uo$ (Proof of Theorem~\ref{thm:thmCln}).
\end{enumerate}
That is, either a corrupted column will be thresholded or it is close to $\Uo$ while inliers ($\Do$) have little likelihood of being thresholded (step 1,2 above).
%Since in each iteration, Algorithm~\ref{alg:ncpcacl} removes all columns which have large residual or incoherence, any remaining outliers should fall under Step 3 above, and the top singular subspace of this thresholded matrix should be much closer to the true subspace $\Uo$. 
We now present the formal statements and their proofs. We start with two lemmata establishing Steps 1,2 above. Detailed proofs of the lemmata are given in Appendix~\ref{sec:pfclResCl} and \ref{sec:pfclExpCl}, respectively. 

\begin{lemma}
	\label{lem:clResCl}
%	Let $\Mo = \Lo + \Co$ where $\Lo$ and $\Co$ satisfy Assumptions \ref{as:rank} and \ref{as:colSup} respectively.
Consider the setting of Theorem~\ref{thm:thmCln}.
Let $S \subset [n]$ denote a subset of columns of $\Mo$ such that $\abs{S} \leq 2 \nThresh n$. Let $\MoS$ ($\LoS$) be obtained from $\Mo$ ($\Lo$) by setting the columns corresponding to indices specified in $S$ to $0$. Let $\US \SigS (\VS)^\top$ ($\UoS \SigoS (\VoS)^\top$) be the rank-$r\ \mathcal{SVD}$ of $\MoS$ ($\LoS$), then $\forall i$:
	\begin{equation*}
		\norm{(I - \US (\US)^\top) \Lo_{i}} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}} \norm{(I - \Uo {(\Uo)}^\top) \MoS}
	\end{equation*}
\end{lemma}
\begin{lemma}
	\label{lem:clExpCl}
%	Let $\Mo = \Lo + \Co$ where $\Lo$ and $\Co$ satisfy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Let $S \subset [n]$ denote a subset of columns of $\Mo$ such that $\abs{S} \leq 2 \nThresh n$. Let $M_S$ ($L_S$) be obtained from $\Mo$ ($\Lo$) by setting the columns corresponding to indices specified in $S$ to $0$. Let $U_S \Sigma_S (V_S)^\top$ ($U^*_S \Sigma^*_S (V^*_S)^\top$) be the rank-$r\ \mathcal{SVD}$ of $M_S$ ($L_S$), then $\forall i$:
Under the setting of Lemma~\ref{lem:clResCl}, we have for every $i$:
	\begin{equation*}
	\norm{\SigS^{-1} \US^\top \Lo_{i}} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}}.
	\end{equation*}
\end{lemma}

We now present the proof of Theorem \ref{thm:thmCln} where we illustrate Step 3:
\begin{proof}
	We will start by showing the quantity $\frob{(I - U^*(U^*)^\top) \Mt[t+1]}$ decreases at a geometric rate, where $\Mt[t+1]=\Mo-\Cot{t+1}$. Let $\Qt{t}$ denote the columns of $\Co$ that are not thresholded in iteration $t$. Also let $\St{t}$ denote the columns of $\Lo$ that are thresholded in iteration $t$. Let $\Ltt[t+1] \coloneqq \Lo_{\setminus \St{t}}$, $\Ctt[t+1] \coloneqq \Co_{\Qt{t}}$, and $P_{\perp}^{\U}(M)=(I-\U(\U)^\top)M$. Then, we have:
	\begin{align}
		&\frob{P_{\perp}^{\Uo}(\Mt[t+1])}^2  = \frob{P_{\perp}^{\Uo}(\Ltt[t+1] + \Ctt[t+1])} ^2 = \frob{P_{\perp}^{\Uo}(\Ctt[t+1])}^2 \notag\\&= \sum\limits_{j \in \Qt{t}} \norm{ \pperpuo(\Uot{t} \Sigot{t} W^{(t )}_j + R^{(t )}_j)}^2 
		 \leq 2 \sum\limits_{j \in \Qt{t}} \norm{\pperpuo(\Uot{t}) \Sigot{t}W^{(t)}_j}^2 + \norm{R^{(t)}_j}^2,\label{eq:cl1}
	\end{align}
	where $W^{(t)}_j=(\Sigot{t})^{-1}(\Uot{t})^T\Co_j$ and $R^{(t)}_j=\pperput(\Co_j)$, $\forall j\in \Qt{t}$. %	for some $v^{t - 1, j}$ and $r^{t - 1, j}$ for all $j \in \St{t - 1}$. 
	The last inequality follows from triangle inequality and the fact that $(a + b)^2 \leq 2(a^2 + b^2)$. %We will now show the existence of a good choice of $v^{t - 1, j}$ and $r^{t - 1, j}$. 

	Recall, that we threshold a particular column $l$ in iteration $t$ based on $\norm{\pperput(\Mo_{l})}$ and $\norm{(\Sigot{t})^{-1} (\Uot{t})^\top \Mo_{l}}$. For a particular $j \in \St{t}$ that wasn't thresholded in iteration $t$, we know that there exists a column $i_j$ such that $\norm{(\Sigot{t})^{-1} (\Uot{t})^\top \Lo_{i_j}} \geq \norm{(\Sigot{t})^{-1} (\Uot{t})^\top \Co_{j}}$. Similarly, there exists a column $k_j$ such that $\norm{\pperput(\Lo_{k_j})} \geq \norm{\pperput( \Co_{j})}$. From Lemmas \ref{lem:clExpCl} and \ref{lem:clResCl}, we have:
	\begin{equation}\label{eq:cl2}
		\norm{W^{(t)}_j} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}} \qquad \norm{R^{(t)}_j} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}} \norm{\pperpuo(\Mt[t])}
	\end{equation}
	Using \eqref{eq:cl1} and \eqref{eq:cl2}, we have: 
	\begin{multline*}
		\frob{P_{\perp}^{\Uo}(\Mt[t+1])}^2\leq 2 \sum\limits_{j \in \St{t}} \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{\pperpuo(\Uot{t})\Sigot{t}}^2 + \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{\pperpuo(\Mt[t])}^2\\ 
		\leq 4 \cdot \frac{9}{8} \cdot \frac{\mu^2 r}{n}\cdot \rho n \cdot \|\pperpuo(\Mt[t])\|^2\leq \frac{1}{4} \norm{\pperpuo(\Mt[t])}^2, 
	\end{multline*}
	where second last inequality follows from $|\St{t}|\leq \rho n$ and the last inequality follows from $\rho\leq \alpha \leq \frac{1}{128 \mu^2 r}$. 
	By recursively applying the above inequality, we obtain:
	\begin{equation}\label{eq:cl3}
		\frob{\pperpuo( \Mt[T + 1])} \leq \frac{\epsilon}{20n}.
	\end{equation}
Also, note that using variational characterization of SVD, we have $\|\pperpu(\Mt[T+1])\|_F\leq \frob{\pperpuo( \Mt[T + 1])}$. Theorem now follows from the following argument: 
	\begin{multline*}
		\frob{\pperpu(\Lo)}^2 = \frob{\pperpu(\Ltt[T + 1])}^2 + \sum\limits_{i \in \St{T}} \norm{\pperpu(\Lo_{i})}^2
		\leq \frob{\pperpu(\Mt[T + 1])}^2 + \sum\limits_{i \in \St{T}} \frac{33^2}{32^2} \mu^2 \frac{r}{n} \norm{\pperpu(\Ltt[T + 1])}^2\\
		\leq \frob{\pperpu(\Mt[T + 1])}^2 + 2\nThresh n \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \frob{\pperpu(\Mt[T + 1])}^2\leq \frac{\epsilon}{10n},
	\end{multline*}
	where the first inequality follows from Lemma~\ref{lem:incPres} and using $\Mt[T+1]=\Ltt[T+1]+\Ctt[T+1]$, and the fact that $\Ltt[T+1]$ and $\Ctt[T+1]$ have different support. The second inequality follows from the fact that at most $2 \rho\cdot n$ points can be thresholded and then using \eqref{eq:cl3}. 
\end{proof}



%
%\begin{proof}
%	We will start by showing the quantity $\frob{(I - U^*(U^*)^\top) \Mt[t+1]}$ decreases at a geometric rate, where $\Mt[t+1]=\Mo-\Cot{t+1}$. Let $\Qt{t}$ denote the columns of $\Co$ that are not thresholded in iteration $t$. Also let $\St{t}$ denote the columns of $\Lo$ that are thresholded in iteration $t$. Let $\Ltt[t] \coloneqq \Lo_{\setminus \St{t - 1}}$, $\Ctt[t] \coloneqq \Co_{\Qt{t - 1}}$, and $P_{\perp}^{\Uo}(M)=(I-\Uo(\Uo)^\top)M$. Then, we have:
%	\begin{align*}
%	\frob{P_{\perp}^{\Uo}(\Mt[t])}^2  &= \frob{P_{\perp}^{\Uo}(\Ltt[t] + \Ctt[t])} ^2 = \frob{P_{\perp}^{\Uo}(\Ctt[t])}^2 \leq \sum\limits_{j \in \Qt{t - 1}} \norm{ \pperpuo(\Uot{t - 1}) \Sigot{t - 1} v^{t - 1, j} + r^{t - 1, j}}^2 \\
%	& \leq 2 \sum\limits_{j \in \Qt{t - 1}} \norm{\pperpu(\Uot{t - 1}) \Sigot{t - 1}v^{t - 1, j}}^2 + \norm{r^{t - 1, j}}^2
%	\end{align*}
%	for some $v^{t - 1, j}$ and $r^{t - 1, j}$ for all $j \in \St{t - 1}$. The last inequality follows from triangle inequality and the fact that $(a + b)^2 \leq 2(a^2 + b^2)$. We will now show the existence of a good choice of $v^{t - 1, j}$ and $r^{t - 1, j}$. 
%	
%	Recall, that we threshold a particular column $l$ in iteration $t$ based on $\norm{(I - \Uot{t-1}(\Uot{t-1})^\top)\Mo_{l}}$ and $\norm{(\Sigot{t - 1})^{-1} (\Uot{t - 1})^\top \Mo_{l}}$. For a particular $j \in \St{t - 1}$ that wasn't thresholded in iteration $t - 1$, we know that there exists a column $i_j$ such that $\norm{(\Sigot{t - 1})^{-1} (\Uot{t - 1})^\top \Lo_{i_j}} \geq \norm{(\Sigot{t - 1})^{-1} (\Uot{t - 1})^\top \Co_{j}}$. Similarly, there exists a column $k_j$ such that $\norm{(I - \Uot{t-1}(\Uot{t-1})^\top) \Lo_{k_j}} \geq \norm{(I - \Uot{t-1}(\Uot{t-1})^\top) \Co_{j}}$. From Lemmas \ref{lem:clExpCl} and \ref{lem:clResCl}, we have:
%	\begin{equation*}
%	\norm{v^{t - 1, j}} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}} \qquad \norm{r^{t - 1, j}} \leq \frac{33}{32} \mu \sqrt{\frac{r}{n}} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}
%	\end{equation*}
%	
%	By substituting the above inequalities, we have:
%	
%	\begin{multline*}
%	\frob{(I - U^*(U^*)^\top) \Mt[t]} \leq \lprp{2 \sum\limits_{j \in \St{t - 1}} \norm{(I - U^*(U^*)^\top) \Uot{t - 1}\Sigot{t - 1}v^{t - 1, j}}^2 + \norm{r^{t - 1, j}}^2}^\frac{1}{2} \\ 
%	\leq \lprp{2 \sum\limits_{j \in \St{t - 1}} \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - U^*(U^*)^\top) \Uot{t - 1}\Sigot{t - 1}}^2 + \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2}^\frac{1}{2} \\
%	\leq \lprp{2 \sum\limits_{j \in \St{t - 1}} \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2 + \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2}^\frac{1}{2} \\ 
%	\leq \lprp{4 \sum\limits_{j \in \St{t - 1}} \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2}^\frac{1}{2} \leq 2 \lprp{\norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2 \frac{9}{8} \mu^2 \frac{r}{n} \nThresh n}^{\frac{1}{2}} \\ 
%	\leq 2 \lprp{\frac{\norm{(I - U^*(U^*)^\top) \Mt[t - 1]}^2}{16}}^{\frac{1}{2}} \leq \frac{1}{2} \norm{(I - U^*(U^*)^\top) \Mt[t - 1]}
%	\end{multline*}
%	
%	By recursively applying the above inequality, we obtain:
%	\begin{equation*}
%	\frob{(I - UU^\top) \Mt[T + 1]} \leq \frac{\epsilon}{20n}
%	\end{equation*}
%	
%	The theorem can now be proved as follows:
%	\begin{multline*}
%	\frob{(I - UU^\top) \Lo} = \lprp{\frob{(I - UU^\top) \Ltt[T + 1]}^2 + \sum\limits_{i \in \St{T}} \norm{(I - UU^\top) \Lo_{i}}^2}^{\frac{1}{2}} \\ 
%	\leq \lprp{\frob{(I - UU^\top) \Mt[T + 1]}^2 + \sum\limits_{i \in \St{T}} \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - UU^\top) \Ltt[T + 1]}^2}^{\frac{1}{2}} \\
%	\leq \lprp{\frob{(I - UU^\top) \Mt[T + 1]}^2 + 2\nThresh n \lprp{\frac{33}{32}}^2 \mu^2 \frac{r}{n} \norm{(I - UU^\top) \Mt[T + 1]}^2}^{\frac{1}{2}} \\ 
%	\leq \lprp{\lprp{1 + \frac{1}{16}} \frob{(I - UU^\top) \Mt[T + 1]}^2}^2 \leq \frac{5}{4} \frob{(I - UU^\top) \Mt[T + 1]} \leq \frac{\epsilon}{10n}
%	\end{multline*}
%\end{proof}

==> ArXiv/analysisG.tex <==
%!TEX root = rpca.tex

%\section{Analysis}
Our analysis of \ncpcag\ show that the algorithm maintains the following critical invariant with high probability: 
\begin{invariant}
  \label{inv:incMnt}
  We assume that the following hold with respect to the two thresholding steps used in Algorithm~\ref{alg:ncpcag}. 
  \begin{enumerate}[leftmargin=*,labelindent=\labelwidth+\labelsep]
  	\item With respect to $\zeta_1$: If a column $i \not\in \supp{\Co}$ is thresholded, then the following condition holds:
  	\begin{equation*}
  		\norm{\No_{i}} \geq \sigma \lprp{\sqrt{d} + 2d^{\frac{1}{4}} \sqrt{\log\lprp{\frac{\mu^2 r}{c_2}}}}.
  	\end{equation*}
    and consequently only $\frac{3nc_2}{2\mu^2 r}$ points are removed in this step.
  	\item With respect to $\zeta_2$: If a thresholding step occurs due to the second thresholding step with $\zeta_2$, then at least half the points thresholded in this step are corrupted points. 
  \end{enumerate}
\end{invariant}

%The next lemma proves we will show that Invariant~\ref{inv:incMnt} holds till the termination of the algorithm. 
\begin{lemma}
	\label{lem:invGau}
	Assume the conditions of Theorem~\ref{thm:thmG}. Then, Invariant \ref{inv:incMnt} holds at any point in the running of Algorithm \ref{alg:ncpcag} with probability at least $1-\delta$.
\end{lemma}
	See Appendix \ref{sec:pfInvGau} for a detailed proof. 

Our proof then uses the above invariant along with a careful analysis of each of the two thresholding steps (Line 10, 12) to obtain the desired result. See Appendix \ref{sec:pfThmGauss} for a detailed proof. 
%\begin{theorem}
%  \label{thm:thmGau}
%  Let $\Mo = \Lo + \No + \Co$ such that Assumptions~\ref{as:rank} and \ref{as:colSup} hold for $\Lo$ and $\Co$ respectively. Furthermore, suppose that each entry of $\No$ is generated iid according to $\mathcal{N} (0, \sigma^2)$. Then, the matrix $U$ satisfies:
%  \begin{equation*}
%    \norm{(I - U_{1:r}U_{1:r}^\top) \Lo} \leq 4 \sigma\sqrt{n \log(d)}
%  \end{equation*}
%  with probability at least $\delta$ as long as $n \geq \max \left\{\frac{16\mu^2rd}{c_1} \left[\log\lprp{\frac{1}{3\delta}} + d\log(40d)\right], \right. \\
%  \left. 200 \lprp{d + 2 \log \lprp{\frac{1}{2\delta}}}, \frac{16\mu^2 r}{c_2} \log \lprp{\frac{1}{3\delta}}\right\}$ for some $c_1 = \Omega(\frac{1}{r})$ and $c_2 = \Omega(1)$.
%\end{theorem}


==> ArXiv/analysisN.tex <==
%!TEX root = rpca.tex
\renewcommand{\u}{\bm{u}}
\section{Analysis - With Noise}
\label{sec:analysisN}

We will state the main theorem for the noisy case here:
\begin{theorem}
  \label{thm:masterN}
  Let $\Mo = \Lo + \Co + \No,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo,\ \Co \text{ and } \No$ satisfying Assumptions \ref{as:rank} , \ref{as:colSup} and \ref{as:nNorm} respectively. Then, there exists two matrices $\widetilde{L}$ and $\widetilde{C}$ such that $\widetilde{L} + \widetilde{C} = \Lo + \Co$, $\Pr{U^*}(\widetilde{L}) = \widetilde{L}$ and $\Pr{\supp{\Co}} (\widetilde{C}) = \widetilde{C}$ satisfying:
  \begin{equation*}
    \norm{\widetilde{L} - \widehat{L}} \leq \frac{\epsilon}{5\sqrt{n}} + 25 \frob{\No}, \qquad \norm{\widetilde{C} - \widehat{C}} \leq \frac{\epsilon}{5\sqrt{n}} + 25 \frob{\No}
  \end{equation*}
\end{theorem}

We can now prove the correctness of Algorithm \ref{alg:ncpcan}. In addition to Assumptions \ref{as:rank} and \ref{as:colSup} on $\Lo$ and $\Co$ respectively, we will also require Assumption \ref{as:nNorm} on the noise matrix $\No$. Throughout the lemmas that will follow, we will assume that only a small fraction of columns of $\Lo$ have been thresholded by the algorithm. Specifically, we will assume that only a $\frac{c}{\mu^2r}$ fraction of columns in the support of $\Lo$ have been thresholded. We will show that this will indeed happen when we prove the main theorem of this section.

% \begin{theorem}
%   \label{thm:master}
%   Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $L$ satisfying:
%   \begin{equation*}
%     \frob{L - \Lo} \leq \epsilon
%   \end{equation*}
% \end{theorem}

Similar to the proof for the non-noisy case, we track two important quantities:
\begin{equation}
  \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])},\ \itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}
\end{equation}

We well state an analogue to Lemma \ref{lem:inItProg} which will guarantee progress in an inner iteration of our algorithm. We will use $\Lot{q}$, $\Cot{q}$ and $\Not{q}$ to refer to the matrices $\Lo$, $\Co$ and $\No$ projected onto the column support of $\Mt[q]$. The last two claims of the lemma are used to show that the norm of $\No$ in a column in the support of $\Lo$ that has been thresholded is sufficiently high to ensure that not too many columns of $\Lo$ are thresholded.

\begin{lemma}
  \label{lem:inItProgN}
  Let $\Mo = \Lo + \Co + \No$ be a matrix such that $\Lo$, $\Co$ and $\No$ satisfy Assumptions \ref{as:rank}, \ref{as:colSup} and \ref{as:nNorm} respectively. Also, assume that the following conditions hold before the $q^{th}$ inner iteration:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{1,\ldots,k-1\}$
    \item $ \frac{\supp{\Lot{q}}}{n} \geq 1 - \frac{c}{\mu^2r} $ for a small enough constant $c$
  \end{enumerate}
  Then, after the $q^{th}$ inner iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{(I - U_kU_k^\top) \Lot{q}} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\zeta_q \geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  First, we note that $\sigma_{k}(\Mt[q]) \geq \frac{63}{64}\sigma^*_{k} - \norm{\No}$. We now decompose $\Mt{q}$ as $\Pr{U^*_{\sigma^*_k / 2}}(\Mt{q}) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Lo) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q]) + \Not{q}$. Let $U_k$ denote singular vectors corresponding to the top $k$ singular vales of $\Mt$. We will now bound $\norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k / 2}}}^\perp}$.

  By the Davis Kahan theorem, we get the following bound:
  \begin{equation}
    \label{eqn:projBound}
    \norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k} / 2}}^\perp} \leq \frac{\norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])} + \norm{\No}}{\sigma_k(\Mt{q}) - \sigma^*_{Pos^*(\sigma^*_{k} / 2) + 1}} \leq \frac{17\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])}}{8\sigma^*_k}
  \end{equation}

  We will now analyze a fixed column in the support of $\Lot{q}$. We fix $i$ such that $i \in \supp{\Lo}$.

  \begin{align}
    \label{eqn:clBound}
    \norm{(I - U_kU_k^\top) \Lo_i} &= \norm{(I - U_kU_k^\top) (\Lot{q} + \Pr{U^*}(\Ct[q])) e_i} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{(I - U_kU_k^\top) (\Lot{q} + \Pr{U^*}(\Ct[q]))} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - U_kU_k^\top)\Mt[q]} + \norm{\No} + \norm{\Pr{U^*}^\perp(\Ct[q])}} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1} (\Mt) + \norm{\Pr{U^*}^\perp(\Ct[q])} + \norm{\No}}
  \end{align}

  We will now bound the quantity $\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])e_i},\ \forall i \in \{1,\ldots,n\}$. For a thresholded column, the quantity is bounded by $0$. For a column that is not thresholded, we have:
  \begin{align*}
    \eta \geq \norm{(I - U_kU_k^\top)\Ct[q + 1]e_i} &= \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i) + \Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i))} \\
    &\geq \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)U^*\Sigma^*v} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)\Lot{q}} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Lot{q} + \Pr{U^*_{\sigma^*_k/2}}(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Mt - \Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q]) - \Not{q})} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}} \right)
  \end{align*}

  From this, we get:
  \begin{equation}
    \label{eqn:corBound}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} \leq \frac{32}{31} \lprp{\zeta + \frac{33}{2}\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}} \right)}
  \end{equation}

  With these inequalities in hand, we can proceed to bound the value of $\sigma_{k + 1}(\Mt)$. Using Weyl's inequality, we know that $\sigma_{k + 1}(\Mt) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct)} + \norm{\Not{q}}$. Here, we consider two cases:

  \textit{Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}}$.

  \textit{Case 2: } $\sigma^*_{k + 1} \geq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$.

  We now bound $\sigma_k(\Mt)$. Similar to Case 2 above, consider index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_k$. Again, we know that $\sigma_{k}(\Mt) \leq \sigma^*_{k} + \norm{\Pr{U^*_{k - 1}}^\perp (\Ct)}$. And we also have that $ 2\sigma^*_{k} \geq \sigma^*_{i + 1} $ and that $ (U^*_{k - 1})^\perp \subset (U^*_{\sigma^*_i / 2})^\perp $. From these two observations, we have $\sigma_k(\Mt) \leq \frac{33}{32} \sigma^*_k + \norm{\Not{q}}$.

  From \ref{eqn:clBound}, we have for $i \in \supp{\Lo}$:

  \begin{equation*}
    \norm{(I - U_kU_k^\top)L^*_i} \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma^*_{k + 1} + \frac{1}{16} \lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}} + \frac{\sigma^*_{k + 1}}{32} + 2\norm{\Not{q}}} \leq \frac{5}{4}\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{equation*}

  We can also prove a lower bound on $\zeta$ as follows:
  \begin{align*}
    &\zeta = 2\mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma_k(\Mt) + \sigma_{k + 1} (\Mt)} \\
    &\geq 2\mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma_k(\Lot{q}) + \sigma_{k + 1} (\Lot{q}) - 3\norm{\Not{q}}} \\
    &\geq \frac{31}{16} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}} \\
    &\geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  This proves the third claim of the lemma.

  Similarly, from \ref{eqn:corBound}, we have:
  \begin{align*}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} &\leq \frac{32}{31} \lprp{\zeta + \frac{33}{2}\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}}\right)} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{37}{2}\sigma_{k + 1} + 2\lprp{\frac{1}{2}}^{q + 1}\sigma_{k} + \frac{33}{2}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \frac{33}{2} \norm{\Not{q}}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \frac{37}{2}\sigma^*_{k + 1}} + 36 \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + 27 \norm{\Not{q}}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \frac{37}{2}\sigma^*_{k + 1}} + \frac{36}{32}\lprp{\lprp{\frac{1}{2}}^{q}\sigma^*_k + \sigma^*_{k + 1}} + 27 \norm{\Not{q}}} \\
    &\leq 24 \mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  With the two inequalities defined above, we have proved the lemma.
\end{proof}

In the following lemma, we will prove that the thresholding steps at the end of the outer loop establishes control on the quantity, $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}$.

\begin{lemma}
  \label{lem:incohContN}
  Let $\Mo = \Lo + \Co + \No$ be a matrix such that $\Lo$, $\Co$ and $\No$ satisfy Assumptions \ref{as:rank}, \ref{as:colSup} and \ref{as:nNorm} respectively. Also, assume that the following conditions hold after the inner iteration in the $k^{th}$ outer iteration concludes:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[T + 1])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{0,\ldots,k\}$
  \end{enumerate}
  Then, after the $k^{th}$ outer iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k + 1} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{US^{-1}U^\top \Lo} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}}$
    \item $\norm{US^{-1}U^\top} \leq \frac{31}{32\sigma^*_{k + 1}}$
    \item $\itnorm{(I - UU^\top) \Lo} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}$
    \item $\zeta \geq \frac{3}{2} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}$
  \end{enumerate}
\end{lemma}

% TODO: Finish Lemma
\begin{proof}
  Similarly to the previous lemma, we bound $ \sigma_{k + 1}(\Mt[T + 1]) $ by $ \lprp{\sigma^*_{k + 1}(\Mt[T + 1]) + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} + \Not{T + 1}}$. Now consider the index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. From our assumptions, we know that $\sigma^*_{i + 1} \leq 2\sigma^*_{k + 1}$. Also, we know that $(U^*_{k})^\perp \subset (U^*_{\sigma^*_{i} / 2})^\perp$. This implies that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \frac{1}{32} \sigma^*_{k + 1}$ by our assumptions on $\alpha$ and by using Lemma \ref{lem:spNrm}.

  We first prove the fourth claim of the lemma:

  For the thresholding with respect to $\zeta$, we have:
  \begin{align*}
    \norm{(I - UU^\top) \Lo_i} &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}}\norm{(I - UU^\top) \Lot{T + 1}} \\
    &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{(I - UU^\top) (\Lot{T + 1} + \Pr{\sigma^*_{k} / 2} (\Ct[T + 1]))} \\
    &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - UU^\top) \Mt[T + 1]} + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])} + \norm{\Not{T + 1}}} \\
    &\overset{(\zeta_1)}{\leq} \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Mt[T + 1]) + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])} + \norm{\Not{T + 1}}} \\
    &\leq \frac{35}{32}\mu\sqrt{\frac{r}{n}} \sigma^*_{k + 1} \\
    &\leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}
  \end{align*}

  where the $(\zeta_1)$ holds from Lemma \ref{lem:spNrm} and our assumptions on $\alpha$, $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])}$ and $\norm{\Not{T + 1}}$.

  This proves the fourth claim of the lemma. We will now prove the fifth claim of the lemma.
  \begin{equation*}
    \zeta = 4 \mu \sqrt{\frac{r}{n}} \sigma_{k + 1}(\Mt[T + 1]) \geq 4 \mu \sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Lot{T + 1}) - \norm{\Not{T + 1}}} \geq 4\mu \sqrt{\frac{r}{n}} \lprp{\frac{63}{64}\sigma^*_{k + 1} - \norm{\Not{T + 1}}} \geq \frac{3}{2} \mu\sqrt{\frac{r}{n}} \sigma^*_{k + 1}
  \end{equation*}

  The third claim of the lemma, can be proved with a lower bound on $\sigma_{k + 1}(\Mt[T + 1])$:
  \begin{equation*}
    \sigma_{k + 1}(\Mt[T + 1]) \geq \sigma_{k + 1}(\Lot{T + 1}) - \norm{\Not{T + 1}} \geq \frac{31}{32} \sigma^*_{k + 1}
  \end{equation*}
  This implies the third claim of the lemma.

  We will now prove the second claim of the lemma:
  \begin{align*}
    \norm{US^{-1}U^\top \Lo_i} &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top \Lot{T + 1}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top (\Lot{T + 1} + \Pr{U^*_{\sigma^*_{k} / 2}} (\Ct))} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{US^{-1}U^\top \Mt[T + 1]} + \norm{US^{-1}U^\top \Pr{U^*_{\sigma^*_{k} / 2}}^\perp (\Ct)} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{31}{32\sigma^*_{k + 1}} \norm{\Pr{U^*_{\sigma^*_{k}}}^\perp (\Ct)} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{31}{32\sigma^*_{k + 1}} \frac{\sigma^*_{k + 1}}{32} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{5}{4} \mu\sqrt{\frac{r}{n}}
  \end{align*}

  This concludes the proof of the second claim of the lemma. We will now prove the first claim of the lemma. We first note that a column $i \in \supp{\Ct[T + 1]}$ can be written as $USv + v_{res}$ such that $\norm{v} \leq 2\mu\sqrt{\frac{r}{n}}$ and $\norm{v_{res}} \leq \zeta$. We now prove claim 2 as follows:

  \begin{align*}
    &\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]_i}\\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top (USv + v_{res})} \\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top USv} +  \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top v_{res}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 4\mu\sqrt{\frac{r}{n}} \frac{2}{\sigma^*_{k + 1}} \sigma_{k + 1}(\Mt[T + 1]) \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 9 \mu\sqrt{\frac{r}{n}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{2\sigma_{k + 1}(\Mt[T + 1])}{\sigma^*_{k + 1}}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{33}{16}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \lprp{\Lot{T + 1} + \Ct[T + 1] + \Not{T + 1}}}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{1 + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]} + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Not{T + 1}}} \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\norm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \norm{\sum\limits_{i = Pos^*(\sigma^*_k / 2) + 1}^{Pos^*(\sigma^*_{k + 1} / 2)} \frac{u^*_i (u^*_i)^\top}{\sigma^*_i} \Ct[T + 1]} + \frac{2\norm{\No}}{\sigma^*_{k + 1}}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\sqrt{\alpha n} \itnorm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \frac{2\sqrt{\alpha n}}{\sigma^*_{k + 1} / 2} \itnorm{\Pr{U^*_{\sigma^*_{k} / 2}}^\perp \Ct[T + 1]} + \frac{1}{32}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu \sqrt{\frac{r}{n}} \lprp{\frac{1}{32} + \frac{1}{32} + \frac{1}{32}} \\
    &\leq 16\mu\sqrt{\frac{r}{n}}
  \end{align*}

  This establishes Claim 1 of the lemma.

\end{proof}

We can now prove the main theorem of the paper.

\begin{proof}
  \textit{Proof of Theorem \ref{thm:masterN}} \\
  We will prove the main theorem of the paper in three stages. In the first stage, we will analyze the first outer iteration of the algorithm. In the second, we will show that the conditions required for the application of theorem \ref{thm:aux}. In the final stage, we will show the correctness of the incoherence preserving projection operator. In the first and second stages of the algorith, we will assume that at most a small fraction ($\frac{c}{\mu^2r}$ for small enough $c$) of columns of $\Lo$ are thresholded during the running of the algorithm. We will show that this will be the case when at the end of stage 2.

  \textit{Stage 1:}\\
  First, we note that $\sigma_1 (\Mt[q]) \geq \frac{63}{64} \sigma^*_1 - \norm{\No} \geq \frac{31}{32} \sigma^*_1$ from Weyl's inequality and our upper bound on the number of columns of $\Lo$ thresholded. We now prove an upper bound on $\sigma_1(\Mt[T + 1])$ at the end of the first inner iteration.

  We have the following recurrence inequality for $\sigma_1(\Mt[q]) \ \forall q \geq 1$ from Weyl's inequality and our condition on $\alpha$.
  \begin{equation}
    \label{eqn:sig1Rec}
    \sigma_1(\Mt[q]) \leq \sigma_1^* + \norm{\Ct[q - 1]} \leq \sigma_1^* + \norm{\Not{q}} + \frac{1}{64} \sigma_1(\Mt[q - 1])
  \end{equation}

  By expanding on this recurrence and from our setting of $T$, we get:
  \begin{equation}
    \sigma_1(\Mt[T + 1]) \leq \sigma_1^* \sum\limits_{i = 0}^{T} \lprp{\frac{1}{64}}^i + 2\norm{\No} + \lprp{\frac{1}{64}}^T \sigma_1(\Mo) \leq \frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n}
  \end{equation}

  From our lower bounds on $\sigma_1(\Mt[q])$, we can see that the following inequalities hold:
  \begin{equation*}
    \itnorm{(I - U_1U_1^\top) \Lot{q}} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_1, \quad \zeta_q \geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  In the if condition at the end of the first inner iteration, we consider two cases: \\
  \textit{Case 1: The Algorithm Returns} In this case, we know that $\frac{31}{32}\sigma_1^* \leq \frac{\epsilon}{10n}$ which implies that $\sigma^*_1 \leq \frac{\epsilon}{12n}$. With this inequality, we return the empty matrix for $\widehat{L}$ and $\Mo$ as estimates of $\Lo$ and $\Co$ respectively. Given our bound on the singular values of $\Lo$ (and $\No$), the statement of the theorem follows.
  \\
  \textit{Case 2: The Algorithm Continues To the Next Iteration} In this case, we know that $\sigma_1^* \geq \frac{\epsilon}{12n}$. This follows from using the upper bound $\sigma_1(\Mt[T + 1]) \leq \sigma^*_1 + \norm{\No} + \norm{\Ct[T + 1]}$. We will now prove that the assumptions of Lemma 4 are satisfied at the end of the first inner iteration.

  We know that each column $i$, satisfies:
  \begin{equation*}
    \label{eqn:fItColBnd}
     \norm{\Ct[T + 1]_i} \leq 2\mu\sqrt{\frac{r}{n}} {\frac{65}{64} \sigma^*_1 + \frac{\epsilon}{20n}} \leq 4\mu\sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  The first assumption of Lemma \ref{lem:incohCont} is trivially satisfied as the inner summation is an empty sum. The second assumption also holds simply because of the bound on the length of each column from equation \ref{eqn:fItColBnd}.

  We can thus apply Lemma \ref{lem:incohCont} at the end of the first inner iteration.

  \textit{Stage 2:}\\
  We will now use induction on $k$ and $q$, to prove the theorem. When using induction over $q$, we will assume that the conditions of Lemma \ref{lem:inItProgN} hold at the beginning of each inner iteration $q$. Note that conditions 2 and 3 of Lemma \ref{lem:inItProgN} hold throughout an inner iteration if they hold at the beginning. Condition 4 holds by assumption. By applying Lemma \ref{lem:inItProgN} inductively, we arrive at the following condition which holds at the end of the $(T + 1)^{th}$ inner iteration:

  \[
    \norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp(\frac{\epsilon}{20n} + \sigma^*_{k + 1})
  \]

  Now, we will prove the correctness of the algorithm under two cases: \\
  \textit{Case 1: The Algorithm Returns} In this case, we have that $\sigma^*_{k + 1} \leq \frac{\epsilon}{10n}$. Here, we will prove the correctness of the incoherence preserving projection operator. To prove the theorem, we will need to construct a candidate pair $(\widetilde{L}, \widetilde{C})$ such that $\widetilde{L}$ has the same row space of $\Lo$ and $\widetilde{C}$ has the same column space of $\Co$.
  We will choose $\widetilde{L}$ to be $\Lo + \Pr{U^*} (\Co)$. We will bound $\frob{\widehat{L} - \widetilde{L}}$ by bounding $\frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)}$ and $\norm{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)}$.
  \begin{align*}
    & \frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} \\
    &\leq \frob{\No} + \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} \\
    & \leq \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} + \frob{\No} \\
    & \leq \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo)} + \frob{\No} \\
    & \leq \frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo)} + 2\frob{\No} \\
    & \leq \frac{65}{64} \frob{\Lot{T + 1} - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lot{T + 1})} + 2\frob{\No} \\
    & \overset{(\zeta_1)}{\leq} \frob{\Lot{T + 1} - U^\prime (U^\prime)^\top (\Lot{T + 1})} + 2\frob{\No} \\
    & \leq \frob{(I - U^\prime (U^\prime)^\top) (\Lot{T + 1} + \Pr{U^*} (\Cot{T + 1}))} + 2\frob{\No} \\
    & \leq \frob{(I - U^\prime (U^\prime)^\top) \Mt[T + 1]} + \frob{\Pr{U^*}^\perp (\Cot{T + 1})} + 2\frob{\No} \\
    & \leq \sqrt{n} \sigma_{k + 1} (\Mt[T + 1]) + \frob{\Pr{U^*}^\perp (\Cot{T + 1})} + 2\frob{\No} \\
    & \leq \sqrt{n} \sigma^*_{k + 1} + 2\frob{\Pr{U^*_{k}}^\perp (\Cot{T + 1})} + 3\frob{\No} \\
    & \leq \sqrt{n} \frac{\epsilon}{10n} + \frac{1}{32} (\frac{\epsilon}{20n} + \sigma^*_{k + 1}) + 3\frob{\No} \\
    & \leq \frac{\epsilon}{10\sqrt{n}} + 3\frob{\No}
  \end{align*}

  We will now bound the second term:
  \begin{align*}
    & \frob{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)} \\
    & \leq \sqrt{\alpha n} \itnorm{\norm{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)}} \\
    & \leq \frac{1}{32} \norm{\Pr{U^*}^\perp (US)} \\
    & \leq \frac{1}{32} \norm{\Pr{U^*}^\perp (\Pr{U}(\Mt[T + 1]) - \Mt[T + 1] + \Mt[T + 1])} \\
    & \leq \frac{1}{32} \lprp{\norm{\Pr{U^*}^\perp (\Mt[T + 1])} + \norm{\Pr{U}^\perp (\Mt[T + 1])}} \\
    & \leq \frac{1}{32} \lprp{\norm{\Pr{U^*}^\perp (\Lot{T + 1} + \Not{T + 1} + \Cot{T + 1})} + \frac{\epsilon}{20n}} \\
    & \leq \frac{1}{32} \lprp{\norm{\Not{T + 1}} + \norm{\Pr{U^*}^\perp(\Cot{T + 1})} + \frac{\epsilon}{20n}} \\
    & \leq \frac{1}{32} \lprp{\norm{\No} + \sigma^*_{k + 1} + \frac{\epsilon}{10n}} \\
    & \leq \frac{1}{32} \lprp{\frac{\epsilon}{5n} + \norm{\No}}
  \end{align*}

  Therefore, we can bound $\widetilde{L} - \widehat{L}$ by $\frac{\epsilon}{5\sqrt{n}} + 4\frob{\No}$. Similarly, by noting that $\widehat{L} + \widehat{C} = \widetilde{L} + \widetilde{C} + \No$, we can bound $\widetilde{C} - \widehat{C}$. This proves the theorem in this case.
  \\
  \textit{Case 2: The Algorithm Continues to the Next Iteration} In this case, we have $\frac{\epsilon}{2n} \leq \sigma_{k + 1}(\Mt[T + 1]) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}$. We prove the correctness of the theorem in two subcases:
  \\
  \textit{Sub Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[T + 1])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^{T}\sigma^*_k + \sigma^*_{k + 1}} \leq \frac{1}{32}\lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}}$. Also, with this in hand, we have $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. Note that, assumption 1 of Lemma \ref{lem:incohCont} holds via the inductive hypothesis. For the second assumption, note that $\norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}} \leq 48\mu\sqrt{\frac{r}{n}}$.
  \\
  \textit{Sub Case 2: } $\sigma^*_{k + 1} \geq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$. From this we know that, similarly to the previous subcase, $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. The rest of the proof proceeds similarly to the previous subcase.

  \textit{Stage 3:} \\
  By the induction hypothesis and Lemma \ref{lem:incohContN}, we can apply Theorem \ref{thm:aux} to $\Mt[T + 1]$. The proof of the correctness of the incoherence preserving projection is similar to the proof from \textit{Case 1} of \textit{Stage 2}.
\end{proof}


==> ArXiv/analysisSimp.tex <==
%!TEX root = rpca.tex
%\subsection{Result}
%\label{sec:resGen}
%A theoretical guarantee for the performance is provided by the following theorem:
%% \begin{theorem}
%% 	\label{thm:thmGen}
%% 	Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Furthermore, suppose that $\frob{\No} \leq \frac{\sigma^*_k}{16}$ for some $k \in [r]$. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{128\mu^2 r}$ and $\thresh$ set to $2\mu \sqrt{\frac{r}{n}}$, returns a subspace $U$ such that:
%% 	\begin{equation*}
%% 		\frob{(I - UU^\top) \Lo} \leq  3\frob{(I - U^*_k (U^*_k)^\top) \Lo} + 9 \frob{\No} + \frac{\epsilon}{10n}
%% 	\end{equation*}
%% \end{theorem}
%
%\begin{theorem}[Arbitrary Data]
%	\label{thm:thmGen}
%	Let $\Mo$ be the given corrupted data matrix, i.e., $\Mo=D^*+\Co$ where $D^*=[x_1, \dots, x_n]\in \R^{d\times n}$ contains the clean data points and the corruption matrix $\Co$ has at most $\alpha\cdot n$ non-zero columns. Furthermore, let $L^*$, the best rank-$r$ approximation of $D^*$, be $\mu$-incoherent matrix, i.e., it satisfies Assumption\ref{as:rank}. Then, for all $\alpha\leq \frac{1}{\mu^2 r}$, Algorithm~\ref{alg:} when run with below given parameters for $T=\log \frac{10\|M\|_2\cdot n}{\epsilon}$ iterations, returns a subspace $U$ such that:  %	Let $\Mo = \Lo + \Co$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{64\mu^2 r}$, returns a subspace $U$ such that:
%	\begin{equation*}
%		\frob{(I - UU^\top) L^*} \leq \sqrt{r} \|D^*-\Lo\|_2+9 \|D^*-\Lo\|_F+ \epsilon.
%	\end{equation*}
%Algorithm~\ref{} is applied with parameters $\rho=$ and $\eta=$. 
%\end{theorem}

%\subsection{Analysis}
\label{sec:anGen1}
We now briefly discuss the proof of Theorem~\ref{thm:thmN}. In fact, we prove a stronger result: 
 \begin{theorem}
 	\label{thm:masterN}
 	Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ satisfies Assumption~\ref{as:rank} and $\Co$ has column sparsity $\alpha \leq \frac{1}{128\mu^2 r}$. Furthermore, suppose that $\frob{\No} \leq \frac{\sigma^*_k}{16}$ for some $k \in [r]$. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{128\mu^2 r}$ and $\thresh$ set to $2\mu \sqrt{\frac{r}{n}}$ with $T=\log \frac{20\|\Mo\|_2\cdot n}{\epsilon}$, returns a subspace $U$ such that:
 	\begin{equation*}
 		\frob{(I - UU^\top) \Lo} \leq  3\frob{(I - U^*_k (U^*_k)^\top) \Lo} + 9 \frob{\No} + \frac{\epsilon}{10n}.
 	\end{equation*}
 \end{theorem}
Intuitively, the proof of Theorem~\ref{thm:masterN} proceeds along the same lines as that of Theorem~\ref{thm:thmCln} but requires significantly more careful analysis due to presence of noise and due to the outer loop. For example, due to the presence of noise, we cannot guarantee that Lemma~\ref{lem:clExpCl}, that was critical to proof of Theorem~\ref{thm:thmCln}, holds for all columns $i$. We show instead that the number of data points which have a large influence on the top-$k$ singular vectors is bounded (see Lemma~\ref{lem:clExpGen}). This ensures that the algorithm at least reaches the $k^{th}$ stage of the outer iteration before terminating. Similarly, we generalize Lemma~\ref{lem:clResCl} to handle $\No$ (see Lemma~\ref{lem:clResGen}). Finally, we present the key lemma that shows that if the algorithm does not terminate in the $k^{th}$ outer iteration, then it would have obtained a good approximation to the top-$k$ principal subspace of $\Lo$. 
\begin{lemma}
  \label{lem:inItPerfGen}
  Asume the conditions of Theorem~\ref{thm:thmN}. Furthermore, assume that Algorithm \ref{alg:ncpca} has not terminated during the $k^{th}$ outer iteration. Then, the iterate $U$ at the end of the $k^{th}$ outer iteration satisfies: 
  \begin{equation*}
  	\frob{(I - UU^\top) \Lo} \leq 3\frob{(I - \Uo_{1:k} (\Uo_{1:k})^\top) \Lo} + 9 \frob{\No} + \frac{\epsilon}{10n},
  \end{equation*}
  when Algorithm \ref{alg:ncpca} has been run with parameters $\nThresh = \frac{1}{128 \mu^2 r}$ and $\thresh = 2 \mu \sqrt{\frac{r}{n}}$.
\end{lemma}
See Appendix \ref{sec:pfInItPerfGen} for a detailed proof. We can now prove Theorem \ref{thm:masterN} as follows:
\begin{proof}
	Note that by Lemma \ref{lem:clExpGen}, the algorithm does not terminate before the completion of $k^{th}$ outer iteration. Now, suppose that the algorithm terminates at some iteration $k^\prime > k$. Then, by Lemma \ref{lem:inItPerfGen}, we have:

	\begin{equation*}
		\norm{\pperpu(\Lo)} \leq 3\frob{P_{\perp}^{\Uo_{1:k^\prime - 1}} (\Lo)} + 9 \frob{\No} + \frac{\epsilon}{10n} 
		\leq 3\frob{P_{\perp}^{\Uo_{1:k}} (\Lo)} + 9 \frob{\No} + \frac{\epsilon}{10n}.
	\end{equation*}
	This concludes the proof of the Theorem.
\end{proof}

==> ArXiv/conc.tex <==
\section{Conclusions and Future Works}\label{sec:conc}
In this paper, we studied the outlier robust PCA problem. We proposed a novel thresholding based approach that, under standard regularity conditions, can accurately recover the top principal directions of the clean data points, as long as the number of outliers is less than $O(1/r)$ which is information theoretically tight up to constant factors. For noiseless or arbitrary noise case, our algorithms are based on two thresholding operators to detect outliers and leads to better recovery compared to existing methods in essentially the same time as that taken by vanilla PCA. For Gaussian noise, we obtain improved recovery guarantees but at a cost of higher run time.

Though our bounds have significant improvement over existing ones, they are still weaker than guarantees obtained by vanilla PCA (with out outliers). For instance, for arbitrary  noise, our errors are bounded in the Frobenius norm. In contrast, in absence of outliers, SVD can estimate the principal directions in operator norm. A challenging and important open problem is if the principal directions can be estimated in operator norm even in the presence  of outliers.

Similarly, for Gaussian noise, where each entry has variance $\sigma^2$, our result obtains an error bound of $O(\sigma \sqrt{n})$ which is significantly better than the Frobenius norm bound we get for arbitrary noise. But again in absence of outliers, SVD can estimate the principal directions exactly asymptotically. So, another open problem is if it is possible to do asymptotically consistent estimation of the principal directions with Gaussian noise in the presence of outliers. Moreover, our algorithm for the Gaussian setting is nearly a factor of $n$ slower than that for vanilla PCA. In order for this to be practical, it is very important to design an algorithm for this setting with nearly the same runtime as that of vanilla PCA.

==> ArXiv/intro.tex <==
%!TEX root = rpca.tex

\section{Outlier Robust PCA: General Noise}\label{sec:orpca}
In this section, we introduce our algorithm for the general case of Outlier Robust PCA with arbitrary inlier data $D^*=\Lo+\No$, i.e., the noise matrix $\No$ is arbitrary. Recall that the goal is to recover left singular vectors of $\Lo$. 
\input{algSimp}
%\input{analysisSimp}

==> ArXiv/introAux.tex <==
%!TEX root = main.tex

\section{Auxilliary Algorithm}
\label{sec:introAux}
In this section, we will analyze a simple algorithm that we will use for the noisy case of the problem. Note that in the case where we have additive noise, we may threshold a large number of columns in the support of $\Lo$. For this reason, we use a new algorithm at the end of Algorithm~\ref{alg:ncpca} which does not threshold more than a fixed fraction of columnns of the matrix.


==> ArXiv/introCl.tex <==
%!TEX root = rpca.tex
%\section{Algorithms etc.}
%In all three settings, the basic idea of our algorithm is to maintain estimates of $\Do$ and $\Co$ and keep refining them via alternating projections.

\section{Outlier Robust PCA: Noiseless Setting}\label{sec:orpcacl}
In this section, we present our algorithm \ncpcacl(Algorithm~\ref{alg:ncpcacl}) that applies to the special case of noise-less data, i.e., when  $M^*=\Lo+\Co$, $\Lo$ is rank-$r$, $\mu$-incoherent matrix. While restrictive, this setting allows us to illustrate the main ideas behind our algorithm approach and the analysis techniques in a relatively simpler fashion.
\input{algCl}
%\input{analysisCl}
% \section{Problem Definition}
% Given $M^{*} = L^{*} + C^{*} \text{ where } L^{*}, C^{*} \in \mathbb{R}^{m\times n}$ which is the sum of a low rank column incoherent matrix $L^{*}$ and a column sparse corruption matrix $C^{*}$ such that the column supports of $L^{*}$ and $C^{*}$ are disjoint, the goal is to recover the column space of $L^{*}$.


==> ArXiv/introG.tex <==
%!TEX root = rpca.tex

\section{Outlier Robust PCA: Gaussian Noise}\label{sec:orpcag}
In this section, we present our algorithm for the special case of the Outlier Robust PCA problem when inlier points are generated using a standard Gaussian noise model. That is, when $D^*=\Lo+\No\in \R^{d\times n}$ where each entry of the noise matrix $\No$ is sampled i.i.d. from ${\cal N}(0, \sigma^2)$. Our result for arbitrary $\No$ (Theorem~\ref{thm:thmN}) estimates $\Uo$ up to $\sim \|\No\|_F$ error, which is $\Omega(\sigma \sqrt{dn})$ for Gaussian noise. However, using a slight variant of Algorithm~\ref{alg:ncpca} and exploiting the noise structure, Algorithm~\ref{alg:ncpcag} is able to estimate $\Uo$ up to $\sigma \sqrt{n\log d}$ error, which is better than the previous one by a factor of $\order{d/\log d}$. %We will show that non trivial recovery guarantees can be obtained even in cases where the frobenius norm of the noise is almost $\sqrt{m}$ larger than that of $\Lo$. 
\input{algG}
%\input{analysisG}

==> ArXiv/introN.tex <==
%!TEX root = main.tex
\section{Problem Definition - Noisy Case}
Given $M^{*} = L^{*} + C^{*} + N^* \text{ where } L^{*},M^{*},C^{*} \in \mathbb{R}^{m\times n}$ which is the sum of a low rank column incoherent matrix $L^{*}$, a column sparse corruption matrix $C^{*}$ with disjoint column supports and a noise matrix $N^*$, the goal is to recover $L^{*}$ and $C^{*}$.

Note that in this case, it might not be possible to exactly recover the support of $\Lo$ or the true column space of $\Lo$. We show that we can recover $\Lo$ upto a constant factor times $\frob{\No}$.


==> ArXiv/introduction.tex <==
%!TEX root = rpca.tex

\section{Introduction}
Principal Component Analysis (PCA) is a critical first step for any typical data exploration/analysis effort and is widely used in a variety of applications. A key reason for the success of PCA is that it can be performed efficiently using Singular Value Decomposition (SVD).

However, due to various practical reasons like measurement error, presence of anomalies etc., a large fraction of data points can be corrupted in a somewhat correlated and even adversarial manner. Unfortunately, SVD is fragile with respect to outliers and can lead to arbitrarily inaccurate principal directions in the presence of even a small number of outliers. So, designing an outlier robust PCA (\orpca) algorithm is critical for several application domains. 

%The goal of this work is to devise Outlier Robust PCA algorithm that can recover the principal directions despite presence of a large number of outliers.
Formally, the setting of \orpca~is as follows: given a data matrix $\Mo=\Do+\Co\in \R^{d\times n}$ where  $D^*=[x_1, \dots, x_n]$ corresponds to $n$ clean ``inlier'' data points and $\Co$ has at most $\alpha$-fraction of non-zero columns that can corrupt the corresponding clean data points arbitrarily, the goal of \orpca~is to estimate the principal components of $\Do$ accurately, i.e., recover $\Uo\in \R^{d\times r}$, the top-$r$ left singular vectors of $D^*$. %$\Uo$ accurately. That is, given $M=\Lo+\Co+\No$ where $\Lo$ is a low-rank matrix, $\Co$ is a column-sparse matrix and $\No$ is a noise matrix, the goal is to recover left singular vectors of $\Lo$. 

Vanilla SVD does not do the job since the top singular vectors of $\Mo$ can be arbitrarily far from $\Uo$ if the operator norm of $\Co$ ($\|\Co\|_2$) is large, as can be the case when $\alpha=\Omega(1)$. Any algorithm trying to solve \orpca~needs to exploit the column sparsity of $\Co$ to obtain a better estimate of $\Uo$. In particular, they need to find $S^*= \supp{\Co}$---$\supp{A}$ is the index of non-zero columns of $A$---so that $\Uo$ can be estimated using top singular directions of $\Mo_{\setminus{S^*}}$, i.e., columns of $\Mo$ restricted to complement set of $S^*$.

Existing results for \orpca~fall into two categories based on: a) Nuclear norm \citep{DBLP:journals/tit/XuCS12,DBLP:journals/tit/ZhangLZ16}, b) iterative PCA \citep{DBLP:journals/tit/XuCM13}. Nuclear norm based approaches work with exactly same setting as ours, but require $O(nd^2)$ computational time which is prohibitive for typical applications.
%Moreover, as mentioned in Table~\ref{tab:comp1}, \ref{tab:comp2} their error bounds are significantly weaker than our results.
Iterative PCA based techniques require $O(n^2d)$ computation which in general is significantly higher than our algorithms. Moreover, these results do not recover the exact principal directions even if the inliers are restricted to a low-dimensional subspace and just a constant number of outliers are present. 

Our approach is based on solving the following natural optimization problem: $$\orpca:\ \ \min_{\D, \C \in \R^{d\times n}} \|\Mo-\D-\C\|_F^2 \text{ s.t. } rank(\D)\leq r,\ \ |\supp{\C}|\leq \alpha n.$$
{\em Technical Challenges}: The main challenges with \orpca~are its non-convexity and combinatorial structure which rules out standard tools from convex optimization. Furthermore, due to the column-sparsity constraint standard SVD based techniques also do not apply. Instead, we propose a simple iterative method that constructs an estimate of outliers $C$ and using that, an estimate of the inliers $\Mo-C$. SVD of the estimated inliers is then used to obtain an estimate of the principal directions. Now, a significant challenge is to use these principal directions to re-estimate outliers. There are two different scenarios here: 
\begin{itemize}
	\item	\emph{Length of all the outliers is smaller than the smallest singular value of the inliers and hence do not stand out}: In this case however, the principal directions are not much affected by outliers. So, outliers can be recognized by taking a projection on to the orthogonal space to the estimated principal directions. As we get better estimate of principal directions, we can be more aggressive in determining the outliers. 
	\item	\emph{Length of at least one of the outliers is larger than the small singular values of inliers}: In this case again, length based thresholding fails since the lengths of the inliers are dominated by the larger singular values. Similarly, the above mentioned thresholding scheme also fails as some of the estimated principal directions will be heavily biased towards those outliers. A key and somewhat surprising algorithmic insight of our work is that:  as some of the estimated singular vectors are heavily affected by outliers, projection of such outliers on these spurious singular vectors will be inordinately high. So, in contrast to the above thresholding operator, we can use the length of projection of points along estimated principal directions as well to detect and threshold outliers. %In this case, we can compute the contribution of each of the columns to the singular vectors -- outliers stand out by showing a inordinate effect on spurious singular directions, while the real singular directions have consistent contribution from many inliers.
\end{itemize}
In both the scenarios, we can identify more outliers and repeat the procedure till convergence.
%A critical reason for success of such a technique is that $\|C\|_2$ can be controlled due to column-sparsity of $\Co$. However, if $\Co$ has a few points which have large norm, then the principal directions will be arbitrary biased along those columns of $\Co$ and hence the above mentioned iterative approach will fail. A key and somewhat surprising algorithmic insight of our work is that even if a column of $\Co$ has very high projection along estimated principal directions, then that also indicates that the column and the principal directions are "abnormal", so such columns can also be considered to be outliers and can be thresholded.
A key assumption we make, in order to ensure that inliers are not thresholded, is that most of the inliers have ``limited'' influence on the principal directions, i.e., the data matrix is incoherent (see Assumption~\ref{as:rank}). Such an assumption holds for various typical settings, for example when inliers are noisy and uniform samples from a low-dimensional subspace.  
%non-convex alternating projection style method for this problem. Fortunately, each of the non-convex projections onto set of low-rank matrix and set of column sparse matrix can be computed efficiently. But owing to non-convexity, the algorithm is not even guaranteed to converge in general. 

\noindent{\em Contributions}: \textit{The main contribution of our work is to show that, under some regularity conditions, it is indeed possible to solve \orpca~near optimally, in essentially the same time as that taken by vanilla PCA.} In particular, we propose  a thresholding based approach that iteratively estimates inliers using {\em two} different thresholding operators and then use SVD to estimate the principal directions. We also show that our method recovers $\Uo$ nearly optimally and efficiently as long as the fraction of corrupted data points (column-support of $\Co$) is less than $O(1/r)$ where $r$ is the dimensionality of principal subspace $\Uo$. More concretely, we study the problem in three settings:
\begin{enumerate}
\item {\em Noiseless setting}: $\Mo=\Do+\Co$ where the clean data matrix $D^*$ is a rank-$r$ matrix with $\mu$-incoherent right singular vectors (see Assumption~\ref{as:rank}) and $\Co$ has at most $\alpha\cdot n$ non-zero columns. For this setting, we design a novel \textbf{T}hresholding based \textbf{O}uliter \textbf{R}obust \textbf{P}CA algorithm (\ncpcacl) that recovers  $\Uo$ up to an error of $\epsilon$ in time $\order{ndr\log \frac{n\twonorm{\Mo}}{\epsilon}}$, if $\alpha\leq \frac{1}{128\mu^2 r}$. Note that this is essentially the time taken for vanilla PCA as well. In contrast, existing results for the same setting require $O(\frac{nd^2}{\epsilon^2})$\footnote{Dependence on $\epsilon$ is due to the standard rates of gradient descent when applied to the non-smooth non-strongly convex optimization problem given in \eqref{eq:nuc}; however, using more refined RSC-style analysis, $\epsilon$ dependency might be improved but we are not aware of such an existing result.} computation to recover $\Uo$. Note that the number of outliers our results can handle (i.e., $\alpha \leq 1/128 \mu^2 r$) is optimal up to constant factors in the sense that if $\alpha > 1/\mu^2 r$, then there exists a matrix $\Mo$ which has more than one decomposition satisfying the above conditions.
\item {\em Arbitrary noise}: In the second setting, $\Mo=\Do+\Co$ where the clean data matrix $\Do$ can be written as $\Lo + \No$ and $\Lo$, the rank-$r$ projection of $\Do$ has $\mu$ incoherent right singular vectors. $\Co$ on the other hand, again has at most $\alpha\cdot n$ non-zero columns. If $\alpha\leq \frac{1}{128\mu^2 r}$, our proposed algorithm \ncpcan~ guarantees recovery of $\Uo$ (left singular vectors of $\Lo$) up to $\order{\sqrt{r} \frob{\No} + \epsilon}$ error, in $\order{ndr\log \frac{n\twonorm{\Mo}}{\sqrt{r} \frob{\No} + \epsilon}}$ time. Again this is essentially the same as the time taken for vanilla PCA up to $\log$ factors. In contrast, existing results for this problem get stuck at a significantly larger error of ($\sqrt{n} \frob{\No}$), with a runtime of $O(\frac{nd^2}{\epsilon^2})$, which is slower than ours by a factor of $d$. 
\item {\em Gaussian noise}: In this setting, we again have $\Mo=\Do+\Co$ where the clean data matrix $D^*$ is a sum of low-rank matrix $\Lo$ and a Gaussian noise matrix $\No$, i.e., each element of $\No$ is sampled independently and identically (iid) from $\mathcal{N}(0,\sigma^2)$. \ncpcag, which is our proposed algorithm for this special case, recovers $\Uo$ up to an error of $\order{\sqrt{r\log d}\twonorm{\No}}$. This not only improves upon the result we obtained for the arbitrary noise case above, which is $\order{\sqrt{r} \frob{\No}}$, it also improves significantly upon the existing results. However, in order to achieve this improvement in error, we require $ n > d^2$ and the algorithm has a runtime of $\order{n^2 d}$. 
\end{enumerate}
To summarize, our results obtain stronger guarantees in terms of both final error and runtime, while being able to handle a large number of outliers, for three different settings of \orpca. Moreover, in the first two settings, our run time matches that of standard PCA up to $\log$ factors. Please refer Tables~\ref{tab:comp1} and~\ref{tab:comp2} for comparison of our results with existing results.
{
%	\renewcommand{\arraystretch}{1.5}
	\begin{table}[h]
		\begin{center}
			\begin{tabular}{| c | c | c |}
				\hline
				& \thead{Run time} & \thead{Error ($\frob{(I - \U\U^{\top})\Lo}$)} \\ \hline
				\cite{XuCS12}	& $\order{\frac{d^2n}{\epsilon^2}}$ & $\order{\sqrt{n} \frob{\No} + \epsilon}$ \\ \hline
				\ncpcan & $\order{dnr \log \frac{n \twonorm{\Mo}}{\epsilon}}$ & $\order{\sqrt{r} \frob{\No} + \epsilon}$ \\ \hline
			\end{tabular} \\
			\caption{Arbitrary noise: comparison of our results and existing results for the arbitrary noise setting. Here, $\Mo = \Do + \Co$, where $\Do = \Lo + \No$ is the clean data matrix with $\Lo$, the rank-$r$ projection of $\Do$ having $\mu$-incoherent right singular vectors (Assumption~\ref{as:rank}) and $\Co$ has $O(\frac{1}{\mu^2 r})$ is a column sparse matrix. The error is measured as the residual of $\Lo$ when projected on to the estimated space $\U$. Note that we obtain better error and better runtime compared to existing results. Also, the noiseless case is a special case with $\No = 0$.}
			\label{tab:comp1}
			\begin{tabular}{| c | c | c |}
				\hline
				& \thead{Run time} & \thead{Error($\frob{(I - \U\U^{\top})\Lo}$)} \\ \hline
				\cite{XuCS12} & $\order{\frac{n d^2 r}{\epsilon^2}}$ & $\order{\sigma n \sqrt{d}+\epsilon}$ \\ \hline
				\ncpcan & $\order{ndr^2 \log {\frac{\twonorm{\Mo}}{\epsilon}}}$ & $\order{\sigma \sqrt{nd} + \epsilon}$ \\ \hline
				\ncpcag & $\order{n^2 d r \log {\frac{\twonorm{\Mo}}{\epsilon}}}$ & $\order{\sigma \sqrt{n \log (d)}+\epsilon}$ \\ \hline
			\end{tabular}
		\caption{Gaussian noise: comparison of existing results with ours for the Gaussian noise setting: $\Mo = \Do + \Co$, where inliers $\Do = \Lo + \No$ with $\Lo$ being a rank-$r$ matrix with $\mu$-incoherent right singular vectors (Assumption~\ref{as:rank}) and $\No$ is a Gaussian matrix with variance $\sigma^2$.  Specializing \ncpcan~ for this setting already gives us faster and better results than existing ones. \ncpcag~ further improves the error by a factor of $\sqrt{d/\log d}$. The algorithm however requires extra $O(n)$ factor in the runtime.}
		\label{tab:comp2}\vspace*{-20pt}
		\end{center}
	\end{table}
}

\textbf{Paper Outline}: The paper is organized as follows. We will review related work in Section~\ref{sec:related}. We then present a formal definition of the problem in Section~\ref{sec:form} and our main results in Section~\ref{sec:results}. We then present our algorithm for each of the three settings: a) noise-less setting, b) arbitrary data, c) Gaussian noise, in Section~\ref{sec:orpcacl}, \ref{sec:orpca}, \ref{sec:orpcag}, respectively. We provide a brief overview of our proofs in Section~\ref{sec:po}. Finally, we conclude with a few open problems and promising future directions in Section~\ref{sec:conc}. 
\subsection{Related Works}
\label{sec:related}
In this section, we will discuss related work and compare existing results with ours. Existing theoretical results for OR-PCA fall into two categories:

a) The first category of approaches, more in-line with our own work, are based on Outlier-Pursuit (\cite{DBLP:journals/tit/XuCS12}) which optimizes a convex relaxation of the OR-PCA problem where the rank and column sparsity constraints are replaced by the trace-norm (sum of singular values) and $\norm{.}_{2, 1}$ (sum of the column lengths) penalties. That is, they solve the following optimization problem:
\begin{equation}\label{eq:nuc}
	\text{(Outlier Pursuit): } \min \norm{L}_{*} + \lambda \norm{C}_{2, 1}\ s.t\ \frob{M - L + C} \leq \frob{\No}.
\end{equation}
While outlier pursuit obtains optimal recovery guarantees in absence of any noise, a main drawback is that its computational complexity is quadratic in $d$, i.e., $O(nd^2)$. Moreover, in presence of noise the bounds given in \cite{DBLP:journals/tit/XuCS12} are $O(\sqrt{n})$ worse than our result. Extensions of Outlier-Pursuit to the partially observed setting (\cite{DBLP:journals/tit/ChenXCS16}) and online setting \cite{DBLP:conf/nips/FengXY13} have also been proposed but share the drawback of high computational complexity. Recently, \cite{DBLP:journals/tit/ZhangLZ16} showed that Outlier Pursuit achieves recovery even with the fraction of outliers larger than the information theoretic lower bound. However, this requires the outliers to be ``well-spread'' which in practice is restrictive; our results allow the corruption matrix to be constructed in adversarial manner although the corruptions cannot depend on the Gaussian noise in the setting (3) described in previous section. 

b) The second line of approaches based on HR-PCA (\cite{DBLP:journals/tit/XuCM13}) iteratively prune or reweigh data points which have a large influence on the singular vectors and select an estimate with the Robust Variance Estimator metric. When applied to our finite sample setting, these results cannot achieve exact recovery even in the noiseless case with a single outlier. Moreover, their running time in this setting is $\order{n^2dr}$ while ours is nearly linear in the input size. In the special case of Gaussian noise, these results incur at least a constant error $\order{\sigma_1(\Lo)}$ whereas our recovery guarantee scales linearly with the standard deviation of the noise $\order{\sqrt{r} \sigma\log d}$, achieving exact recovery when $\sigma = 0$. \cite{DBLP:conf/icml/FengXY12} propose a deterministic variant of HR-PCA and \cite{DBLP:conf/icml/YangX15} extend HR-PCA to PCA-like algorithms like Sparse PCA and Non-Negative PCA.

There has been much recent work on the related problem of Robust PCA (\cite{CandesLMW11}, \cite{NIPS2014_5430}, \cite{DBLP:conf/nips/YiPCC16}, \cite{DBLP:journals/corr/CherapanamjeriG16}). In contrast to the setting considered here, the corruptions are assumed to be both row and column sparse i.e., unlike our setting no data can be corrupted in all its dimensions. This restriction allows stronger recovery guarantees but makes the results inapplicable to the setting of outlier robust PCA. 

\subsection{Notations}
We use the following notations in this paper. For a vector $v$, $\norm{v}$ and $\twonorm{v}$ denote the $\ell_2$ norm of $v$. For a matrix $\M$, $\norm{\M}$ and $\twonorm{\M}$ denote the operator norm of $\M$ while $\frob{\M}$ denotes the Frobenius norm of $\M$. $\sigma_k(\M)$ denotes the $k^{\textrm{th}}$ largest singular value of $\M$. SVD refers to singular value decomposition of a matrix. $\mathcal{SVD}_r(\M)$ refers to the rank-$r$ SVD of $\M$. Given a matrix $\M$, $\M_i$ denotes the $i^{\textrm{th}}$ column of $\M$ while $\M_{i,:}$ denotes the $i^{\textrm{th}}$ row of $M$. Given a matrix $\M \in \R^{d\times n}$ and a set $S\subseteq [n]$, $\M_S$ is defined as
\begin{align*}
	(\M_S)_i = \left\{ \begin{array}{ll}
	\M_i &\mbox{ for } i \in S,\\
	0 &\mbox{ otherwise.}
	\end{array}\right.			
\end{align*}
$\M_{\setminus S}$ denotes $\M_{[n]\setminus S}$. $\supp{M}$ denotes column support of $M$, i.e., the set of indices of non-zero columns of $M$. 

We use two hard -thresholding operators in this paper.
Given a matrix $\Rm$, the first hard-thresholding operator, $\mathcal{HT}_\nThresh \lprp{\Rm}$ denotes the set of indices $j$ of the top $\nThresh$ fraction of largest columns (in $\ell_2$ norm) in $\Rm$. Given a matrix $\Rm$, the second hard-thresholding operator $\widetilde{\HT{\zeta}}(\Rm)$ is defined as,
\begin{equation}
\label{eqn:httDef}
\widetilde{\HT{\zeta}}(N)=\{i:\ \text{s.t. } \|N_{i}\|_2 \geq \zeta\}.
\end{equation}
$\pperpu(M)$ denotes $(I-UU^\top)M$. For any set $\mathcal{S} \in \mathbb{R}^{d}$, we will use $\Pr{\mathcal{S}}$ to denote the projection onto the set $\mathcal{S}$. We will also use $\Pr{U}$ to denote the projection onto the column space of $U$ for $U \in \mathbb{R}^{d \times r}$. 

==> ArXiv/introduction_bk.tex <==
\section{Introduction}
Principal Component Analysis (PCA) is one of the most important first step for a typical data exploration/analysis effort. While PCA can be performed optimally and efficiently using the Singular Value Decomposition (SVD), the algorithm itself is fragile w.r.t. outliers. That is, in presence of a small number of corrupted/outlier points, SVD can output arbitrarily inaccurate principal directions. 

The goal of this work is to devise Outlier Robust PCA (ORPCA) algorithm that can recover the principal directions despite presence of a large number of outliers. Given data matrix $M=[x_1, \dots, x_n]\in \R^{d\times n}$ where $(1-\rho)$ fraction of points $x_i$ are noisy samples from a subspace $\Uo$ and the remaining $\rho$ fraction of points can be arbitrary corrupted, the goal of ORPCA is to recover $\Uo$ accurately. That is, given $M=\Lo+\Co+\No$ where $\Lo$ is a low-rank matrix, $\Co$ is a column-sparse matrix and $\No$ is a noise matrix, the goal is to recover left singular vectors of $\Lo$. 

Note that the top singular vectors of $M$ can be arbitrary far from $\Uo$ as the operator norm of $\Co$ ($\|\Co\|_2$) can be quite large when $\rho=\Omega(1)$ even if dimensionality of $\Uo$ is a constant. So, the goal of ORPCA algorithms is to exploit the column sparsity of $\Co$ to obtain better estimator for $\Uo$. That is, the goal is to find $S^*=$column-support$(\Co)$ (where column-support($A$) is the index of non-zero columns of $A$) so that $\Uo$ can be estimated using top singular directions of $M_{\bar{S^*}}$, i.e., columns of $M$ restricted to complement set of $S^*$. 

Existing result for ORPCA falls in two categories: a) nuclear norm based, b) truncated inner product based. YESHWANTH provide details here. Main thing is to say that nuclear norm based methods are $O(d^2 n)$ while (b) are weak because ...

In contrast, our approach is based on solving the following natural optimization problem: $$\textsf{(ORPCA)}:\ \ \min_{L, C} \|M-L-C\|_F^2 \text{ s.t. } rank(L)\leq r, |\text{column-support}(C)|\leq s.$$
The main challenge with ORPCA is non-convexity and combinatorial structure of the above optimization problem which rules out standard optimization tools. Instead, we propose a simple non-convex alternating projection style method for this problem. Fortunately, each of the non-convex projection onto set of low-rank matrix and set of column sparse matrix can be computed efficiently. But owing to non-convexity, the algorithm is not even guaranteed to converge in general. 

The main contribution of our work is to show that despite non-convexity of the projection sets, our algorithm recover $\Uo$ nearly optimally as long as the fraction of corrupted data points (column-support of $\Co$) is less than $O(1/r)$ where $r$  
is the dimensionality of principal subspace $\Uo$. Concretely, we study the problem in three settings: \begin{enumerate}
\item {\em Noiseless Setting}: $M=D^*+\Co$ where clean data matrix $D^*$ is a rank-$r$ matrix with $\mu$-incoherent right singular vectors (see Definition~\ref{defn:incoh}). 
\item {\em Gaussian noise Setting}: 
\item {\em Arbitrary Data Matrix}: 
\end{enumerate}
\subsection{Related Works}

==> ArXiv/notations_praneeth.tex <==
We use two hard -thresholding operators in this paper.
Given a matrix $\Rm$, the first hard-thresholding operator, $\mathcal{HT}_\nThresh \lprp{\Rm}$ denotes the set of indices $j$ of the top $\nThresh$ fraction of largest columns (in $\ell_2$ norm) in $\Rm$. Given a matrix $\Rm$, the second hard-thresholding operator $\widetilde{\HT{\zeta}}(\Rm)$ is defined as,
\begin{equation}
\label{eqn:httDef}
\widetilde{\HT{\zeta}}(N)=\{i:\ \text{s.t. } \|N_{i}\|_2 \geq \zeta\}.
\end{equation}
$\pperpu(M)$ denotes $(I-UU^\top)M$. For any set $\mathcal{S} \in \mathbb{R}^{d}$, we will use $\Pr{\mathcal{S}}$ to denote the projection onto the set $\mathcal{S}$. We will also use $\Pr{U}$ to denote the projection onto the column space of $U$ for $U \in \mathbb{R}^{d \times r}$.

==> ArXiv/proofoverview.tex <==
\section{Proof Overview}\label{sec:po}
In this section, we provide a brief overview of our analysis for the three main results. 
\subsection{Noiseless Setting---Theorem~\ref{thm:thmCln}}
\input{analysisCl}
\subsection{Arbitrary Noise---Theorem~\ref{thm:thmN}}
\input{analysisSimp}
\subsection{Gaussian Noise---Theorem~\ref{thm:thmG}}
\input{analysisG}

==> ArXiv/result.tex <==
\section{Our Results}\label{sec:results}
In this section, we will present our results for the three settings mentioned above.
\subsection{\orpca~-- Noiseless Setting}
Recall that in the noiseless setting, we observe $\Mo = \Do + \Co$ where $\Do$ is a rank-$r$, $\mu$-incoherent matrix corresponding to clean data points and the column-support of $\Co$ is at most $\alpha n$. % column sparse matrix with only $\alpha$ fraction of non-zero columns corresponding to outliers.
The following theorem is our main result for this setting.
\begin{theorem}[Noise-less Setting]
	\label{thm:thmCln}
	Let $\Mo, \Do$ and $\Co$ be as described above. If $\alpha\leq \frac{1}{128 \mu^2 r}$, then Algorithm~\ref{alg:ncpcacl} run with parameters $\nThresh = \frac{1}{128\mu^2 r}$ and $T=\log \frac{10 n \|\Mo\|_2}{\epsilon}$, returns a subspace $U$ such that,  %	Let $\Mo = \Lo + \Co$ such that 
%	Let $\Mo$ be the given corrupted data matrix, i.e., $\Mo=D^*+\Co$ where $D^*=[x_1, \dots, x_n]\in \R^{d\times n}$ contains the clean data points and the corruption matrix $\Co$ has at most $\alpha\cdot n$ non-zero columns. Furthermore, let $D^*$ be rank-$r$ and $\mu$-incoherent matrix, i.e., it satisfies Assumption\ref{as:rank}. Then, for all $\alpha\leq \frac{1}{\mu^2 r}$, Algorithm~\ref{alg:ncpcacl} when run with parameter $\nThresh = \frac{1}{64\mu^2 r}$ for $T=\log \frac{10\|M\|_2\cdot n}{\epsilon}$ iterations, returns a subspace $U$ such that,  %	Let $\Mo = \Lo + \Co$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{64\mu^2 r}$, returns a subspace $U$ such that:
	\begin{equation*}
	\frob{(I - UU^\top) D^*} \leq \epsilon.
	\end{equation*}
\end{theorem}
\textbf{Remarks}:
\begin{itemize}
	\item	Note that the guarantee of Theorem~\ref{thm:thmCln} can be right away converted to a bound on the subspace distance between $U$ and that spanned by the columns of $\Do$. In particular, we obtain $\frob{(I - UU^\top)\Uo} \leq \epsilon/\sigma_r(\Do)$, where $\sigma_r(\Do)$ denotes the smallest singular value of $\Do$ and $\Uo$ contains the singular vectors of $\Do$.
	\item	Since the most time consuming step in each iteration is computing the top-$r$ SVD of an $n\times d$ matrix, the total runtime of the algorithm is $\order{ndr\log \frac{10 n \|\Mo\|_2}{\epsilon}}$.
	\item	The above assumption on the column sparsity of $\Co$ is tight up to constant factors i.e., we may construct an incoherent matrix $\Lo$ and column sparse matrix $\Co$ such that it is not possible to recover the true column space of $\Lo$ when the column sparsity of $\Co$ is larger than $\frac{1}{\mu^2 r}$.
\end{itemize}
%Remarks: subspace distance, run-time complexity (near optimal and contrast to existing results), bring down factor of $r$ furthermore using binary search, value of $\rho$, incoherence-standard assumption. 
\subsection{\orpcan~-- Arbitrary Noise}
We now consider the noisy setting. Here we observe $\Mo = \Do + \Co$, where $\Do$ is a near low rank matrix i.e., $\Do = \Lo + \No$ where $\Lo$ is the best rank $r$ approximation to $\Do$ and is a $\mu$ incoherent matrix, while $\No$ is a noise matrix. $\Co$ is again column sparse with at most an $\alpha$ fraction of the columns being non-zero.
\begin{theorem}[Arbitrary Noise]
	\label{thm:thmN}
Consider the setting above. If $\alpha\leq \frac{1}{128 \mu^2 r}$, then Algorithm~\ref{alg:ncpca} when run with parameters $\rho=\frac{1}{128\mu^2 r}$, $\eta=2\mu \sqrt{\frac{r}{n}}$ and $T=\log \frac{20\|\Mo\|_2\cdot n}{\epsilon}$ iterations, returns a subspace $U$ such that:%\praneeth{Check the parameter choices.} %	Let $\Mo = \Lo + \Co$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{64\mu^2 r}$, returns a subspace $U$ such that:
	\begin{equation*}
	\frob{(I - UU^\top) L^*} \leq 60 \sqrt{r} \frob{\No} + \epsilon.
	\end{equation*}
\end{theorem}
\textbf{Remarks}:
\begin{itemize}
	\item	The theorem shows that up to $\sqrt{r}\frob{\No}$ error, recovered directions $U$ contains top $r$ principle directions of inliers. We do not optimize the constants in our proof. In fact, we obtain a stronger result in Theorem~\ref{thm:masterN} which for certain regime of noise $\No$ can lead to significantly better error bound. Note that when there is no noise i.e., $\No = 0$, we recover Theorem~\ref{thm:thmCln}.
	\item	The guarantee here can again be converted to a bound on subspace distance. For instance, for any $k \leq r$, we have $\frob{(I - \U\U^{\top})\Uo_{[k]}}\leq \left(60 \sqrt{r} \frob{\No}+ \epsilon\right)/\sigma_k(\Lo)$, where $\Uo_k$ denotes the top-$k$ left singular subspace of $\Lo$ and $\sigma_k(\Lo)$ denotes the $k^{\textrm{th}}$ largest singular value of $\Lo$.
	\item	The total runtime of the algorithm is $\order{ndr^2 \log \frac{10\|\Mo\|_2\cdot n}{\epsilon}}$. However, the outer loop over $k$ in Algorithm~\ref{alg:ncpca} can be replaced by a binary search for values of $k$ between $1$ and $r$. This reduces the runtime to $\order{ndr \log r\log \frac{10 \|\Mo\|_2\cdot n}{\epsilon}}$. See Algorithm~\ref{alg:ncpcab} for more details. %\praneeth{Yeshwanth: reference here for binary search argument}.
	%\item	subspace distance, quick reminder of run-time complexity and contrat to existing one, but we have better error bound with same $\rho$, why frob norm in $N$ and point that it can be improved if $N$ has special structure (Gaussian case),   tighter statement and intuition of $k$
\end{itemize}


\subsection{\orpcag -- Gaussian Noise}
We now consider the Gaussian noise setting. Here we observe $\Mo = \Do + \Co$, where $\Do$ is a near low rank matrix i.e., $\Do = \Lo + \No$ where $\Lo$ is a rank-$r$, $\mu$ incoherent matrix, while $\No$ is a Gaussian matrix with each entry sampled iid from $\mathcal{N}(0,\sigma^2)$. $\Co$ is again column sparse with at most an $\alpha$ fraction of the columns being non-zero.

\begin{theorem}[Gaussian Data]
	\label{thm:thmG}
%	Let $\Mo$ be the given corrupted data matrix, i.e., $\Mo=D^*+\Co$ where $D^*=[x_1, \dots, x_n]\in \R^{d\times n}$ contains the clean data points and the corruption matrix $\Co$ has at most $\alpha\cdot n$ non-zero columns. Furthermore, let $D^*=\Lo+N^*$ where $L^*$ is $\mu$-incoherent rank-$r$ matrix (i.e. it sastisfies Assumption\ref{as:rank}) and each entry of $N^*$ is sampled from $N(0, \sigma^2)$.
Consider the setting mentioned above. Suppose $\alpha\leq \frac{1}{1024\mu^2 r}$. Then, Algorithm~\ref{alg:ncpcag} stops after at most $T=\alpha n$ iterations and returns a subspace $U$ such that:  %	Let $\Mo = \Lo + \Co$ such that $\Lo$ and $\Co$ satisfiy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Then, Algorithm \ref{alg:ncpcacl} run with $\nThresh = \frac{1}{64\mu^2 r}$, returns a subspace $U$ such that:
	\begin{equation*}
	\|(I - UU^\top) L^*\|_2\leq 4\sqrt{\log d}\|N^*\|_2.
	\end{equation*}
with probability at least $1-\delta$ as long as $n \geq \frac{16\mu^2r^2d}{c_1} \left[\log\lprp{\frac{1}{3\delta}} + d\log(80d)\right]$ for some absolute constants $c_1$ and $c_2$.
\end{theorem}%\praneeth{Please check the theorem statement and remarks. I think the statement is not correct -- it should not have a $T$. Runtime also needs a tighter argument.}

\textbf{Remarks}:
\begin{itemize}
	\item	Data points coming from a low-dimensional subspace with additive Gaussian noise is a standard statistical model that is used to justify PCA. Though this can be seen as a special case of arbitrary noise model, we get a much tighter bound than that obtained from Theorem~\ref{thm:thmN}.
	\item	While Theorem~\ref{thm:thmN} gives an asymptotic error bound of $\frob{(I - UU^\top) L^*} \leq 60 \sqrt{r} \frob{\No}$, Theorem~\ref{thm:thmG} gives an asymptotic error bound of $\frob{(I - UU^\top) L^*} \leq 4  \twonorm{\No}$. Note that the right hand sides above refer to Frobenius and operator norms respectively.
	\item	The improvement mentioned above is obtained by carefully leveraging the fact that Gaussian random vectors are spread uniformly in all directions and that there is a small fraction of vectors which is correlated. However, in order to make this argument, we need $n = \order{d^2}$. It is an open problem to get rid of this assumption.% Moreover, the algorithm also has a run time of $\order{n^2d}$.
	\item	Note also that our result is tight in the sense that as $\sigma \rightarrow 0$, we recover the result of Theorem~\ref{thm:thmCln}. However, the running time of the algorithm is $O(n^2 d)$ which is significantly worse than that of \ncpcacl. We leave design/analysis of a more efficient algorithm that achieves similar error bounds as Theorem~\ref{thm:thmG} as an open problem. 
	\item 	We can obtain the above result even when each column in $\No$ is drawn from a sub-Gaussian distribution rather than each entry being iid $\mathcal{N} (0, \sigma^2)$.
\end{itemize}

==> ArXiv/setup.tex <==
%!TEX root = rpca.tex

\section{Problem Formulation}
\label{sec:form}
In this section, we will formally present the setting of the paper. We are given $\Mo = \Do + \Co \in \R^{d\times n}$, where columns of $\Do$ are inliers and $\Co$ are outliers. Only an $\alpha$ fraction of the points are outliers, i.e., only $alpha$ fraction of the columns of $\Co$ are non-zero. Broadly, we consider three scenarios:
\begin{itemize}
	\item	\textit{\orpca} (Noiseless setting): The points in $\Do$ lie \textit{entirely} in a low-dimensional subspace i.e., $\Do=\Lo$ is a rank-$r$ matrix.
	\item	\textit{\orpcan} (Noisy setting): The points in $\Do$ lie \textit{approximately} in a low-dimensional subspace i.e., $\Do = \Lo + \No$ where $\Lo$ is the rank-$r$ projection of $\Do$ and $\No$ is the noise matrix.
	\item	\textit{\orpcag} (Gaussian noise setting): The points in $\Do$ come from a low-dimensional subspace with additive Gaussian noise i.e., $\Do = \Lo + \No$ where $\Lo$ is a rank-$r$ matrix and $\No$ is a Gaussian noise matrix i.e., each element of $\No$ is sampled iid from $\mathcal{N}(0,\sigma^2)$.
\end{itemize}
In all the above settings, the goal is to find the low dimensional subspace spanned by the columns of $\Lo$.
%In this section, we will formalize the problem of Outlier Robust PCA and its variants. In this paper, we propose algorithms for two variants of the problem. We will assume that we are provided $n$ data points in $\mathbb{R}^m$ such that a $\colSp$ fraction of the points are corrupted. We will denote our data matrix as $\Mo \in \mathbb{R}^{m \times n}$ where the data points are arranged along the columns of $\Mo$. Since, data points lying exactly on a low dimensional subspace is rare in realistic scenarios, we also allow the remaining $(1 - \colSp)$ to be contaminated by noise. Therefore, we may decompose our data matrix $\Mo$ as the sum of three matrices $\Lo$, $\No$ and $\Co$ where $\Lo$ is a low rank matirx whose column space we wish to recover, $\No$ represents the noise present in the dataset and $\Co$ represents the $\colSp n$ corrupted points. We propose the following two formulations of the problem depending on the nature of $\No$:
%
%\begin{itemize}
%	\item \textbf{Outlier Robust PCA: } In the most general formulation of the problem, we are given a matrix $\Mo = \Lo + \No + \Co$ where $\Lo$ is low rank, $\No$ is an arbitrary noise matrix and $\Co$ is column sparse and the goal is to recover the column space of $\Lo$. To solve this problem, we attempt to solve the following non-convex optimization problem.
%
%	\begin{equation}
%		\label{eqn:ncpcaNDef}
%		\orpcan \text{ : } \argmin\limits_{U \in \mathbb{R}^{m \times r}} \frob{(I - UU^\top) (\Mo - C)} \text{ s.t } \supp{C} \leq \nThresh n
%	\end{equation}
%
%	\item \textbf{Outlier Robust PCA with Gaussian Noise: } In a special case of the above problem, we are given a matrix $\Mo = \Lo + \No + \Co$ where $\Lo$ is low rank, $\No$ is a statistical noise matrix whose entries are iid Gaussian $\mathcal{N}(0, \sigma^2)$ and $\Co$ is column sparse. The goal, again, is to to recover the column space of $\Lo$. Similar to the perviously defined problem, we try to solve the following optimization problem:
%
%	\begin{equation}
%		\label{eqn:ncpcaGDef}
%		\orpcag \text{ : } \argmin\limits_{U \in \mathbb{R}^{m \times r}} \norm{(I - UU^\top) (\Mo - C)} \text{ s.t } \supp{C} \leq \nThresh n
%	\end{equation}	
%\end{itemize}
%
%Note that while the second formulation is much more stringent than the first, assuming Gaussian noise as opposed to the much more general arbitrary noise assumption, we will see that we may still obtain non trivial estimates of the principal subspace even in cases when the Frobenius norm of the noise matrix $\No$ is much larger than that of $\Lo$ (By almost a factor of $\sqrt{d}$)!

This problem is in general ill-posed. Consider for instance the case, when most of the true data points $\Lo$ are zero and only an $\alpha$ fraction of them are non-zero. These points can either be considered inliers or outliers. In order to overcome this issue, standard assumption used in literature~\citep{DBLP:journals/tit/XuCS12, DBLP:conf/nips/FengXY13} is that of incoherence. Also, incoherence is satisfied in several standard settings; for example, when the inliers are noise and uniform samples from a low-dimensional subspace. 
%To justify our choice of optimization problems, consider the case when $\No = 0$. In this case, setting $C$ to $\Co$ and $U$ to the column space of $\Lo$ is an optimal solution to both optimization problems. Note that without further assumptions, this still doesn't guarantee that all solutions will recover the true subspace of $\Lo$. One such case is when both $\Co$ and $\Lo$ have supports of size $\colSp n$. To discount such trivial cases, we impose additional assumptions on the matrices $\Lo$ and $\Co$:
\begin{assumption}
  \label{as:rank}
  \textbf{Rank and incoherence of $\Lo$: } $\Lo\in \mathbb{R}^{d\times n}$ is a rank-$r$ incoherent matrix, i.e., $\twonorm{e_{i}^{\top}V^*} \leq \mu \sqrt{\frac{r}{n}} \ \forall i\in [n]$, where $\Lo = U^*\Sigma^* (V^*)^{\top}$ is the SVD of $\Lo$.
\end{assumption}

%\begin{assumption}
%  \label{as:colSup}
%  \textbf{Fraction of outliers: } $\Co \in \mathbb{R}^{d\times n}$ is a column sparse matrix with column sparsity $\colSp$ satisfying $\colSp \leq \frac{1}{128\mu^2r}$.
%\end{assumption}

%The above assumption on the column sparsity of $\Co$ is tight up to constant factors i.e., we may construct an incoherent matrix $\Lo$ and column sparse matrix $\Co$ such that it is not possible to recover the true column space of $\Lo$ when the column sparsity of $\Co$ is $\frac{1}{\mu^2 r}$.

==> algo.tex <==
%!TEX root = main.tex
\section{Algorithm - Without Noise}\label{sec:prob}

Here, we present our algorithm for solving the Robust PCA problem.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \ncpca$(M, r, \thresh, \beta, \epsilon)$}
  \label{alg:ncpca}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Thresholding Parameter $\thresh$, Incoherence Thresholding Parameter $\beta$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    % \FOR {Iteration $q = 0$ to $q = T$}
    %   \STATE $\zeta \leftarrow \thresh \sigma_1 (\Mt[q])$
    %   \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q]}$
    % \ENDFOR
    %
    % \STATE $\Mt[0] \leftarrow \Mt[T + 1]$

    \FOR{Outer Iteration $k = 0$ to $k = r$}
      \FOR{Inner Iteration $q = 0$ to $q = T$}
        \STATE $L = \Pk[k] (\Mt[q])$
        \STATE $\zeta \leftarrow \thresh \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma_{k}(\Mt[q]) + \sigma_{k + 1}(\Mt[q])}$
        \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q] - L}$
      \ENDFOR
      \IF{$\sigma_{k + 1}(\Mt[T + 1]) \leq \frac{\epsilon}{2n}$}
        \STATE \textbf{break}
      \ENDIF
      \STATE $[U, S, V] \leftarrow \mathcal{SVD}_{k + 1} \lprp{\Mt[T + 1]}$
      \STATE $\zeta \leftarrow 2\thresh \sigma_{k + 1}(\Mt[T + 1])$
      \STATE $\Mt[0] \leftarrow \HTz \lprp{\Mt[T + 1], \Mt[T + 1] - USV^\top}$
      \STATE $\Mt[0] \leftarrow \HTb \lprp{\Mt[0], US^{-1}U^{\top} \Mt[T + 1]}$
    \ENDFOR
    \STATE {\bf Return: }$\Pr{r}(\Mt[T + 1])$
  \end{algorithmic}
\end{algorithm}

Here, we $\mathcal{HT}_{\gamma}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htDef}
  (\mathcal{HT}_{\gamma}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ \norm{N_{:, i}} \leq \gamma \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}


==> algoAux.tex <==
%! TEX root = main.tex

\section{Algorithm - Auxilliary}
\label{sec:algAux}
Here, we introduce our algorithm which has a threshold on the maximum number of columns that are thresholded by the matrix at any time.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \auxAlgo$(M, r, \alpha^\prime, \epsilon)$}
  \label{alg:aux}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Maximum Thresholding fraction $\alpha^\prime$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    \FOR{Iteration $t = 0$ to $t = T$}
      \STATE $U^{(t)} \leftarrow LSV_r \lprp{\Mt[t]}$
      \STATE $\Mt[t + 1] \leftarrow \HTap\lprp{M, \Pr{U^{(t)}}^\perp \lprp{M}}$
    \ENDFOR
    \STATE {\bf Return: }$\Mt[T + 1]$
  \end{algorithmic}
\end{algorithm}

Here, we $\mathcal{HT}_{\alpha}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htADef}
  (\mathcal{HT}_{\alpha}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ N_{:, i} \text{ is one of the } \alpha n \text{ longest columns of N} \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}


==> algoN.tex <==
%!TEX root = main.tex
\section{Algorithm - Noisy Case}\label{sec:prob}

Here, we present our algorithm for solving the Robust PCA problem with noise. Due to the noise, it might be possible for columns in the support of $\Lo$ to get thresholded by our algorithm. To solve this problem, we will use the algorithm introducted for the case where there is no noise (Algorithm \ref{alg:ncpca}) except that we will only let $k$ range from $0$ till $r - 1$. Instead of the final outer iteration, we will run Algorithm \ref{alg:aux} which has a bound on the maximum number of columns that are ever thresholded in an iteration. We prove that if the noise ($\frob{\No}$) is suitably small, we will not threshold too many clean columns till we run Algorithm \ref{alg:aux}.

\begin{algorithm}[!h]
  \caption{$L ~ =$ \ncpcan$(M, r, \thresh, \beta, \alpha^\prime, \mu, \epsilon)$}
  \label{alg:ncpcan}
  \begin{algorithmic}[1]
    \STATE {\bf Input}: Corrupted matrix $M \in \mathbb{R}^{m\times n}$, Target rank $r$, Thresholding Parameter $\thresh$, Incoherence Thresholding Parameter $\beta$, Maximum Thresholding Parameter $\alpha^\prime$, Incoherence Parameter $\mu$, Convergence criterion $\epsilon$
    \STATE $T \leftarrow \log{\frac{20n\sigma_1(M)}{\epsilon}}$
    \STATE $\Mt[0] \leftarrow M$

    \FOR{Outer Iteration $k = 0$ to $k = r - 1$}
      \FOR{Inner Iteration $q = 0$ to $q = T$}
        \STATE $L = \Pk[k] (\Mt[q])$
        \STATE $\zeta \leftarrow \thresh \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma_{k}(\Mt[q]) + \sigma_{k + 1}(\Mt[q])}$
        \STATE $\Mt[q + 1] \leftarrow \HTz \lprp{\Mt[q], \Mt[q] - L}$
      \ENDFOR

      \IF{$\sigma_{k + 1}(\Mt[T + 1]) \leq \frac{\epsilon}{2n}$}

        \STATE $[U^\prime, S^\prime, V^\prime] \leftarrow SVD_k(\Mt[T + 1])$
        \STATE $\widehat{L} \leftarrow \Pr{U^\prime S^\prime, 2\mu \sqrt{r / n}} (M)$
        \STATE $\widehat{C} \leftarrow M - \widehat{L}$

        \STATE \textbf{Return: } $(\widehat{L}, \widehat{C})$
      \ENDIF

      \STATE $[U, S, V] \leftarrow \mathcal{SVD}_{k + 1} \lprp{\Mt[T + 1]}$
      \STATE $\zeta \leftarrow 2\thresh \sigma_{k + 1}(\Mt[T + 1])$
      \STATE $\Mt[0] \leftarrow \HTz \lprp{\Mt[T + 1], \Mt[T + 1] - USV^\top}$
      \STATE $\Mt[0] \leftarrow \HTb \lprp{\Mt[0], US^{-1}U^{\top} \Mt[T + 1]}$
    \ENDFOR

    \STATE $L^\prime \leftarrow $ \auxAlgo$(\Mt[T + 1], r, \alpha^\prime, \epsilon / n^2)$
    \STATE $[U^\prime, S^\prime, V^\prime] \leftarrow SVD_r(L^\prime)$
    \STATE $\widehat{L} \leftarrow \Pr{U^\prime, S^\prime, 2\mu \sqrt{r / n}} (M)$
    \STATE $\widehat{C} \leftarrow M - \widehat{L}$

    \STATE {\bf Return: }$(\widehat{L}, \widehat{C})$
  \end{algorithmic}
\end{algorithm}

Here, we define $\mathcal{HT}_{\gamma}(M, N)$ is defined as:

\begin{equation}
  \label{eqn:htDef}
  (\mathcal{HT}_{\gamma}(M, N))_{:, i} =
  \begin{cases}
    & M_{:, i},\ \norm{N_{:, i}} \leq \gamma \\
    & 0,\text{ otherwise}
  \end{cases}
\end{equation}

We also define the incoherence preserving projection operator ($\Pr{U, S, \delta}$) on a matrix $A$ as follows:

\begin{equation}
  \label{eqn:iProjDef}
  (\Pr{U, S, \delta} (A))_{:, i} = \argmin\limits_{\norm{U S^{-1} U^\top y} \leq \delta} \norm{A_{:, i} - y}
\end{equation}


==> analysis.tex <==
%!TEX root = main.tex
\renewcommand{\u}{\bm{u}}
\section{Analysis - Without Noise}\label{sec:analysis}

\begin{assumption}
  \label{as:rank}
  \textbf{Rank and incoherence of $\Lo$: } $\Lo\in \mathbb{R}^{m\times n}$ is a rank-$r$ incoherent matrix, i.e., $\twonorm{e_{i}^{\top}V^*} \leq \mu \sqrt{\frac{r}{n}} \ \forall i\in [n]$, where $\Lo = U^*\Sigma^* (V^*)^{\top}$ is the SVD of $\Lo$.
\end{assumption}

\begin{assumption}
  \label{as:colSup}
  \textbf{Column Sparsity of $\Co$: } $\Co \in \mathbb{R}^{m\times n}$ is a column sparse matrix with column sparsity $\colSp$ satisfying $\colSp \leq \frac{c}{\mu^2r}$ for some suitable small constant $c$.
\end{assumption}

Assumptions \ref{as:rank} and \ref{as:colSup} as standard assumptions for the Robust PCA problem. Note that column sparsity above $\frac{1}{\mu^2r}$ cannot be tolerated by any algorithm for robust PCA as the low rank component and the column sparse component may become indistinguishable.

We obtain the following theorem guaranteeing the optimality of our algorithm under the assumptions specified.

% \begin{theorem}
%   \label{thm:master}
%   Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $L$ satisfying:
%   \begin{equation*}
%     \frob{L - \Lo} \leq \epsilon
%   \end{equation*}
% \end{theorem}

\begin{theorem}
  \label{thm:master}
  Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $\Lo$.
\end{theorem}

\textbf{Notation}: We use $Pos^{*}(\sigma)$ to denote the number of singular values of $\Lo$ greater than $\sigma$. Let the column support of a matrix be denoted as $\supp{M}$. Let $\itnorm{M}$ denote the length of the longest column of a matrix.

We track two important quantities during outer iteration $k$ through the proof of Theorem \ref{thm:master}:
\begin{equation}
  \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])},\ \itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}
\end{equation}

We will now present some lemmas useful for the analysis. The first lemma bounds the norm of a column sparse matrix.

\begin{lemma}
  \label{lem:spNrm}
  Let $A \in \mathbb{R}^{m \times n}$ be a column sparse matrix with column sparsity $\alpha$ such that $\itnorm{A} \leq B$. Then $\norm{A} \leq \sqrt{\alpha n} B$
\end{lemma}

\begin{proof}
  The forbenius norm of $A$ is bounded by $\sqrt{\alpha n} B$ which is an upper bound on $\norm{A}$.
\end{proof}

In the next lemma, we show that adding columns in the column space of an incoherent matrix does not change the incoherence condition for the columns that were present previously.

\begin{lemma}
  \label{lem:clInc}
  Let $M \in \mathbb{R}^{m \times n}$ be a rank $r$, $\mu$ incoherent matrix with singular value decomposition $U\Sigma V^{\top}$. Then adding matrix $C$ to $M$ such that $\supp{C} \cap \supp{M} = \phi$ and $\Pr{U}(C) = C$, then if $U^\prime \Sigma^\prime (V^\prime)^\top$ is the singular value decomposition of $M + C$, then the following inequality holds:
  \begin{equation*}
    \norm{e_{i}^\top V^\prime} \leq \mu \sqrt{\frac{r}{n}},\ \forall i \in \supp{M}
  \end{equation*}
\end{lemma}

\begin{proof}
  First, let $V_c^\top = (V^\top + \Sigma^{-1}U^\top C)$. We can now write $M + C = U\Sigma (V + V_c)$. $V^\prime$ now forms an orthogonal basis for $V + V_c$. Note that $\supp{V^\top} \cap \supp{V_c^\top} = \phi$. Hence, there exists an upper triangular matrix $R$ and an orthogonal matrix $Q$ such that $(V + V_c)RQ = V^\prime$. Now, we note that $(Q^\top R^\top) (I + V_c^\top V_c) RQ = I$ which implies $R^\top (I + V_c^\top V_c)R = I$. From this, we obtain that $\norm{R} \leq 1$. We continue to bound the required quantity as follows:
  \begin{equation*}
    \norm{e_{i}^\top V^\prime} = \norm{e_{i}^\top (V + V_c)RQ} \overset{(\zeta_1)}{\leq} \norm{e_{i}^\top(V + V_c)} \overset{(\zeta_2)}{\leq} \mu\sqrt{\frac{r}{n}}
  \end{equation*}
  Where $(\zeta_1)$ and $(\zeta_2)$ follow from the bound on $\norm{R}$ and the fact that $i \in \supp{M}$.
\end{proof}

We will denote by $\Ct[q]$ as the corrupted columns that have not been thresholded by the algorithm before inner iteration $q$. We will see that we will never threshold a column $i \in \supp{\Lo}$. Therefore, we can write $\Mt = \Lo + \Ct[q]$. In all the lemmas that follow, we will assume that $\thresh$ and $\incThresh$ are set to $2\mu\sqrt{\frac{r}{n}}$ and $2\mu\sqrt{\frac{r}{n}}$ respectively.

The theorem is proved by induction over the inner and outer loops respectively. We will first state a lemma which guarantees progress in the inner iteration.

\begin{lemma}
  \label{lem:inItProg}
  Let $\Mo = \Lo + \Co$ be a matrix such that $\Lo$ and $\Co$ satisfies Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Also, assume that the following conditions hold before the $q^{th}$ inner iteration:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{1,\ldots,k-1\}$
  \end{enumerate}
  Then, after the $q^{th}$ inner iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\supp{\Lo} \subset \supp{\Mt[q + 1]}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  First, we note that $\sigma_{k}(\Mt{q}) \geq \sigma^*_{k}$. We now decompose $\Mt{q}$ as $\Pr{U^*_{\sigma^*_k / 2}}(\Mt{q}) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Lo) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])$. Let $U_k$ denote singular vectors corresponding to the top $k$ singular vales of $\Mt$. We will now bound $\norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k / 2}}}^\perp}$.

  % By Weyl's perturbation inequality, we have
  % \begin{equation}
  %   \sigma_{i}(\Mt[q]) \leq \sigma^*_{i} + \norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])} \overset{(\zeta_1)}{\leq} \frac{16}{31} \sigma^*_k
  % \end{equation}

  By the Davis Kahan theorem, we get the following bound:
  \begin{equation}
    \label{eqn:projBound}
    \norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k} / 2}}^\perp} \leq \frac{\norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])}}{\sigma_k(\Mt{q}) - \sigma^*_{Pos^*(\sigma^*_{k} / 2) + 1}} \leq \frac{2\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])}}{\sigma^*_k}
  \end{equation}

  We now prove that the columns in the support of $\Lo$ are not thresholded by the algorithm. We fix $i$ such that $i \in \supp{\Lo}$.

  \begin{align}
    \label{eqn:clBound}
    \norm{(I - U_kU_k^\top) \Lo_i} &= \norm{(I - U_kU_k^\top) (\Lo + \Pr{U^*}(\Ct[q])) e_i} \\
        &\leq \mu\sqrt{\frac{r}{n}} \norm{(I - U_kU_k^\top) (\Lo + \Pr{U^*}(\Ct[q]))} \\
        &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - U_kU_k^\top)\Mt{q}} + \norm{\Pr{U^*}^\perp(\Ct[q])}} \\
        &\leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1} (\Mt) + \norm{\Pr{U^*}^\perp(\Ct[q])}}
  \end{align}

  The above inequalities prove that a column in the support of $\Lo$ will not be thresholded as part of the thresholding procedure.

  We will now bound the quantity $\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])e_i},\ \forall i \in \{1,\ldots,n\}$. For a thresholded column, the quantity is bounded by $0$. For a column that is not thresholded, we have:
  \begin{align*}
    \eta \geq \norm{(I - U_kU_k^\top)\Ct[q + 1]e_i} &= \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i) + \Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i))} \\
    &\geq \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)U^*\Sigma^*v} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)\Lo} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Lo + \Pr{U^*_{\sigma^*_k/2}}(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Mt - \Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)
  \end{align*}

  From this, we get:
  \begin{equation}
    \label{eqn:corBound}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} \leq \frac{32}{31} \lprp{\zeta + 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)}
  \end{equation}

  With these inequalities in hand, we can proceed to bound the value of $\sigma_{k + 1}(\Mt)$. Using Weyl's inequality, we know that $\sigma_{k + 1}(\Mt) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct)}$. Here, we consider two cases:

  \textit{Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}}$.

  \textit{Case 2: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$.

  We now bound $\sigma_k(\Mt)$. Similar to Case 2 above, consider index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_k$. Again, we know that $\sigma_{k}(\Mt) \leq \sigma^*_{k} + \norm{\Pr{U^*_{k - 1}}^\perp (\Ct)}$. And we also have that $ 2\sigma^*_{k} \geq \sigma^*_{i + 1} $ and that $ (U^*_{k - 1})^\perp \subset (U^*_{\sigma^*_i / 2})^\perp $. From these two observations, we have $\sigma_k(\Mt) \leq \frac{33}{32} \sigma^*_k$.

  From \ref{eqn:clBound}, we have for $i \in \supp{\Lo}$:

  \begin{equation*}
    \norm{(I - U_kU_k^\top)L^*_i} \leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma^*_{k + 1} + \frac{1}{16} \lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}} + \frac{\sigma^*_{k + 1}}{32}} \leq 2\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{equation*}

  Similarly, from \ref{eqn:corBound}, we have:
  \begin{align*}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} &\leq \frac{32}{31} \lprp{\zeta + 16\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}\right)} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{18\sigma_{k + 1} + 2\lprp{\frac{1}{2}}^{q + 1}\sigma_{k} + 16\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + 18\sigma^*_{k + 1}} + 30 \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + 18\sigma^*_{k + 1}} + \frac{30}{32}\lprp{\lprp{\frac{1}{2}}^{q}\sigma^*_k + \sigma^*_{k + 1}}} \\
    &\leq 24 \mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  With the two inequalities defined above, we have proved the lemma.
\end{proof}

In the following lemma, we will prove that the thresholding steps at the end of the outer loop establishes control on the quantity, $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}$.

\begin{lemma}
  \label{lem:incohCont}
  Let $\Mo = \Lo + \Co$ be a matrix such that $\Lo$ and $\Co$ satisfies Assumptions \ref{as:rank} and \ref{as:colSup} respectively. Also, assume that the following conditions hold after the inner iteration in the $k^{th}$ outer iteration concludes:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[T + 1])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{0,\ldots,k\}$
  \end{enumerate}
  Then, after the $k^{th}$ outer iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k + 1} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\supp{\Lo} \subset \supp{\Mt[0]}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  Similarly to the previous lemma, we bound $ \sigma_{k + 1}(\Mt[T + 1]) $ by $ \lprp{\sigma^*_{k + 1}(\Mt[T + 1]) + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}}$. Now consider the index $i := \argmax\limits_j \sigma^*_j \geq \sigma^*_{k + 1}$. From our assumptions, we know that $\sigma^*_{i + 1} \leq 2\sigma^*_{k + 1}$. Also, we know that $(U^*_{k})^\perp \subset (U^*_{\sigma^*_{i} / 2})^\perp$. This implies that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \frac{1}{32} \sigma^*_{k + 1}$ by our assumptions on $\alpha$ and by using Lemma \ref{lem:spNrm}.

  We first prove the second claim of the lemma where we show that any column $i$ such that $i \in \supp{\Lo}$ is not thresholded.

  For the thresholding with respect to $\zeta$, we have:
  \begin{align*}
    \norm{(I - UU^\top) \Lo_i} &\leq \mu\sqrt{\frac{r}{n}}\norm{(I - UU^\top) U^*\Sigma^*} \\
    &\leq \mu\sqrt{\frac{r}{n}} \norm{(I - UU^\top) (\Lo + \Pr{\sigma^*_{k} / 2} (\Ct[T + 1]))} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - UU^\top) \Mt[T + 1]} + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Mt[T + 1]) + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])}} \\
    &\leq \frac{34}{32}\mu\sqrt{\frac{r}{n}}\lprp{\sigma^*_{k + 1}}
  \end{align*}

  where the last inequality holds from Lemma \ref{lem:spNrm}, our assumption on $\alpha$ and our assumption on $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])}$.

  Now, we will prove that the column $i$ is not thresholded in the second thresholding step.

  \begin{align*}
    \norm{US^{-1}U^\top \Lo_i} &\leq \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top \Lo} \\
    &\leq \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top (\Lo + \Pr{U^*_{\sigma^*_{k} / 2}} (\Ct)} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{\norm{US^{-1}U^\top \Mt[T + 1]} + \norm{US^{-1}U^\top \Pr{U^*_{\sigma^*_{k} / 2}}^\perp (\Ct)}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{2}{\sigma^*_{k + 1}} \norm{\Pr{U^*_{\sigma^*_{k}}}^\perp (\Ct)}} \\
    &\leq \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{2}{\sigma^*_{k + 1}} \frac{\sigma^*_{k + 1}}{32}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}}
  \end{align*}

  Thus, we have proved the second claim of the lemma. We will now prove the first claim of the lemma. We first note that a column $i \in \supp{\Ct[T + 1]}$ can be written as $USv + v_{res}$ such that $\norm{v} \leq 2\mu\sqrt{\frac{r}{n}}$ and $\norm{v_{res}} \leq \zeta$. We now prove claim 2 as follows:

  \begin{align*}
    &\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]_i}\\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top (USv + v_{res})} \\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top USv} +  \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top v_{res}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 4\mu\sqrt{\frac{r}{n}} \frac{2}{\sigma^*_{k + 1}} \sigma_{k + 1}(\Mt[T + 1]) \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 9 \mu\sqrt{\frac{r}{n}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{2\sigma_{k + 1}(\Mt[T + 1])}{\sigma^*_{k + 1}}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{33}{16}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \lprp{\Lo + \Ct[T + 1]}}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{1 + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]}} \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\norm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \norm{\sum\limits_{i = Pos^*(\sigma^*_k / 2) + 1}^{Pos^*(\sigma^*_{k + 1} / 2)} \frac{u^*_i (u^*_i)^\top}{\sigma^*_i} \Ct[T + 1]}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\sqrt{\alpha n} \itnorm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \frac{2\sqrt{\alpha n}}{\sigma^*_{k + 1} / 2} \itnorm{\Pr{U^*_{\sigma^*_{k} / 2}}^\perp \Ct}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu \sqrt{\frac{r}{n}} \lprp{\frac{1}{32} + \frac{1}{32}} \\
    &\leq 16\mu\sqrt{\frac{r}{n}}
  \end{align*}

  This establishes Claim 2 of the lemma.

\end{proof}

We can now prove the main theorem of the paper.

\begin{proof}
  \textit{Proof of Theorem \ref{thm:master}}
  We analyze the first outer iteration separately. And we subsequently prove the theorem through induction on the inner and outer iterations.

  First, we note that $\sigma_1 (\Mo) \geq  \sigma^*_1$. For our setting of $\thresh$, this ensures that we never threshold a column $i \in \supp{\Lo}$. We now prove an upper bound on $\sigma_1(\Mt[T + 1])$ at the end of the first inner iteration.

  We have the following recurrence inequality for $\sigma_1(\Mt[q]) \ \forall q \geq 1$ from Weyl's inequality and our condition on $\alpha$.
  \begin{equation}
    \label{eqn:sig1Rec}
    \sigma_1(\Mt[q]) \leq \sigma_1^* + \norm{\Ct[q - 1]} \leq \sigma_1^* + \frac{1}{64} \sigma_1(\Mt[q - 1])
  \end{equation}

  By expanding on this recurrence and from our setting of $T$, we get:
  \begin{equation}
    \sigma_1(\Mt[T + 1]) \leq \sigma_1^* \sum\limits_{i = 0}^{T} \lprp{\frac{1}{64}}^i + \lprp{\frac{1}{64}}^T \sigma_1(\Mo) \leq \frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n}
  \end{equation}

  In the if condition at the end of the first inner iteration, we consider two cases:
  \\
  \textit{Case 1: The Algorithm Breaks} In this case, we know that $\frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n} \leq \frac{\epsilon}{10n}$ which implies that $\sigma^*_1 \leq \frac{\epsilon}{10n}$. With this inequality, we have $\frob{\Lo - \Pr{r}(\Mt[T + 1])} \leq \frob{\Lo} + \frob{\Pr{r}(\Mt[T + 1])} \leq \sqrt{r} (\frac{\epsilon}{10n} + \frac{\epsilon}{10n}) \leq \frac{\epsilon}{5\sqrt{n}}$. Also, given our assumption on $\epsilon$, we have eliminated all the corrupted columns of $\Mo$.
  \\
  \textit{Case 2: The Algorithm Continues To the Next Iteration} In this case, we know that $\sigma_1^* \geq \frac{\epsilon}{12n}$. We will now prove that the assumptions of Lemma 4 are satisfied at the end of the first inner iteration.

  We know that each column $i$, satisfies:
  \begin{equation*}
    \label{eqn:fItColBnd}
     \norm{\Ct[T + 1]_i} \leq 2\mu\sqrt{\frac{r}{n}}\frac{65}{64} \sigma^*_1 + \frac{\epsilon}{20n} \leq 4\mu\sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  The first assumption of Lemma \ref{lem:incohCont} is trivially satisfied as the inner summation is an empty sum. The second assumption also holds simply because of the bound on the length of each column from equation \ref{eqn:fItColBnd}.

  We can thus apply Lemma \ref{lem:incohCont} at the end of the first inner iteration.

  We will now use induction on $k$ and $q$, to prove the theorem. When using induction over $q$, we will assume that the conditions of Lemma \ref{lem:inItProg} hold at the beginning of each inner iteration $q$. Note that conditions 2 and 3 of Lemma \ref{lem:inItProg} hold throughout an inner iteration if they hold at the beginning. By applying Lemma \ref{lem:inItProg} inductively, we arrive at the following condition which holds at the end of the $(T + 1)^{th}$ inner iteration:

  \[
    \norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp(\frac{\epsilon}{20n} + \sigma^*_{k + 1})
  \]

  Now, we will prove the correctness of the algorithm under two cases: \\
  \textit{Case 1: The Algorithm Breaks} In this case, we have that $\sigma^*_{k + 1} \leq \frac{\epsilon}{2n}$. Also, given our assumption on $\epsilon$, we have eliminated all the corrupted columns as the length of a corrupted column is bounded by $24\mu\sqrt{\frac{r}{n}}\lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}}$. Now, the matrix that is returned is indeed $\Lo$ as we do not eliminate a column $i\ i\in \supp{\Lo}$.
  \\
  \textit{Case 2: The Algorithm Continues to the Next Iteration} In this case, we have $\frac{\epsilon}{2n} \leq \sigma_{k + 1}(\Mt[T + 1]) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}$. We prove the correctness of the theorem in two subcases:
  \\
  \textit{Sub Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[T + 1])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^{T}\sigma^*_k + \sigma^*_{k + 1}} \leq \frac{1}{32}\lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}}$. Also, with this in hand, we have $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. Note that, assumption 1 of Lemma \ref{lem:incohCont} holds via the inductive hypothesis. For the second assumption, note that $\norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}} \leq 48\mu\sqrt{\frac{r}{n}}$.
  \\
  \textit{Case 2: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$. From this we know that, similarly to the previous subcase, $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. The rest of the proof proceeds similarly to the previous subcase.

  By the induction, hypothesis and noting the fact that the algorithm will always terminate in at most $r$ outer iterations, we have the correctness of the theorem.
\end{proof}


==> analysisAux.tex <==
%!TEX root = main.tex
\section{Analysis - Auxilliary Algorithm}
\label{sec:analysisAux}

In this section, we will give some bounds explaining when the algorithm introduced in the previous section will work. For our analysis, we assume that the givem matrix $M$ can be decomposed as the sum of three matrices $\Lo$, $\Co$ and $\No$ where $\Lo$ and $\Co$ satisfy Assumptions \ref{as:rank} and \ref{as:colSup} respectively. In addition to these, we require the following assumptions on $\No$ and $\Co$ to guarantee the success of Algorithm \ref{alg:aux}:

\begin{assumption}
  \label{as:nNorm}
  \textbf{Norm of $\No$: } The frobenius norm of the noise matrix $\No$ is bounded by a small constant times $\sigma^*_r$, i.e, $\frob{\No} \leq c \sigma^*_r$ for a small enough constant $c$.
\end{assumption}

\begin{assumption}
  \label{as:incResC}
  \textbf{Incoherence and Residual of $\Co$: } We require the following conditions on $\Co$:
  \begin{enumerate}
    \item $\infnorm{\Pr{U^*}^\perp \Co} \leq 60\mu\sqrt{\frac{r}{n}} \sigma^*_r$
    \item $\infnorm{\sum\limits_{i = 1}^{r} \frac{u_i^*(u_i^*)^\top \Co}{\sigma^*_i}} \leq 20\mu \sqrt{\frac{r}{n}}$
  \end{enumerate}
\end{assumption}

Assumption \ref{as:nNorm} is a bound on the amount of noise that we can tolerate while Assumption \ref{as:incResC} can be guaranteed by an initial run of Algorithm \ref{alg:ncpca} upto $k = r - 1$.

We will now prove a lemma which states that the removal of a small number of columns from an incoherent matrix preserves the incoherence and the singular values of the matrix.

\begin{lemma}
  \label{lem:clIncRem}
  Let $A \in \mathbb{R}^{m\times n}$ be a $\mu$-incoherent, rank-$r$ matrix. Let $S \subseteq [n]$ such that $\abs{S} \leq \alpha n$ with $\alpha \leq \frac{c}{\mu^2r}$ be used to index a subset of columns of $A$. Let $A^\prime$ be defined as follows:
  \begin{equation*}
    A^\prime_{:, i} =
    \begin{cases}
      & A_{:, i},\ i \not\in S \\
      & 0, \text{ otherwise}
    \end{cases}
  \end{equation*}

  In other words, $A^\prime$ is the matrix obtained by setting the columns corresponding to the indices in $S$ to $0$. Let the $A = USV^\top$ and $A^\prime = U^\prime S^\prime (V^\prime)^\top$ denote the singular value decompositions of $A$ and $A^\prime$ respectively. We have for all $S$ satisfying the contraints with small enough constant $c$, the following bound on the incoherence of $A^\prime$:

  \begin{equation*}
    \norm{e_i^\top V^\prime} \leq \frac{65}{64} \mu \sqrt{\frac{r}{n}}, \qquad A = U^\prime S^\prime V^{\prime\prime} \text{ with } \norm{e_i^\top V^{\prime\prime}} \leq \frac{65}{64} \mu \sqrt{\frac{r}{n}}, \qquad \frac{63}{64} \sigma_i(A) \leq \sigma_i(A^\prime) \leq \sigma_i(A)
  \end{equation*}
\end{lemma}

\begin{proof}
  It is easy to see that $V^\prime$ is a full rank matrix for small enough $c$. Now, since $V^\prime$ forms the basis of the right singular vectors of $A^\prime$, there exists a matrix $R \in \mathbb{m\times n}$ such that $(V - \Pr{S}(V)) R = V^\prime$. From our condition on $S$, we know that for any vector $x \in \{y \in \mathbb{R}^r:  \norm{y} = 1\}$, $\norm{(V - \Pr{S}(V))x}$ can be bounded as follows:
  \begin{equation*}
    1 - c \leq \norm{Vx} - \norm{\Pr{S}(V)x} \leq \norm{(V - \Pr{S}(V)) x} \leq 1
  \end{equation*}
  From this, we get that for any vector $w$ such that $\norm{w} = 1$, we have:
  \begin{equation*}
    (1 - c) \norm{Rw} \leq 1 \leq \norm{Rw}
  \end{equation*}
  This means that all the singular values of $R$ are between $1$ and $\frac{1}{1-c}$ where $c$ can be arbitrarily small. From the fact that $(V - \Pr{S}(V))R = V^\prime$, we have the first claim of the lemma.

  For the second claim of the lemmma, note that $U^\prime S^\prime (V^\prime)^\top = US(V - \Pr{S} (V))^\top$. Along with the fact that $(V - \Pr{S}(V))R = V^\prime$ and noting that $(V - \Pr{S}(V))$ is a full rank matrix, we get that $U^\prime S^\prime R^\top = US$. This means that we can write the matrix $A$ as $A = U^\prime S^\prime R^\top V^\top $. The second claim of the lemma follows from the incoherence of $V$ and the bound on singular values of $R$.

  For the final claim of the lemma, we note that the singular values of $A^\prime$ are the singular values of $USR^{-1}$. We will first prove the upper bound in the lemma. We know that $\sigma_i (A^\prime) = \min\limits_{W \in \mathbb{R}^{m \times i - 1}, W^\top W = I} \norm{(I - WW^\top) A^\prime}$. From this identity, the upper bound can be obtained by setting $W$ to $U_{:, 1:i - 1}$ and noting that the singular values of $R^{-1}$ are between $1 - c$ and $1$. For the lower bound, consider any $W$ which forms the basis of an $(i - 1)$-dimensional subspace. Now, there exists $v \in span(U_{:, 1:i}) : v^\top W = 0 \text{ and } \norm{v} = 1$. For this $v$, we have that $(1-c)\sigma_i(A) \leq v^\top USR^{-1}$. Since, such a $v$ exists for all choices of $W$, the lower bound is proved.
\end{proof}

We will denote the columns of $\Lo$, $\Co$ and $\No$ in the support of $\Mt{t}$ by $\Lot{t}$, $\Cot{t}$ and $\Not{t}$ respectively. An important quantity required for our proof to go through is the projection of $\Cot{t}$ orthogonal to the row space of $\Lo$, i.e $\frob{\Pr{U^*}^\perp (\Cot{t})}$. We will show progress in the estimation of the subspace depends on $\frob{\Pr{U^*}^\perp (\Cot{t})}$. Specifically, we show how the quantity $\frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}$ depends on $\frob{\Pr{U^*}^\perp (\Cot{t})}$

\begin{lemma}
  \label{lem:auxLProg}
  Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC}, and $\No$ satisfies \ref{as:nNorm}. In the $t^{th}$ iteration of the algorithm:
  \begin{equation*}
    \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \leq 4\frob{\No} + 2\frob{\Pr{U^*}^\perp (\Cot{t})}
  \end{equation*}
\end{lemma}

\begin{proof}
  We prove the lemma as follows:
  \begin{align*}
    & \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \overset{(\zeta_1)}{\leq} \frob{(I - U^{(t)}(U^{(t)})^\top) (\Lo - \Lot{t})} + \frob{(I - U^{(t)}(U^{(t)})^\top) \Lot{t}} \\
    & \leq (1 + \frac{1}{32}) \frob{(I - U^{(t)}(U^{(t)})^\top) \Lot{t}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^{(t)}(U^{(t)})^\top) \lprp{\Lot{t} + \Not{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    % & \leq \frac{33}{32} \lprp{\sigma_{r + 1}(\Lot{t} + \Not{t} + \Cot{t}) + \frob{\No}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^{(t)}(U^{(t)})^\top) \lprp{\Lot{t} + \Not{t} + \Cot{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    & \leq \frac{33}{32} \lprp{\frob{(I - U^*(U^*)^\top) \lprp{\Lot{t} + \Not{t} + \Cot{t}}} + \frob{(I - U^{(t)}(U^{(t)})^\top)\Not{t}}} \\
    & \overset{(\zeta_2)}{\leq} \frac{33}{32} \lprp{2\frob{\No} + \frob{\Pr{U^*}^\perp (\Not{t} + \Cot{t})}} \\
    & \leq \frac{33}{32} \lprp{3\frob{\No} + \frob{\Pr{U^*}^\perp (\Cot{t})}} \\
    & \leq 4\frob{\No} + 2\frob{\Pr{U^*}^\perp (\Cot{t})}
  \end{align*}
  where $(\zeta_1)$ follows from Lemma \ref{lem:clIncRem} and the column sparsity of $\Lo - \Lot{t}$ and $(\zeta_2)$ follows from Weyl's inequality and the fact that $\supp{\Cot{t}} \cap \supp{\Lot{t} + \Not{t}} = \phi$.
\end{proof}

In the next lemma, we show how the quantity $\frob{\Pr{U^*}^\perp (\Cot{t + 1})}$ depends on the improved estimation of $U^*$.

\begin{lemma}
  \label{lem:auxCProg}
  Let $\Mo = \Lo + \Co + \No$ such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC}, and $\No$ satisfies \ref{as:nNorm}. In the $t^{th}$ iteration of the algorithm:
  \begin{equation*}
    \frob{\Pr{U^*}^\perp (\Cot{t + 1})} \leq 3 \frob{\No} + \frac{1}{20} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}
  \end{equation*}
\end{lemma}
\begin{proof}
  To prove the lemma, we bound quantity $\norm{\Pr{U^*}^\perp ((\Cot{t + 1})_{:, i})}$ for each column $i$. For a column $i \in \supp{\Co}$, we consider two cases: \\
  \textit{Case 1: Column $i$ is thresholded} \\
  In this case, we have directly $\norm{\Pr{U^*}^\perp ((\Cot{t + 1})_{:, i})} = 0$. \\
  \textit{Case 2: Column $i$ is not thresholded} \\
  If $i$ is not thresholded, there exists a column $j_i \in \supp{\Lo + \No}$ such that $\norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}} \leq \norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, i} + \Co_{:, i})}$ (Note that this can be done with a different index $j_i$ for each column $i$ that is not thresholded). We first begin by providing a lower bound on $\norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}}$. We do this as follows:
  \begin{multline*}
     \norm{(I - U^{(t)}(U^{(t)})^\top) \Co_{:, i}} = \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}(\Co_{:, i}) + \Pr{U^*}^\perp(\Co_{:, i}))} \\ \geq \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}^\perp(\Co_{:, i})} - \norm{(I - U^{(t)}(U^{(t)})^\top) (\Pr{U^*}(\Co_{:, i})} \\ \overset{(\zeta_1)}{\geq} \frac{31}{32} \norm{\Pr{U^*}^\perp (\Co_{:, i})} - 20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}
  \end{multline*}
  Here, $(\zeta_1)$ follows from a bound on $\Pr{U^{(t)}}^\perp \Pr{U^*}^\perp$ obtained via the Davis Kahan along with Assumptions \ref{as:nNorm} and \ref{as:incResC} for the first term and from using Assumption \ref{as:incResC} for the second term.

  We can now prove a bound on $\frob{\Pr{U^*}^\perp (\Cot{t + 1})}$:
  \begin{align*}
    & \frob{\Pr{U^*}^\perp (\Cot{t + 1})} \\
    & \leq \frac{33}{32} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \lprp{\norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, j_i} + \No_{:, j_i})} + 20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^2}^\frac{1}{2} \\
    & \leq \frac{33}{32} \sqrt{2} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \lprp{\norm{(I - U^{(t)}(U^{(t)})^\top) (\Lo_{:, j_i} + \No_{:, j_i})}}^2 + \lprp{20 \mu \sqrt{\frac{r}{n}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^2}^{\frac{1}{2}} \\
    & \leq \frac{33}{16} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2 + \norm{(I - U^{(t)}(U^{(t)})^\top) \No_{:, j_i}}^2}^\frac{1}{2} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \begin{aligned}
     & \leq \frac{33}{16} \lprp{\lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2}^\frac{1}{2} + \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \No_{:, j_i}}^2}^\frac{1}{2}} + \\
     & \qquad \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
     \end{aligned} \\
    & \leq \frac{33}{16} \lprp{\sum\limits_{i \in \supp{\Cot{t + 1}}} \norm{(I - U^{(t)}(U^{(t)})^\top) \Lo_{:, j_i}}^2}^\frac{1}{2} + 3 \frob{\No} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \leq \frac{33}{16} \lprp{\mu^2\frac{r}{n}\sum\limits_{i \in \supp{\Cot{t + 1}}} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo}}^\frac{1}{2} + 3 \frob{\No} + \frac{1}{25} \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} \\
    & \leq \frac{1}{20}  \frob{(I - U^{(t)}(U^{(t)})^\top) \Lo} + 3 \frob{\No}
  \end{align*}
\end{proof}

We are now ready to prove a theorem which guarantees the correctness of our algorithm under the assumptions stated. Recall that the true sparsity of $\Co$ is denoted by $\alpha$.

\begin{theorem}
  \label{thm:aux}
  Let $\Mo = \Lo + \Co + \No$ be given such that $\Lo$ satisfies Assumption \ref{as:rank}, $\Co$ satisfies Assumptions \ref{as:colSup} and \ref{as:incResC} and $\No$ satisfies Assumption \ref{as:nNorm}. Then, Algorithm \ref{alg:aux} run with $\alpha^\prime = \alpha$. returns a matrix $\Mt[T + 1]$ which satisfies:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 20 \frob{\No} + \frac{\epsilon}{n^2}
  \end{equation*}
  where $U^{(T + 1)}$ denotes the top-$r$ left singular vectors of $\Mt[T + 1]$.
\end{theorem}

\begin{proof}
  Note that the first singular value of $\Mo$ is at least $\frac{31}{32} \sigma^*_1$ from using Weyl's inequality along with our assumptions on $\No$ and $\Co$. In addition, we also have:
  \begin{multline*}
    \frob{(I - U^{(0)}(U^{(0)})^\top) \Lo} \leq \frob{(I - U^{(0)}(U^{(0)})^\top) (\Lo + \No)} + \frob{\No} \overset{(\zeta_1)}{\leq} \frob{\No} + \frob{(I - U^{(0)}(U^{(0)})^\top) (\Lo + \No + \Co)} \\
    \overset{(\zeta_2)}{\leq} 2\frob{\No} + \frob{\Pr{U^*}^\perp \Co} \leq \frac{1}{8} \sigma^*_r
  \end{multline*}
  where $(\zeta_1)$ follows from the fact that $\supp{\Lo + \No} \cap \supp{\Co} = \phi$ and $(\zeta_2)$ follows from the fact that $U^{(0)}$ are the top-$r$ left singular vectors of $\Lo + \Co + \No$.

  Now, from Lemmas \ref{lem:auxLProg} and \ref{lem:auxCProg}, we get the following recursion:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 4\frob{\No} + 2 \frob{\Pr{U^*}^\perp (\Cot{T + 1})} \leq 10\frob{\No} + \frac{1}{20} \frob{(I - U^{(T)}(U^{(T)})^\top) \Lo}
  \end{equation*}
  By applying the recursion $T + 1$ times, we get:
  \begin{equation*}
    \frob{(I - U^{(T + 1)}(U^{(T + 1)})^\top) \Lo} \leq 20\frob{\No} + \lprp{\frac{1}{20}}^{T + 1} \frob{(I - U^{(0)}(U^{(0)})^\top) \Lo} \leq 20\frob{\No} + \frac{\epsilon}{n^2}
  \end{equation*}
  where the last inequality follows from our bound on $\frob{(I - U^{(0)}(U^{(0)})^\top) \Lo}$ and out definition of $T$.
\end{proof}


==> analysisN.tex <==
%!TEX root = rpca.tex
\renewcommand{\u}{\bm{u}}
\section{Analysis - With Noise}
\label{sec:analysisN}

We will state the main theorem for the noisy case here:
\begin{theorem}
  \label{thm:masterN}
  Let $\Mo = \Lo + \Co + \No,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo,\ \Co \text{ and } \No$ satisfying Assumptions \ref{as:rank} , \ref{as:colSup} and \ref{as:nNorm} respectively. Then, there exists two matrices $\widetilde{L}$ and $\widetilde{C}$ such that $\widetilde{L} + \widetilde{C} = \Lo + \Co$, $\Pr{U^*}(\widetilde{L}) = \widetilde{L}$ and $\Pr{\supp{\Co}} (\widetilde{C}) = \widetilde{C}$ satisfying:
  \begin{equation*}
    \norm{\widetilde{L} - \widehat{L}} \leq \frac{\epsilon}{5\sqrt{n}} + 25 \frob{\No}, \qquad \norm{\widetilde{C} - \widehat{C}} \leq \frac{\epsilon}{5\sqrt{n}} + 25 \frob{\No}
  \end{equation*}
\end{theorem}

We can now prove the correctness of Algorithm \ref{alg:ncpcan}. In addition to Assumptions \ref{as:rank} and \ref{as:colSup} on $\Lo$ and $\Co$ respectively, we will also require Assumption \ref{as:nNorm} on the noise matrix $\No$. Throughout the lemmas that will follow, we will assume that only a small fraction of columns of $\Lo$ have been thresholded by the algorithm. Specifically, we will assume that only a $\frac{c}{\mu^2r}$ fraction of columns in the support of $\Lo$ have been thresholded. We will show that this will indeed happen when we prove the main theorem of this section.

% \begin{theorem}
%   \label{thm:master}
%   Let $\Mo = \Lo + \Co,\ \Mo, \Lo, \Co \in \mathbb{R}^{m\times n}$ with $\Lo\text{ and }\Co$ satisfying Assumptions \ref{as:rank} and \ref{as:colSup} respectively and $\epsilon$ set such that $\epsilon \leq \min\limits_i \norm{\Pr{U^*}^\perp(\Co_i)}$. Then, Algorithm \ref{alg:ncpca} run with parameters $\thresh \text{ and } \beta$ set to $2\mu\sqrt{\frac{r}{n}}$ returns $L$ satisfying:
%   \begin{equation*}
%     \frob{L - \Lo} \leq \epsilon
%   \end{equation*}
% \end{theorem}

Similar to the proof for the non-noisy case, we track two important quantities:
\begin{equation}
  \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])},\ \itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}
\end{equation}

We well state an analogue to Lemma \ref{lem:inItProg} which will guarantee progress in an inner iteration of our algorithm. We will use $\Lot{q}$, $\Cot{q}$ and $\Not{q}$ to refer to the matrices $\Lo$, $\Co$ and $\No$ projected onto the column support of $\Mt[q]$. The last two claims of the lemma are used to show that the norm of $\No$ in a column in the support of $\Lo$ that has been thresholded is sufficiently high to ensure that not too many columns of $\Lo$ are thresholded.

\begin{lemma}
  \label{lem:inItProgN}
  Let $\Mo = \Lo + \Co + \No$ be a matrix such that $\Lo$, $\Co$ and $\No$ satisfy Assumptions \ref{as:rank}, \ref{as:colSup} and \ref{as:nNorm} respectively. Also, assume that the following conditions hold before the $q^{th}$ inner iteration:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{1,\ldots,k-1\}$
    \item $ \frac{\supp{\Lot{q}}}{n} \geq 1 - \frac{c}{\mu^2r} $ for a small enough constant $c$
  \end{enumerate}
  Then, after the $q^{th}$ inner iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\itnorm{(I - U_kU_k^\top) \Lot{q}} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
    \item $\zeta_q \geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}$
  \end{enumerate}
\end{lemma}

\begin{proof}
  First, we note that $\sigma_{k}(\Mt[q]) \geq \frac{63}{64}\sigma^*_{k} - \norm{\No}$. We now decompose $\Mt{q}$ as $\Pr{U^*_{\sigma^*_k / 2}}(\Mt{q}) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Lo) + \Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q]) + \Not{q}$. Let $U_k$ denote singular vectors corresponding to the top $k$ singular vales of $\Mt$. We will now bound $\norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k / 2}}}^\perp}$.

  By the Davis Kahan theorem, we get the following bound:
  \begin{equation}
    \label{eqn:projBound}
    \norm{\Pr{U_k}\Pr{U^*_{\sigma^*_{k} / 2}}^\perp} \leq \frac{\norm{\Pr{U^*_{\sigma^*_k / 2}}^\perp(\Ct[q])} + \norm{\No}}{\sigma_k(\Mt{q}) - \sigma^*_{Pos^*(\sigma^*_{k} / 2) + 1}} \leq \frac{17\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])}}{8\sigma^*_k}
  \end{equation}

  We will now analyze a fixed column in the support of $\Lot{q}$. We fix $i$ such that $i \in \supp{\Lo}$.

  \begin{align}
    \label{eqn:clBound}
    \norm{(I - U_kU_k^\top) \Lo_i} &= \norm{(I - U_kU_k^\top) (\Lot{q} + \Pr{U^*}(\Ct[q])) e_i} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{(I - U_kU_k^\top) (\Lot{q} + \Pr{U^*}(\Ct[q]))} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - U_kU_k^\top)\Mt[q]} + \norm{\No} + \norm{\Pr{U^*}^\perp(\Ct[q])}} \\
        &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1} (\Mt) + \norm{\Pr{U^*}^\perp(\Ct[q])} + \norm{\No}}
  \end{align}

  We will now bound the quantity $\norm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q + 1])e_i},\ \forall i \in \{1,\ldots,n\}$. For a thresholded column, the quantity is bounded by $0$. For a column that is not thresholded, we have:
  \begin{align*}
    \eta \geq \norm{(I - U_kU_k^\top)\Ct[q + 1]e_i} &= \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i) + \Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i))} \\
    &\geq \norm{(I - U_kU_k^\top)(\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)\Pr{U^*_{\sigma^*_k/2}} (\Ct[q + 1]e_i))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \norm{(I - U_kU_k^\top)U^*\Sigma^*v} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)\Lot{q}} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Lot{q} + \Pr{U^*_{\sigma^*_k/2}}(\Ct[q]))} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\norm{(I - U_kU_k^\top)(\Mt - \Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q]) - \Not{q})} \\
    &\geq \frac{31}{32}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} - \frac{33}{2} \mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}} \right)
  \end{align*}

  From this, we get:
  \begin{equation}
    \label{eqn:corBound}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} \leq \frac{32}{31} \lprp{\zeta + \frac{33}{2}\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}} \right)}
  \end{equation}

  With these inequalities in hand, we can proceed to bound the value of $\sigma_{k + 1}(\Mt)$. Using Weyl's inequality, we know that $\sigma_{k + 1}(\Mt) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct)} + \norm{\Not{q}}$. Here, we consider two cases:

  \textit{Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[q])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}}$.

  \textit{Case 2: } $\sigma^*_{k + 1} \geq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$.

  We now bound $\sigma_k(\Mt)$. Similar to Case 2 above, consider index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_k$. Again, we know that $\sigma_{k}(\Mt) \leq \sigma^*_{k} + \norm{\Pr{U^*_{k - 1}}^\perp (\Ct)}$. And we also have that $ 2\sigma^*_{k} \geq \sigma^*_{i + 1} $ and that $ (U^*_{k - 1})^\perp \subset (U^*_{\sigma^*_i / 2})^\perp $. From these two observations, we have $\sigma_k(\Mt) \leq \frac{33}{32} \sigma^*_k + \norm{\Not{q}}$.

  From \ref{eqn:clBound}, we have for $i \in \supp{\Lo}$:

  \begin{equation*}
    \norm{(I - U_kU_k^\top)L^*_i} \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma^*_{k + 1} + \frac{1}{16} \lprp{\lprp{\frac{1}{2}}^q\sigma^*_k + \sigma^*_{k + 1}} + \frac{\sigma^*_{k + 1}}{32} + 2\norm{\Not{q}}} \leq \frac{5}{4}\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{equation*}

  We can also prove a lower bound on $\zeta$ as follows:
  \begin{align*}
    &\zeta = 2\mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma_k(\Mt) + \sigma_{k + 1} (\Mt)} \\
    &\geq 2\mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma_k(\Lot{q}) + \sigma_{k + 1} (\Lot{q}) - 3\norm{\Not{q}}} \\
    &\geq \frac{31}{16} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}} \\
    &\geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1} \sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  This proves the third claim of the lemma.

  Similarly, from \ref{eqn:corBound}, we have:
  \begin{align*}
    \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp (\Ct[q + 1]e_i)} &\leq \frac{32}{31} \lprp{\zeta + \frac{33}{2}\mu\sqrt{\frac{r}{n}}\left(\sigma_{k + 1}(\Mt) + \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \norm{\Not{q}}\right)} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{37}{2}\sigma_{k + 1} + 2\lprp{\frac{1}{2}}^{q + 1}\sigma_{k} + \frac{33}{2}\norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + \frac{33}{2} \norm{\Not{q}}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \frac{37}{2}\sigma^*_{k + 1}} + 36 \norm{\Pr{U^*_{\sigma^*_k/2}}^\perp(\Ct[q])} + 27 \norm{\Not{q}}} \\
    &\leq \frac{32}{31} \mu\sqrt{\frac{r}{n}} \lprp{\frac{33}{32}\lprp{\lprp{\frac{1}{2}}^{q} \sigma^*_k + \frac{37}{2}\sigma^*_{k + 1}} + \frac{36}{32}\lprp{\lprp{\frac{1}{2}}^{q}\sigma^*_k + \sigma^*_{k + 1}} + 27 \norm{\Not{q}}} \\
    &\leq 24 \mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^{q + 1}\sigma^*_k + \sigma^*_{k + 1}}
  \end{align*}

  With the two inequalities defined above, we have proved the lemma.
\end{proof}

In the following lemma, we will prove that the thresholding steps at the end of the outer loop establishes control on the quantity, $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[q]}{\sigma^{*}_i}}$.

\begin{lemma}
  \label{lem:incohContN}
  Let $\Mo = \Lo + \Co + \No$ be a matrix such that $\Lo$, $\Co$ and $\No$ satisfy Assumptions \ref{as:rank}, \ref{as:colSup} and \ref{as:nNorm} respectively. Also, assume that the following conditions hold after the inner iteration in the $k^{th}$ outer iteration concludes:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[T + 1])} \leq 48\mu\sqrt{\frac{r}{n}}\sigma^*_{i + 1} \quad \forall i \in \{0,\ldots,k\}$
  \end{enumerate}
  Then, after the $k^{th}$ outer iteration, we have:
  \begin{enumerate}
    \item $\itnorm{\sum\limits_{i = 1}^{Pos^{*}(\sigma^{*}_{k + 1} / 2)} \frac{u^{*}_i (u^{*}_i)^\top \Ct[T + 1]}{\sigma^{*}_i}} \leq 16\mu \sqrt{\frac{r}{n}}$
    \item $\itnorm{US^{-1}U^\top \Lo} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}}$
    \item $\norm{US^{-1}U^\top} \leq \frac{31}{32\sigma^*_{k + 1}}$
    \item $\itnorm{(I - UU^\top) \Lo} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}$
    \item $\zeta \geq \frac{3}{2} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}$
  \end{enumerate}
\end{lemma}

% TODO: Finish Lemma
\begin{proof}
  Similarly to the previous lemma, we bound $ \sigma_{k + 1}(\Mt[T + 1]) $ by $ \lprp{\sigma^*_{k + 1}(\Mt[T + 1]) + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} + \Not{T + 1}}$. Now consider the index $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. From our assumptions, we know that $\sigma^*_{i + 1} \leq 2\sigma^*_{k + 1}$. Also, we know that $(U^*_{k})^\perp \subset (U^*_{\sigma^*_{i} / 2})^\perp$. This implies that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \frac{1}{32} \sigma^*_{k + 1}$ by our assumptions on $\alpha$ and by using Lemma \ref{lem:spNrm}.

  We first prove the fourth claim of the lemma:

  For the thresholding with respect to $\zeta$, we have:
  \begin{align*}
    \norm{(I - UU^\top) \Lo_i} &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}}\norm{(I - UU^\top) \Lot{T + 1}} \\
    &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{(I - UU^\top) (\Lot{T + 1} + \Pr{\sigma^*_{k} / 2} (\Ct[T + 1]))} \\
    &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{(I - UU^\top) \Mt[T + 1]} + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])} + \norm{\Not{T + 1}}} \\
    &\overset{(\zeta_1)}{\leq} \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Mt[T + 1]) + \norm{\Pr{\sigma^*_{k} / 2}^\perp (\Ct[T + 1])} + \norm{\Not{T + 1}}} \\
    &\leq \frac{35}{32}\mu\sqrt{\frac{r}{n}} \sigma^*_{k + 1} \\
    &\leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_{k + 1}
  \end{align*}

  where the $(\zeta_1)$ holds from Lemma \ref{lem:spNrm} and our assumptions on $\alpha$, $\itnorm{\Pr{U^{*}_{\sigma^{*}_{i}/2}}^\perp(\Ct[q])}$ and $\norm{\Not{T + 1}}$.

  This proves the fourth claim of the lemma. We will now prove the fifth claim of the lemma.
  \begin{equation*}
    \zeta = 4 \mu \sqrt{\frac{r}{n}} \sigma_{k + 1}(\Mt[T + 1]) \geq 4 \mu \sqrt{\frac{r}{n}} \lprp{\sigma_{k + 1}(\Lot{T + 1}) - \norm{\Not{T + 1}}} \geq 4\mu \sqrt{\frac{r}{n}} \lprp{\frac{63}{64}\sigma^*_{k + 1} - \norm{\Not{T + 1}}} \geq \frac{3}{2} \mu\sqrt{\frac{r}{n}} \sigma^*_{k + 1}
  \end{equation*}

  The third claim of the lemma, can be proved with a lower bound on $\sigma_{k + 1}(\Mt[T + 1])$:
  \begin{equation*}
    \sigma_{k + 1}(\Mt[T + 1]) \geq \sigma_{k + 1}(\Lot{T + 1}) - \norm{\Not{T + 1}} \geq \frac{31}{32} \sigma^*_{k + 1}
  \end{equation*}
  This implies the third claim of the lemma.

  We will now prove the second claim of the lemma:
  \begin{align*}
    \norm{US^{-1}U^\top \Lo_i} &\leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top \Lot{T + 1}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \norm{US^{-1}U^\top (\Lot{T + 1} + \Pr{U^*_{\sigma^*_{k} / 2}} (\Ct))} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{\norm{US^{-1}U^\top \Mt[T + 1]} + \norm{US^{-1}U^\top \Pr{U^*_{\sigma^*_{k} / 2}}^\perp (\Ct)} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{31}{32\sigma^*_{k + 1}} \norm{\Pr{U^*_{\sigma^*_{k}}}^\perp (\Ct)} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{65}{64} \mu\sqrt{\frac{r}{n}} \lprp{1 + \frac{31}{32\sigma^*_{k + 1}} \frac{\sigma^*_{k + 1}}{32} + \norm{US^{-1}U^\top\Not{T + 1}}} \\
    & \leq \frac{5}{4} \mu\sqrt{\frac{r}{n}}
  \end{align*}

  This concludes the proof of the second claim of the lemma. We will now prove the first claim of the lemma. We first note that a column $i \in \supp{\Ct[T + 1]}$ can be written as $USv + v_{res}$ such that $\norm{v} \leq 2\mu\sqrt{\frac{r}{n}}$ and $\norm{v_{res}} \leq \zeta$. We now prove claim 2 as follows:

  \begin{align*}
    &\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]_i}\\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top (USv + v_{res})} \\
    &\leq \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top USv} +  \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top v_{res}} \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 4\mu\sqrt{\frac{r}{n}} \frac{2}{\sigma^*_{k + 1}} \sigma_{k + 1}(\Mt[T + 1]) \\
    &\leq 2\mu\sqrt{\frac{r}{n}} \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top US} + 9 \mu\sqrt{\frac{r}{n}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{2\sigma_{k + 1}(\Mt[T + 1])}{\sigma^*_{k + 1}}} \\
    &\leq 9\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Mt[T + 1]} + \frac{33}{16}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{\norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \lprp{\Lot{T + 1} + \Ct[T + 1] + \Not{T + 1}}}} \\
    &\leq \frac{27}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \lprp{1 + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Ct[T + 1]} + \norm{U^*_{\sigma^*_{k + 1} / 2} (\Sigma^*_{\sigma^*_{k + 1} / 2})^{-1} (U^*_{\sigma^*_{k + 1} / 2})^\top \Not{T + 1}}} \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\norm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \norm{\sum\limits_{i = Pos^*(\sigma^*_k / 2) + 1}^{Pos^*(\sigma^*_{k + 1} / 2)} \frac{u^*_i (u^*_i)^\top}{\sigma^*_i} \Ct[T + 1]} + \frac{2\norm{\No}}{\sigma^*_{k + 1}}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu\sqrt{\frac{r}{n}} \left(\sqrt{\alpha n} \itnorm{U^*_{\sigma^*_{k} / 2} (\Sigma^*_{\sigma^*_{k} / 2})^{-1} (U^*_{\sigma^*_{k} / 2})^\top \Ct[T + 1]} + \frac{2\sqrt{\alpha n}}{\sigma^*_{k + 1} / 2} \itnorm{\Pr{U^*_{\sigma^*_{k} / 2}}^\perp \Ct[T + 1]} + \frac{1}{32}\right) \\
    &\leq \frac{31}{2}\mu\sqrt{\frac{r}{n}} + 2\mu \sqrt{\frac{r}{n}} \lprp{\frac{1}{32} + \frac{1}{32} + \frac{1}{32}} \\
    &\leq 16\mu\sqrt{\frac{r}{n}}
  \end{align*}

  This establishes Claim 1 of the lemma.

\end{proof}

We can now prove the main theorem of the paper.

\begin{proof}
  \textit{Proof of Theorem \ref{thm:masterN}} \\
  We will prove the main theorem of the paper in three stages. In the first stage, we will analyze the first outer iteration of the algorithm. In the second, we will show that the conditions required for the application of theorem \ref{thm:aux}. In the final stage, we will show the correctness of the incoherence preserving projection operator. In the first and second stages of the algorith, we will assume that at most a small fraction ($\frac{c}{\mu^2r}$ for small enough $c$) of columns of $\Lo$ are thresholded during the running of the algorithm. We will show that this will be the case when at the end of stage 2.

  \textit{Stage 1:}\\
  First, we note that $\sigma_1 (\Mt[q]) \geq \frac{63}{64} \sigma^*_1 - \norm{\No} \geq \frac{31}{32} \sigma^*_1$ from Weyl's inequality and our upper bound on the number of columns of $\Lo$ thresholded. We now prove an upper bound on $\sigma_1(\Mt[T + 1])$ at the end of the first inner iteration.

  We have the following recurrence inequality for $\sigma_1(\Mt[q]) \ \forall q \geq 1$ from Weyl's inequality and our condition on $\alpha$.
  \begin{equation}
    \label{eqn:sig1Rec}
    \sigma_1(\Mt[q]) \leq \sigma_1^* + \norm{\Ct[q - 1]} \leq \sigma_1^* + \norm{\Not{q}} + \frac{1}{64} \sigma_1(\Mt[q - 1])
  \end{equation}

  By expanding on this recurrence and from our setting of $T$, we get:
  \begin{equation}
    \sigma_1(\Mt[T + 1]) \leq \sigma_1^* \sum\limits_{i = 0}^{T} \lprp{\frac{1}{64}}^i + 2\norm{\No} + \lprp{\frac{1}{64}}^T \sigma_1(\Mo) \leq \frac{65}{64}\sigma_1^* + \frac{\epsilon}{20n}
  \end{equation}

  From our lower bounds on $\sigma_1(\Mt[q])$, we can see that the following inequalities hold:
  \begin{equation*}
    \itnorm{(I - U_1U_1^\top) \Lot{q}} \leq \frac{5}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_1, \quad \zeta_q \geq \frac{7}{4} \mu \sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  In the if condition at the end of the first inner iteration, we consider two cases: \\
  \textit{Case 1: The Algorithm Returns} In this case, we know that $\frac{31}{32}\sigma_1^* \leq \frac{\epsilon}{10n}$ which implies that $\sigma^*_1 \leq \frac{\epsilon}{12n}$. With this inequality, we return the empty matrix for $\widehat{L}$ and $\Mo$ as estimates of $\Lo$ and $\Co$ respectively. Given our bound on the singular values of $\Lo$ (and $\No$), the statement of the theorem follows.
  \\
  \textit{Case 2: The Algorithm Continues To the Next Iteration} In this case, we know that $\sigma_1^* \geq \frac{\epsilon}{12n}$. This follows from using the upper bound $\sigma_1(\Mt[T + 1]) \leq \sigma^*_1 + \norm{\No} + \norm{\Ct[T + 1]}$. We will now prove that the assumptions of Lemma 4 are satisfied at the end of the first inner iteration.

  We know that each column $i$, satisfies:
  \begin{equation*}
    \label{eqn:fItColBnd}
     \norm{\Ct[T + 1]_i} \leq 2\mu\sqrt{\frac{r}{n}} {\frac{65}{64} \sigma^*_1 + \frac{\epsilon}{20n}} \leq 4\mu\sqrt{\frac{r}{n}} \sigma^*_1
  \end{equation*}

  The first assumption of Lemma \ref{lem:incohCont} is trivially satisfied as the inner summation is an empty sum. The second assumption also holds simply because of the bound on the length of each column from equation \ref{eqn:fItColBnd}.

  We can thus apply Lemma \ref{lem:incohCont} at the end of the first inner iteration.

  \textit{Stage 2:}\\
  We will now use induction on $k$ and $q$, to prove the theorem. When using induction over $q$, we will assume that the conditions of Lemma \ref{lem:inItProgN} hold at the beginning of each inner iteration $q$. Note that conditions 2 and 3 of Lemma \ref{lem:inItProgN} hold throughout an inner iteration if they hold at the beginning. Condition 4 holds by assumption. By applying Lemma \ref{lem:inItProgN} inductively, we arrive at the following condition which holds at the end of the $(T + 1)^{th}$ inner iteration:

  \[
    \norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp(\frac{\epsilon}{20n} + \sigma^*_{k + 1})
  \]

  Now, we will prove the correctness of the algorithm under two cases: \\
  \textit{Case 1: The Algorithm Returns} In this case, we have that $\sigma^*_{k + 1} \leq \frac{\epsilon}{10n}$. Here, we will prove the correctness of the incoherence preserving projection operator. To prove the theorem, we will need to construct a candidate pair $(\widetilde{L}, \widetilde{C})$ such that $\widetilde{L}$ has the same row space of $\Lo$ and $\widetilde{C}$ has the same column space of $\Co$.
  We will choose $\widetilde{L}$ to be $\Lo + \Pr{U^*} (\Co)$. We will bound $\frob{\widehat{L} - \widetilde{L}}$ by bounding $\frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)}$ and $\norm{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)}$.
  \begin{align*}
    & \frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} \\
    &\leq \frob{\No} + \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} \\
    & \leq \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo + \No)} + \frob{\No} \\
    & \leq \frob{\Lo + \No - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo)} + \frob{\No} \\
    & \leq \frob{\Lo - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lo)} + 2\frob{\No} \\
    & \leq \frac{65}{64} \frob{\Lot{T + 1} - \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Lot{T + 1})} + 2\frob{\No} \\
    & \overset{(\zeta_1)}{\leq} \frob{\Lot{T + 1} - U^\prime (U^\prime)^\top (\Lot{T + 1})} + 2\frob{\No} \\
    & \leq \frob{(I - U^\prime (U^\prime)^\top) (\Lot{T + 1} + \Pr{U^*} (\Cot{T + 1}))} + 2\frob{\No} \\
    & \leq \frob{(I - U^\prime (U^\prime)^\top) \Mt[T + 1]} + \frob{\Pr{U^*}^\perp (\Cot{T + 1})} + 2\frob{\No} \\
    & \leq \sqrt{n} \sigma_{k + 1} (\Mt[T + 1]) + \frob{\Pr{U^*}^\perp (\Cot{T + 1})} + 2\frob{\No} \\
    & \leq \sqrt{n} \sigma^*_{k + 1} + 2\frob{\Pr{U^*_{k}}^\perp (\Cot{T + 1})} + 3\frob{\No} \\
    & \leq \sqrt{n} \frac{\epsilon}{10n} + \frac{1}{32} (\frac{\epsilon}{20n} + \sigma^*_{k + 1}) + 3\frob{\No} \\
    & \leq \frac{\epsilon}{10\sqrt{n}} + 3\frob{\No}
  \end{align*}

  We will now bound the second term:
  \begin{align*}
    & \frob{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)} \\
    & \leq \sqrt{\alpha n} \itnorm{\norm{(I - U^*(U^*)^\top) \Pr{U^\prime, S^\prime, 2\mu\sqrt{r / n}} (\Co)}} \\
    & \leq \frac{1}{32} \norm{\Pr{U^*}^\perp (US)} \\
    & \leq \frac{1}{32} \norm{\Pr{U^*}^\perp (\Pr{U}(\Mt[T + 1]) - \Mt[T + 1] + \Mt[T + 1])} \\
    & \leq \frac{1}{32} \lprp{\norm{\Pr{U^*}^\perp (\Mt[T + 1])} + \norm{\Pr{U}^\perp (\Mt[T + 1])}} \\
    & \leq \frac{1}{32} \lprp{\norm{\Pr{U^*}^\perp (\Lot{T + 1} + \Not{T + 1} + \Cot{T + 1})} + \frac{\epsilon}{20n}} \\
    & \leq \frac{1}{32} \lprp{\norm{\Not{T + 1}} + \norm{\Pr{U^*}^\perp(\Cot{T + 1})} + \frac{\epsilon}{20n}} \\
    & \leq \frac{1}{32} \lprp{\norm{\No} + \sigma^*_{k + 1} + \frac{\epsilon}{10n}} \\
    & \leq \frac{1}{32} \lprp{\frac{\epsilon}{5n} + \norm{\No}}
  \end{align*}

  Therefore, we can bound $\widetilde{L} - \widehat{L}$ by $\frac{\epsilon}{5\sqrt{n}} + 4\frob{\No}$. Similarly, by noting that $\widehat{L} + \widehat{C} = \widetilde{L} + \widetilde{C} + \No$, we can bound $\widetilde{C} - \widehat{C}$. This proves the theorem in this case.
  \\
  \textit{Case 2: The Algorithm Continues to the Next Iteration} In this case, we have $\frac{\epsilon}{2n} \leq \sigma_{k + 1}(\Mt[T + 1]) \leq \sigma^*_{k + 1} + \norm{\Pr{U^*_k}^\perp (\Ct[T + 1])}$. We prove the correctness of the theorem in two subcases:
  \\
  \textit{Sub Case 1: } $\sigma^*_{k + 1} \leq \frac{\sigma^*_{k}}{2}$. In this case, we know that $\norm{\Pr{U^*_k}^\perp (\Ct[T + 1])} \leq \sqrt{\alpha n} \itnorm{\Pr{U^{*}_{\sigma^{*}_{k}/2}}^\perp(\Ct[T + 1])} \leq \frac{1}{32}\lprp{\lprp{\frac{1}{2}}^{T}\sigma^*_k + \sigma^*_{k + 1}} \leq \frac{1}{32}\lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}}$. Also, with this in hand, we have $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. Note that, assumption 1 of Lemma \ref{lem:incohCont} holds via the inductive hypothesis. For the second assumption, note that $\norm{\Pr{U^*_{\sigma^*_k / 2}}(\Ct[T + 1])} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\lprp{\frac{1}{2}}^T\sigma^*_k + \sigma^*_{k + 1}} \leq 24\mu\sqrt{\frac{r}{n}} \lprp{\frac{\epsilon}{20n} + \sigma^*_{k + 1}} \leq 48\mu\sqrt{\frac{r}{n}}$.
  \\
  \textit{Sub Case 2: } $\sigma^*_{k + 1} \geq \frac{\sigma^*_{k}}{2}$. In this case, let $i := \argmax\limits_j \sigma^*_j \geq 2\sigma^*_{k + 1}$. We know from our assumptions that $\itnorm{\Pr{U^*_{\sigma^*_j/2}}^\perp (\Ct)} \leq 32\mu \sqrt{\frac{r}{n}} \lprp{\sigma^*_{i + 1}}$. Also, given that $2\sigma^*_{k + 1} \geq \sigma^*_{i + 1}$ and $ (U^*_{k})^\perp \subset (U^*_{\sigma^*_{i}})^\perp $, we have $\norm{\Pr{U^*_k}^\perp (\Ct)} \leq \frac{1}{32} \sigma^*_{k + 1}$. From this we know that, similarly to the previous subcase, $\sigma^*_{k + 1} \geq \frac{\epsilon}{4n}$. The rest of the proof proceeds similarly to the previous subcase.

  \textit{Stage 3:} \\
  By the induction hypothesis and Lemma \ref{lem:incohContN}, we can apply Theorem \ref{thm:aux} to $\Mt[T + 1]$. The proof of the correctness of the incoherence preserving projection is similar to the proof from \textit{Case 1} of \textit{Stage 2}.
\end{proof}


==> introAux.tex <==
%!TEX root = main.tex

\section{Auxilliary Algorithm}
\label{sec:introAux}
In this section, we will analyze a simple algorithm that we will use for the noisy case of the problem. Note that in the case where we have additive noise, we may threshold a large number of columns in the support of $\Lo$. For this reason, we use a new algorithm at the end of Algorithm~\ref{alg:ncpca} which does not threshold more than a fixed fraction of columnns of the matrix.


==> introN.tex <==
%!TEX root = main.tex
\section{Problem Definition - Noisy Case}
Given $M^{*} = L^{*} + C^{*} + N^* \text{ where } L^{*},M^{*},C^{*} \in \mathbb{R}^{m\times n}$ which is the sum of a low rank column incoherent matrix $L^{*}$, a column sparse corruption matrix $C^{*}$ with disjoint column supports and a noise matrix $N^*$, the goal is to recover $L^{*}$ and $C^{*}$.

Note that in this case, it might not be possible to exactly recover the support of $\Lo$ or the true column space of $\Lo$. We show that we can recover $\Lo$ upto a constant factor times $\frob{\No}$.


==> introduction_bk.tex <==
\section{Introduction}
Principal Component Analysis (PCA) is one of the most important first step for a typical data exploration/analysis effort. While PCA can be performed optimally and efficiently using the Singular Value Decomposition (SVD), the algorithm itself is fragile w.r.t. outliers. That is, in presence of a small number of corrupted/outlier points, SVD can output arbitrarily inaccurate principal directions. 

The goal of this work is to devise Outlier Robust PCA (ORPCA) algorithm that can recover the principal directions despite presence of a large number of outliers. Given data matrix $M=[x_1, \dots, x_n]\in \R^{d\times n}$ where $(1-\rho)$ fraction of points $x_i$ are noisy samples from a subspace $\Uo$ and the remaining $\rho$ fraction of points can be arbitrary corrupted, the goal of ORPCA is to recover $\Uo$ accurately. That is, given $M=\Lo+\Co+\No$ where $\Lo$ is a low-rank matrix, $\Co$ is a column-sparse matrix and $\No$ is a noise matrix, the goal is to recover left singular vectors of $\Lo$. 

Note that the top singular vectors of $M$ can be arbitrary far from $\Uo$ as the operator norm of $\Co$ ($\|\Co\|_2$) can be quite large when $\rho=\Omega(1)$ even if dimensionality of $\Uo$ is a constant. So, the goal of ORPCA algorithms is to exploit the column sparsity of $\Co$ to obtain better estimator for $\Uo$. That is, the goal is to find $S^*=$column-support$(\Co)$ (where column-support($A$) is the index of non-zero columns of $A$) so that $\Uo$ can be estimated using top singular directions of $M_{\bar{S^*}}$, i.e., columns of $M$ restricted to complement set of $S^*$. 

Existing result for ORPCA falls in two categories: a) nuclear norm based, b) truncated inner product based. YESHWANTH provide details here. Main thing is to say that nuclear norm based methods are $O(d^2 n)$ while (b) are weak because ...

In contrast, our approach is based on solving the following natural optimization problem: $$\textsf{(ORPCA)}:\ \ \min_{L, C} \|M-L-C\|_F^2 \text{ s.t. } rank(L)\leq r, |\text{column-support}(C)|\leq s.$$
The main challenge with ORPCA is non-convexity and combinatorial structure of the above optimization problem which rules out standard optimization tools. Instead, we propose a simple non-convex alternating projection style method for this problem. Fortunately, each of the non-convex projection onto set of low-rank matrix and set of column sparse matrix can be computed efficiently. But owing to non-convexity, the algorithm is not even guaranteed to converge in general. 

The main contribution of our work is to show that despite non-convexity of the projection sets, our algorithm recover $\Uo$ nearly optimally as long as the fraction of corrupted data points (column-support of $\Co$) is less than $O(1/r)$ where $r$  
is the dimensionality of principal subspace $\Uo$. Concretely, we study the problem in three settings: \begin{enumerate}
\item {\em Noiseless Setting}: $M=D^*+\Co$ where clean data matrix $D^*$ is a rank-$r$ matrix with $\mu$-incoherent right singular vectors (see Definition~\ref{defn:incoh}). 
\item {\em Gaussian noise Setting}: 
\item {\em Arbitrary Data Matrix}: 
\end{enumerate}
\subsection{Related Works}

==> notations_praneeth.tex <==
We use two hard -thresholding operators in this paper.
Given a matrix $\Rm$, the first hard-thresholding operator, $\mathcal{HT}_\nThresh \lprp{\Rm}$ denotes the set of indices $j$ of the top $\nThresh$ fraction of largest columns (in $\ell_2$ norm) in $\Rm$. Given a matrix $\Rm$, the second hard-thresholding operator $\widetilde{\HT{\zeta}}(\Rm)$ is defined as,
\begin{equation}
\label{eqn:httDef}
\widetilde{\HT{\zeta}}(N)=\{i:\ \text{s.t. } \|N_{i}\|_2 \geq \zeta\}.
\end{equation}
$\pperpu(M)$ denotes $(I-UU^\top)M$. For any set $\mathcal{S} \in \mathbb{R}^{d}$, we will use $\Pr{\mathcal{S}}$ to denote the projection onto the set $\mathcal{S}$. We will also use $\Pr{U}$ to denote the projection onto the column space of $U$ for $U \in \mathbb{R}^{d \times r}$.
